Evolutionary tracks, ejecta, and ionizing photons from intermediate-mass to very massive stars with PARSEC

Recent advancements in stellar evolution modeling offer unprecedented accuracy in predicting the evolution and deaths of stars. We present new stellar evolutionary models computed with the updated PARSEC V2.0 code for a comprehensive and homogeneous grid of metallicities and initial masses. Nuclear reaction networks, mass loss prescriptions, and the treatment of elemental mixing have all been updated in PARSEC V2.0. We computed models for thirteen initial metallicities spanning $Z = 10^{-11}$ to $Z = 0.03$, with masses ranging from 2.0 M$_{\odot}$ to 2000 M$_{\odot}$, consisting of a library of over 1,100 ($\sim 2100$ tracks including pure-He models) full stellar evolution tracks. For each track, the evolution is followed from the pre-main-sequence to the most advanced early-asymptotic-giant-branch or the pre-supernova phases, depending on the stellar mass. Here, we describe the properties of the tracks and their chemical and structural evolution. We computed the final fates and the remnant masses and built the mass spectrum for each metallicity, finding that the combined black hole (BH) pair-instability mass gap spans just between 100 and 130 M$_{\odot}$. Moreover, the remnant masses provide models consistent with observed BH masses, such as those from the primaries of GW190521, Cygnus X-1, and $\textit{Gaia}$ BH3 binary systems. We computed and provided the chemical ejecta from stellar winds and explosive final fates, along with the ionizing photon rates. Our results show strong overall consistency with other tracks computed with different codes. A comparison with a large sample of observed massive stars in the Tarantula Nebula of the Large Magellanic Cloud shows that our tracks nicely reproduce the majority of stars that lie on the main sequence. All the models are publicly available and can be retrieved on the PARSEC database.

==> biblio.tex <==
% -------------------------- B --------------------------

@ARTICLE{Cassisi1993,
       author = {{Cassisi}, Santi and {Castellani}, Vittorio},
        title = "{An Evolutionary Scenario for Primeval Stellar Populations}",
      journal = {\apjs},
     keywords = {Abundance, Heavy Elements, Metallicity, Stellar Evolution, Stellar Mass, Stellar Structure, Chemical Composition, Helium, Hydrogen, Astrophysics, STARS: EVOLUTION, STARS: GIANTS, STARS: INTERIORS, STARS: POPULATION II},
         year = 1993,
        month = oct,
       volume = {88},
        pages = {509},
          doi = {10.1086/191831},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993ApJS...88..509C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Costa2023,
       author = {{Costa}, Guglielmo and {Mapelli}, Michela and {Iorio}, Giuliano and {Santoliquido}, Filippo and {Escobar}, Gast{\'o}n J. and {Klessen}, Ralf S. and {Bressan}, Alessandro},
        title = "{Massive binary black holes from Population II and III stars}",
      journal = {\mnras},
     keywords = {black hole physics, gravitational waves, methods: numerical, stars: Population II, stars: Population III, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2023,
        month = oct,
       volume = {525},
       number = {2},
        pages = {2891-2906},
          doi = {10.1093/mnras/stad2443},
archivePrefix = {arXiv},
       eprint = {2303.15511},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023MNRAS.525.2891C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tanikawa2022,
       author = {{Tanikawa}, Ataru and {Chiaki}, Gen and {Kinugawa}, Tomoya and {Suwa}, Yudai and {Tominaga}, Nozomu},
        title = "{Can Population III stars be major origins of both merging binary black holes and extremely metal poor stars?}",
      journal = {\pasj},
     keywords = {gravitational waves, stars: black holes, stars: Population II, stars: Population III, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = jun,
       volume = {74},
       number = {3},
        pages = {521-532},
          doi = {10.1093/pasj/psac010},
archivePrefix = {arXiv},
       eprint = {2202.00230},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022PASJ...74..521T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kinugawa2020,
       author = {{Kinugawa}, Tomoya and {Nakamura}, Takashi and {Nakano}, Hiroyuki},
        title = "{Chirp mass and spin of binary black holes from first star remnants}",
      journal = {\mnras},
     keywords = {gravitational waves, binaries: general, stars: black holes, stars: Population III, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = nov,
       volume = {498},
       number = {3},
        pages = {3946-3963},
          doi = {10.1093/mnras/staa2511},
archivePrefix = {arXiv},
       eprint = {2005.09795},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.498.3946K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Belczynski2017,
       author = {{Belczynski}, Krzysztof and {Ryu}, Taeho and {Perna}, Rosalba and {Berti}, Emanuele and {Tanaka}, Takamitsu L. and {Bulik}, Tomasz},
        title = "{On the likelihood of detecting gravitational waves from Population III compact object binaries}",
      journal = {\mnras},
     keywords = {gravitational waves, stars: massive, Astrophysics - High Energy Astrophysical Phenomena, General Relativity and Quantum Cosmology},
         year = 2017,
        month = nov,
       volume = {471},
       number = {4},
        pages = {4702-4721},
          doi = {10.1093/mnras/stx1759},
archivePrefix = {arXiv},
       eprint = {1612.01524},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.471.4702B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Santoliquido2023,
       author = {{Santoliquido}, Filippo and {Mapelli}, Michela and {Iorio}, Giuliano and {Costa}, Guglielmo and {Glover}, Simon C.~O. and {Hartwig}, Tilman and {Klessen}, Ralf S. and {Merli}, Lorenzo},
        title = "{Binary black hole mergers from population III stars: uncertainties from star formation and binary star properties}",
      journal = {\mnras},
     keywords = {black hole physics, gravitational waves, methods: numerical, stars: Population III, galaxies: star formation, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2023,
        month = sep,
       volume = {524},
       number = {1},
        pages = {307-324},
          doi = {10.1093/mnras/stad1860},
archivePrefix = {arXiv},
       eprint = {2303.15515},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023MNRAS.524..307S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{abbottGWTC2.1,
       author = {{Abbott}, R. and {Abbott}, T.~D. and {Acernese}, F. and {Ackley}, K. and {Adams}, C. and {Adhikari}, N. and {Adhikari}, R.~X. and {Adya}, V.~B. and {Affeldt}, C. and {Agarwal}, D. and {Agathos}, M. and {Agatsuma}, K. and {Aggarwal}, N. and {Aguiar}, O.~D. and {Aiello}, L. and {Ain}, A. and {Ajith}, P. and {Albanesi}, S. and {Allocca}, A. and {Altin}, P.~A. and {Amato}, A. and {Anand}, C. and {Anand}, S. and {Ananyeva}, A. and {Anderson}, S.~B. and {Anderson}, W.~G. and {Andrade}, T. and {Andres}, N. and {Andri{\'c}}, T. and {Angelova}, S.~V. and {Ansoldi}, S. and {Antelis}, J.~M. and {Antier}, S. and {Appert}, S. and {Arai}, K. and {Araya}, M.~C. and {Areeda}, J.~S. and {Ar{\`e}ne}, M. and {Arnaud}, N. and {Aronson}, S.~M. and {Arun}, K.~G. and {Asali}, Y. and {Ashton}, G. and {Assiduo}, M. and {Aston}, S.~M. and {Astone}, P. and {Aubin}, F. and {Austin}, C. and {Babak}, S. and {Badaracco}, F. and {Bader}, M.~K.~M. and {Badger}, C. and {Bae}, S. and {Baer}, A.~M. and {Bagnasco}, S. and {Bai}, Y. and {Baird}, J. and {Ball}, M. and {Ballardin}, G. and {Ballmer}, S.~W. and {Balsamo}, A. and {Baltus}, G. and {Banagiri}, S. and {Bankar}, D. and {Barayoga}, J.~C. and {Barbieri}, C. and {Barish}, B.~C. and {Barker}, D. and {Barneo}, P. and {Barone}, F. and {Barr}, B. and {Barsotti}, L. and {Barsuglia}, M. and {Barta}, D. and {Bartlett}, J. and {Barton}, M.~A. and {Bartos}, I. and {Bassiri}, R. and {Basti}, A. and {Bawaj}, M. and {Bayley}, J.~C. and {Baylor}, A.~C. and {Bazzan}, M. and {B{\'e}csy}, B. and {Bedakihale}, V.~M. and {Bejger}, M. and {Belahcene}, I. and {Benedetto}, V. and {Beniwal}, D. and {Bennett}, T.~F. and {Bentley}, J.~D. and {BenYaala}, M. and {Bergamin}, F. and {Berger}, B.~K. and {Bernuzzi}, S. and {Berry}, C.~P.~L. and {Bersanetti}, D. and {Bertolini}, A. and {Betzwieser}, J. and {Beveridge}, D. and {Bhandare}, R. and {Bhardwaj}, U. and {Bhattacharjee}, D. and {Bhaumik}, S. and {Bilenko}, I.~A. and {Billingsley}, G. and {Bini}, S. and {Birney}, R. and {Birnholtz}, O. and {Biscans}, S. and {Bischi}, M. and {Biscoveanu}, S. and {Bisht}, A. and {Biswas}, B. and {Bitossi}, M. and {Bizouard}, M. -A. and {Blackburn}, J.~K. and {Blair}, C.~D. and {Blair}, D.~G. and {Blair}, R.~M. and {Bobba}, F. and {Bode}, N. and {Boer}, M. and {Bogaert}, G. and {Boldrini}, M. and {Bonavena}, L.~D. and {Bondu}, F. and {Bonilla}, E. and {Bonnand}, R. and {Booker}, P. and {Boom}, B.~A. and {Bork}, R. and {Boschi}, V. and {Bose}, N. and {Bose}, S. and {Bossilkov}, V. and {Boudart}, V. and {Bouffanais}, Y. and {Bozzi}, A. and {Bradaschia}, C. and {Brady}, P.~R. and {Bramley}, A. and {Branch}, A. and {Branchesi}, M. and {Brau}, J.~E. and {Breschi}, M. and {Briant}, T. and {Briggs}, J.~H. and {Brillet}, A. and {Brinkmann}, M. and {Brockill}, P. and {Brooks}, A.~F. and {Brooks}, J. and {Brown}, D.~D. and {Brunett}, S. and {Bruno}, G. and {Bruntz}, R. and {Bryant}, J. and {Bulik}, T. and {Bulten}, H.~J. and {Buonanno}, A. and {Buscicchio}, R. and {Buskulic}, D. and {Buy}, C. and {Byer}, R.~L. and {Cadonati}, L. and {Cagnoli}, G. and {Cahillane}, C. and {Bustillo}, J. Calder{\'o}n and {Callaghan}, J.~D. and {Callister}, T.~A. and {Calloni}, E. and {Cameron}, J. and {Camp}, J.~B. and {Canepa}, M. and {Canevarolo}, S. and {Cannavacciuolo}, M. and {Cannon}, K.~C. and {Cao}, H. and {Capote}, E. and {Carapella}, G. and {Carbognani}, F. and {Carlin}, J.~B. and {Carney}, M.~F. and {Carpinelli}, M. and {Carrillo}, G. and {Carullo}, G. and {Carver}, T.~L. and {Diaz}, J. Casanueva and {Casentini}, C. and {Castaldi}, G. and {Caudill}, S. and {Cavagli{\`a}}, M. and {Cavalier}, F. and {Cavalieri}, R. and {Ceasar}, M. and {Cella}, G. and {Cerd{\'a}-Dur{\'a}n}, P. and {Cesarini}, E. and {Chaibi}, W. and {Chakravarti}, K. and {Subrahmanya}, S. Chalathadka and {Champion}, E. and {Chan}, C. -H. and {Chan}, C. and {Chan}, C.~L. and {Chan}, K. and {Chandra}, K. and {Chanial}, P. and {Chao}, S. and {Charlton}, P. and {Chase}, E.~A. and {Chassande-Mottin}, E. and {Chatterjee}, C. and {Chatterjee}, Debarati and {Chatterjee}, Deep and {Chattopadhyay}, D. and {Chaturvedi}, M. and {Chaty}, S. and {Chatziioannou}, K. and {Chen}, H.~Y. and {Chen}, J. and {Chen}, X. and {Chen}, Y. and {Chen}, Z. and {Cheng}, H. and {Cheong}, C.~K. and {Cheung}, H.~Y. and {Chia}, H.~Y. and {Chiadini}, F. and {Chiarini}, G. and {Chierici}, R. and {Chincarini}, A. and {Chiofalo}, M.~L. and {Chiummo}, A. and {Cho}, G. and {Cho}, H.~S. and {Choudhary}, R.~K. and {Choudhary}, S. and {Christensen}, N. and {Chu}, Q. and {Chua}, S. and {Chung}, K.~W. and {Ciani}, G. and {Ciecielag}, P. and {Cie{\'s}lar}, M. and {Cifaldi}, M. and {Ciobanu}, A.~A. and {Ciolfi}, R. and {Cipriano}, F. and {Cirone}, A. and {Clara}, F. and {Clark}, E.~N. and {Clark}, J.~A. and {Clarke}, L. and {Clearwater}, P. and {Clesse}, S. and {Cleva}, F. and {Coccia}, E. and {Codazzo}, E. and {Cohadon}, P. -F. and {Cohen}, D.~E. and {Cohen}, L. and {Colleoni}, M. and {Collette}, C.~G. and {Colombo}, A. and {Colpi}, M. and {Compton}, C.~M. and {Constancio}, M. and {Conti}, L. and {Cooper}, S.~J. and {Corban}, P. and {Corbitt}, T.~R. and {Cordero-Carri{\'o}n}, I. and {Corezzi}, S. and {Corley}, K.~R. and {Cornish}, N. and {Corre}, D. and {Corsi}, A. and {Cortese}, S. and {Costa}, C.~A. and {Cotesta}, R. and {Coughlin}, M.~W. and {Coulon}, J. -P. and {Countryman}, S.~T. and {Cousins}, B. and {Couvares}, P. and {Coward}, D.~M. and {Cowart}, M.~J. and {Coyne}, D.~C. and {Coyne}, R. and {Creighton}, J.~D.~E. and {Creighton}, T.~D. and {Criswell}, A.~W. and {Croquette}, M. and {Crowder}, S.~G. and {Cudell}, J.~R. and {Cullen}, T.~J. and {Cumming}, A. and {Cummings}, R. and {Cunningham}, L. and {Cuoco}, E. and {Cury{\l}o}, M. and {Dabadie}, P. and {Canton}, T. Dal and {Dall'Osso}, S. and {D{\'a}lya}, G. and {Dana}, A. and {DaneshgaranBajastani}, L.~M. and {D'Angelo}, B. and {Danila}, B. and {Danilishin}, S. and {D'Antonio}, S. and {Danzmann}, K. and {Darsow-Fromm}, C. and {Dasgupta}, A. and {Datrier}, L.~E.~H. and {Datta}, S. and {Dattilo}, V. and {Dave}, I. and {Davier}, M. and {Davies}, G.~S. and {Davis}, D. and {Davis}, M.~C. and {Daw}, E.~J. and {Dean}, R. and {DeBra}, D. and {Deenadayalan}, M. and {Degallaix}, J. and {De Laurentis}, M. and {Del{\'e}glise}, S. and {Del Favero}, V. and {De Lillo}, F. and {De Lillo}, N. and {Del Pozzo}, W. and {DeMarchi}, L.~M. and {De Matteis}, F. and {D'Emilio}, V. and {Demos}, N. and {Dent}, T. and {Depasse}, A. and {De Pietri}, R. and {De Rosa}, R. and {De Rossi}, C. and {DeSalvo}, R. and {De Simone}, R. and {Dhurandhar}, S. and {D{\'\i}az}, M.~C. and {Diaz-Ortiz}, M. and {Didio}, N.~A. and {Dietrich}, T. and {Di Fiore}, L. and {Di Fronzo}, C. and {Di Giorgio}, C. and {Di Giovanni}, F. and {Di Giovanni}, M. and {Di Girolamo}, T. and {Di Lieto}, A. and {Ding}, B. and {Di Pace}, S. and {Di Palma}, I. and {Di Renzo}, F. and {Divakarla}, A.~K. and {Divyajyoti} and {Dmitriev}, A. and {Doctor}, Z. and {D'Onofrio}, L. and {Donovan}, F. and {Dooley}, K.~L. and {Doravari}, S. and {Dorrington}, I. and {Drago}, M. and {Driggers}, J.~C. and {Drori}, Y. and {Ducoin}, J. -G. and {Dupej}, P. and {Durante}, O. and {D'Urso}, D. and {Duverne}, P. -A. and {Dwyer}, S.~E. and {Eassa}, C. and {Easter}, P.~J. and {Ebersold}, M. and {Eckhardt}, T. and {Eddolls}, G. and {Edelman}, B. and {Edo}, T.~B. and {Edy}, O. and {Effler}, A. and {Eichholz}, J. and {Eikenberry}, S.~S. and {Eisenmann}, M. and {Eisenstein}, R.~A. and {Ejlli}, A. and {Engelby}, E. and {Errico}, L. and {Essick}, R.~C. and {Estell{\'e}s}, H. and {Estevez}, D. and {Etienne}, Z. and {Etzel}, T. and {Evans}, M. and {Evans}, T.~M. and {Ewing}, B.~E. and {Fafone}, V. and {Fair}, H. and {Fairhurst}, S. and {Fanning}, S.~P. and {Farah}, A.~M. and {Farinon}, S. and {Farr}, B. and {Farr}, W.~M. and {Farrow}, N.~W. and {Fauchon-Jones}, E.~J. and {Favaro}, G. and {Favata}, M. and {Fays}, M. and {Fazio}, M. and {Feicht}, J. and {Fejer}, M.~M. and {Fenyvesi}, E. and {Ferguson}, D.~L. and {Fernandez-Galiana}, A. and {Ferrante}, I. and {Ferreira}, T.~A. and {Fidecaro}, F. and {Figura}, P. and {Fiori}, I. and {Fishbach}, M. and {Fisher}, R.~P. and {Fittipaldi}, R. and {Fiumara}, V. and {Flaminio}, R. and {Floden}, E. and {Fong}, H. and {Font}, J.~A. and {Fornal}, B. and {Forsyth}, P.~W.~F. and {Franke}, A. and {Frasca}, S. and {Frasconi}, F. and {Frederick}, C. and {Freed}, J.~P. and {Frei}, Z. and {Freise}, A. and {Frey}, R. and {Fritschel}, P. and {Frolov}, V.~V. and {Fronz{\'e}}, G.~G. and {Fulda}, P. and {Fyffe}, M. and {Gabbard}, H.~A. and {Gabella}, W. and {Gadre}, B.~U. and {Gair}, J.~R. and {Gais}, J. and {Galaudage}, S. and {Gamba}, R. and {Ganapathy}, D. and {Ganguly}, A. and {Gaonkar}, S.~G. and {Garaventa}, B. and {Garc{\'\i}a}, F. and {Garc{\'\i}a-N{\'u}{\~n}ez}, C. and {Garc{\'\i}a-Quir{\'o}s}, C. and {Garufi}, F. and {Gateley}, B. and {Gaudio}, S. and {Gayathri}, V. and {Gemme}, G. and {Gennai}, A. and {George}, J. and {George}, R.~N. and {Gerberding}, O. and {Gergely}, L. and {Gewecke}, P. and {Ghonge}, S. and {Ghosh}, Abhirup and {Ghosh}, Archisman and {Ghosh}, Shaon and {Ghosh}, Shrobana and {Giacomazzo}, B. and {Giacoppo}, L. and {Giaime}, J.~A. and {Giardina}, K.~D. and {Gibson}, D.~R. and {Gier}, C. and {Giesler}, M. and {Giri}, P. and {Gissi}, F. and {Glanzer}, J. and {Gleckl}, A.~E. and {Godwin}, P. and {Goetz}, E. and {Goetz}, R. and {Gohlke}, N. and {Goncharov}, B. and {Gonz{\'a}lez}, G. and {Gopakumar}, A. and {Gosselin}, M. and {Gouaty}, R. and {Gould}, D.~W. and {Grace}, B. and {Grado}, A. and {Granata}, M. and {Granata}, V. and {Grant}, A. and {Gras}, S. and {Grassia}, P. and {Gray}, C. and {Gray}, R. and {Greco}, G. and {Green}, A.~C. and {Green}, R. and {Gretarsson}, A.~M. and {Gretarsson}, E.~M. and {Griffith}, D. and {Griffiths}, W. and {Griggs}, H.~L. and {Grignani}, G. and {Grimaldi}, A. and {Grimm}, S.~J. and {Grote}, H. and {Grunewald}, S. and {Gruning}, P. and {Guerra}, D. and {Guidi}, G.~M. and {Guimaraes}, A.~R. and {Guix{\'e}}, G. and {Gulati}, H.~K. and {Guo}, H. -K. and {Guo}, Y. and {Gupta}, Anchal and {Gupta}, Anuradha and {Gupta}, P. and {Gustafson}, E.~K. and {Gustafson}, R. and {Guzman}, F. and {Haegel}, L. and {Halim}, O. and {Hall}, E.~D. and {Hamilton}, E.~Z. and {Hammond}, G. and {Haney}, M. and {Hanks}, J. and {Hanna}, C. and {Hannam}, M.~D. and {Hannuksela}, O. and {Hansen}, H. and {Hansen}, T.~J. and {Hanson}, J. and {Harder}, T. and {Hardwick}, T. and {Haris}, K. and {Harms}, J. and {Harry}, G.~M. and {Harry}, I.~W. and {Hartwig}, D. and {Haskell}, B. and {Hasskew}, R.~K. and {Haster}, C. -J. and {Haughian}, K. and {Hayes}, F.~J. and {Healy}, J. and {Heidmann}, A. and {Heidt}, A. and {Heintze}, M.~C. and {Heinze}, J. and {Heinzel}, J. and {Heitmann}, H. and {Hellman}, F. and {Hello}, P. and {Helmling-Cornell}, A.~F. and {Hemming}, G. and {Hendry}, M. and {Heng}, I.~S. and {Hennes}, E. and {Hennig}, J. and {Hennig}, M.~H. and {Hernandez}, A.~G. and {Hernandez Vivanco}, F. and {Heurs}, M. and {Hild}, S. and {Hill}, P. and {Hines}, A.~S. and {Hochheim}, S. and {Hofman}, D. and {Hohmann}, J.~N. and {Holcomb}, D.~G. and {Holland}, N.~A. and {Holley-Bockelmann}, K. and {Hollows}, I.~J. and {Holmes}, Z.~J. and {Holt}, K. and {Holz}, D.~E. and {Hopkins}, P. and {Hough}, J. and {Hourihane}, S. and {Howell}, E.~J. and {Hoy}, C.~G. and {Hoyland}, D. and {Hreibi}, A. and {Hsu}, Y. and {Huang}, Y. and {H{\"u}bner}, M.~T. and {Huddart}, A.~D. and {Hughey}, B. and {Hui}, V. and {Husa}, S. and {Huttner}, S.~H. and {Huxford}, R. and {Huynh-Dinh}, T. and {Idzkowski}, B. and {Iess}, A. and {Ingram}, C. and {Isi}, M. and {Isleif}, K. and {Iyer}, B.~R. and {JaberianHamedan}, V. and {Jacqmin}, T. and {Jadhav}, S.~J. and {Jadhav}, S.~P. and {James}, A.~L. and {Jan}, A.~Z. and {Jani}, K. and {Janquart}, J. and {Janssens}, K. and {Janthalur}, N.~N. and {Jaranowski}, P. and {Jariwala}, D. and {Jaume}, R. and {Jenkins}, A.~C. and {Jenner}, K. and {Jeunon}, M. and {Jia}, W. and {Johns}, G.~R. and {Johnson-McDaniel}, N.~K. and {Jones}, A.~W. and {Jones}, D.~I. and {Jones}, J.~D. and {Jones}, P. and {Jones}, R. and {Jonker}, R.~J.~G. and {Ju}, L. and {Junker}, J. and {Juste}, V. and {Kalaghatgi}, C.~V. and {Kalogera}, V. and {Kamai}, B. and {Kandhasamy}, S. and {Kang}, G. and {Kanner}, J.~B. and {Kao}, Y. and {Kapadia}, S.~J. and {Kapasi}, D.~P. and {Karat}, S. and {Karathanasis}, C. and {Karki}, S. and {Kashyap}, R. and {Kasprzack}, M. and {Kastaun}, W. and {Katsanevas}, S. and {Katsavounidis}, E. and {Katzman}, W. and {Kaur}, T. and {Kawabe}, K. and {K{\'e}f{\'e}lian}, F. and {Keitel}, D. and {Key}, J.~S. and {Khadka}, S. and {Khalili}, F.~Y. and {Khan}, S. and {Khazanov}, E.~A. and {Khetan}, N. and {Khursheed}, M. and {Kijbunchoo}, N. and {Kim}, C. and {Kim}, J.~C. and {Kim}, K. and {Kim}, W.~S. and {Kim}, Y. -M. and {Kimball}, C. and {Kinley-Hanlon}, M. and {Kirchhoff}, R. and {Kissel}, J.~S. and {Kleybolte}, L. and {Klimenko}, S. and {Knee}, A.~M. and {Knowles}, T.~D. and {Knyazev}, E. and {Koch}, P. and {Koekoek}, G. and {Koley}, S. and {Kolitsidou}, P. and {Kolstein}, M. and {Komori}, K. and {Kondrashov}, V. and {Kontos}, A. and {Koper}, N. and {Korobko}, M. and {Kovalam}, M. and {Kozak}, D.~B. and {Kringel}, V. and {Krishnendu}, N.~V. and {Kr{\'o}lak}, A. and {Kuehn}, G. and {Kuei}, F. and {Kuijer}, P. and {Kulkarni}, S. and {Kumar}, A. and {Kumar}, P. and {Kumar}, Rahul and {Kumar}, Rakesh and {Kuns}, K. and {Kuwahara}, S. and {Lagabbe}, P. and {Laghi}, D. and {Lalande}, E. and {Lam}, T.~L. and {Lamberts}, A. and {Landry}, M. and {Lane}, B.~B. and {Lang}, R.~N. and {Lange}, J. and {Lantz}, B. and {La Rosa}, I. and {Lartaux-Vollard}, A. and {Lasky}, P.~D. and {Laxen}, M. and {Lazzarini}, A. and {Lazzaro}, C. and {Leaci}, P. and {Leavey}, S. and {Lecoeuche}, Y.~K. and {Lee}, H.~M. and {Lee}, H.~W. and {Lee}, J. and {Lee}, K. and {Lehmann}, J. and {Lema{\^\i}tre}, A. and {Leroy}, N. and {Letendre}, N. and {Levesque}, C. and {Levin}, Y. and {Leviton}, J.~N. and {Leyde}, K. and {Li}, A.~K.~Y. and {Li}, B. and {Li}, J. and {Li}, T.~G.~F. and {Li}, X. and {Linde}, F. and {Linker}, S.~D. and {Linley}, J.~N. and {Littenberg}, T.~B. and {Liu}, J. and {Liu}, K. and {Liu}, X. and {Llamas}, F. and {Llorens-Monteagudo}, M. and {Lo}, R.~K.~L. and {Lockwood}, A. and {London}, L.~T. and {Longo}, A. and {Lopez}, D. and {Lopez Portilla}, M. and {Lorenzini}, M. and {Loriette}, V. and {Lormand}, M. and {Losurdo}, G. and {Lott}, T.~P. and {Lough}, J.~D. and {Lousto}, C.~O. and {Lovelace}, G. and {Lucaccioni}, J.~F. and {L{\"u}ck}, H. and {Lumaca}, D. and {Lundgren}, A.~P. and {Lynam}, J.~E. and {Macas}, R. and {MacInnis}, M. and {Macleod}, D.~M. and {MacMillan}, I.~A.~O. and {Macquet}, A. and {Hernandez}, I. Maga{\~n}a and {Magazz{\`u}}, C. and {Magee}, R.~M. and {Maggiore}, R. and {Magnozzi}, M. and {Mahesh}, S. and {Majorana}, E. and {Makarem}, C. and {Maksimovic}, I. and {Maliakal}, S. and {Malik}, A. and {Man}, N. and {Mandic}, V. and {Mangano}, V. and {Mango}, J.~L. and {Mansell}, G.~L. and {Manske}, M. and {Mantovani}, M. and {Mapelli}, M. and {Marchesoni}, F. and {Marion}, F. and {Mark}, Z. and {M{\'a}rka}, S. and {M{\'a}rka}, Z. and {Markakis}, C. and {Markosyan}, A.~S. and {Markowitz}, A. and {Maros}, E. and {Marquina}, A. and {Marsat}, S. and {Martelli}, F. and {Martin}, I.~W. and {Martin}, R.~M. and {Martinez}, M. and {Martinez}, V.~A. and {Martinez}, V. and {Martinovic}, K. and {Martynov}, D.~V. and {Marx}, E.~J. and {Masalehdan}, H. and {Mason}, K. and {Massera}, E. and {Masserot}, A. and {Massinger}, T.~J. and {Masso-Reid}, M. and {Mastrogiovanni}, S. and {Matas}, A. and {Mateu-Lucena}, M. and {Matichard}, F. and {Matiushechkina}, M. and {Mavalvala}, N. and {McCann}, J.~J. and {McCarthy}, R. and {McClelland}, D.~E. and {McClincy}, P.~K. and {McCormick}, S. and {McCuller}, L. and {McGhee}, G.~I. and {McGuire}, S.~C. and {McIsaac}, C. and {McIver}, J. and {McRae}, T. and {McWilliams}, S.~T. and {Meacher}, D. and {Mehmet}, M. and {Mehta}, A.~K. and {Meijer}, Q. and {Melatos}, A. and {Melchor}, D.~A. and {Mendell}, G. and {Menendez-Vazquez}, A. and {Menoni}, C.~S. and {Mercer}, R.~A. and {Mereni}, L. and {Merfeld}, K. and {Merilh}, E.~L. and {Merritt}, J.~D. and {Merzougui}, M. and {Meshkov}, S. and {Messenger}, C. and {Messick}, C. and {Meyers}, P.~M. and {Meylahn}, F. and {Mhaske}, A. and {Miani}, A. and {Miao}, H. and {Michaloliakos}, I. and {Michel}, C. and {Middleton}, H. and {Milano}, L. and {Miller}, A. and {Miller}, A.~L. and {Miller}, B. and {Millhouse}, M. and {Mills}, J.~C. and {Milotti}, E. and {Minazzoli}, O. and {Minenkov}, Y. and {Mir}, Ll. M. and {Miravet-Ten{\'e}s}, M. and {Mishra}, C. and {Mishra}, T. and {Mistry}, T. and {Mitra}, S. and {Mitrofanov}, V.~P. and {Mitselmakher}, G. and {Mittleman}, R. and {Mo}, Geoffrey and {Moguel}, E. and {Mogushi}, K. and {Mohapatra}, S.~R.~P. and {Mohite}, S.~R. and {Molina}, I. and {Molina-Ruiz}, M. and {Mondin}, M. and {Montani}, M. and {Moore}, C.~J. and {Moraru}, D. and {Morawski}, F. and {More}, A. and {Moreno}, C. and {Moreno}, G. and {Morisaki}, S. and {Mours}, B. and {Mow-Lowry}, C.~M. and {Mozzon}, S. and {Muciaccia}, F. and {Mukherjee}, Arunava and {Mukherjee}, D. and {Mukherjee}, Soma and {Mukherjee}, Subroto and {Mukherjee}, Suvodip and {Mukund}, N. and {Mullavey}, A. and {Munch}, J. and {Mu{\~n}iz}, E.~A. and {Murray}, P.~G. and {Musenich}, R. and {Muusse}, S. and {Nadji}, S.~L. and {Nagar}, A. and {Napolano}, V. and {Nardecchia}, I. and {Naticchioni}, L. and {Nayak}, B. and {Nayak}, R.~K. and {Neil}, B.~F. and {Neilson}, J. and {Nelemans}, G. and {Nelson}, T.~J.~N. and {Nery}, M. and {Neubauer}, P. and {Neunzert}, A. and {Ng}, K.~Y. and {Ng}, S.~W.~S. and {Nguyen}, C. and {Nguyen}, P. and {Nguyen}, T. and {Nichols}, S.~A. and {Nissanke}, S. and {Nitoglia}, E. and {Nocera}, F. and {Norman}, M. and {North}, C. and {Nuttall}, L.~K. and {Oberling}, J. and {O'Brien}, B.~D. and {O'Dell}, J. and {Oelker}, E. and {Oganesyan}, G. and {Oh}, J.~J. and {Oh}, S.~H. and {Ohme}, F. and {Ohta}, H. and {Okada}, M.~A. and {Olivetto}, C. and {Oram}, R. and {O'Reilly}, B. and {Ormiston}, R.~G. and {Ormsby}, N.~D. and {Ortega}, L.~F. and {O'Shaughnessy}, R. and {O'Shea}, E. and {Ossokine}, S. and {Osthelder}, C. and {Ottaway}, D.~J. and {Overmier}, H. and {Pace}, A.~E. and {Pagano}, G. and {Page}, M.~A. and {Pagliaroli}, G. and {Pai}, A. and {Pai}, S.~A. and {Palamos}, J.~R. and {Palashov}, O. and {Palomba}, C. and {Pan}, H. and {Panda}, P.~K. and {Pang}, P.~T.~H. and {Pankow}, C. and {Pannarale}, F. and {Pant}, B.~C. and {Panther}, F.~H. and {Paoletti}, F. and {Paoli}, A. and {Paolone}, A. and {Park}, H. and {Parker}, W. and {Pascucci}, D. and {Pasqualetti}, A. and {Passaquieti}, R. and {Passuello}, D. and {Patel}, M. and {Pathak}, M. and {Patricelli}, B. and {Patron}, A.~S. and {Patrone}, S. and {Paul}, S. and {Payne}, E. and {Pedraza}, M. and {Pegoraro}, M. and {Pele}, A. and {Penn}, S. and {Perego}, A. and {Pereira}, A. and {Pereira}, T. and {Perez}, C.~J. and {P{\'e}rigois}, C. and {Perkins}, C.~C. and {Perreca}, A. and {Perri{\`e}s}, S. and {Petermann}, J. and {Petterson}, D. and {Pfeiffer}, H.~P. and {Pham}, K.~A. and {Phukon}, K.~S. and {Piccinni}, O.~J. and {Pichot}, M. and {Piendibene}, M. and {Piergiovanni}, F. and {Pierini}, L. and {Pierro}, V. and {Pillant}, G. and {Pillas}, M. and {Pilo}, F. and {Pinard}, L. and {Pinto}, I.~M. and {Pinto}, M. and {Piotrzkowski}, K. and {Pirello}, M. and {Pitkin}, M.~D. and {Placidi}, E. and {Planas}, L. and {Plastino}, W. and {Pluchar}, C. and {Poggiani}, R. and {Polini}, E. and {Pong}, D.~Y.~T. and {Ponrathnam}, S. and {Popolizio}, P. and {Porter}, E.~K. and {Poulton}, R. and {Powell}, J. and {Pracchia}, M. and {Pradier}, T. and {Prajapati}, A.~K. and {Prasai}, K. and {Prasanna}, R. and {Pratten}, G. and {Principe}, M. and {Prodi}, G.~A. and {Prokhorov}, L. and {Prosposito}, P. and {Prudenzi}, L. and {Puecher}, A. and {Punturo}, M. and {Puosi}, F. and {Puppo}, P. and {P{\"u}rrer}, M. and {Qi}, H. and {Quetschke}, V. and {Quitzow-James}, R. and {Raab}, F.~J. and {Raaijmakers}, G. and {Radkins}, H. and {Radulesco}, N. and {Raffai}, P. and {Rail}, S.~X. and {Raja}, S. and {Rajan}, C. and {Ramirez}, K.~E. and {Ramirez}, T.~D. and {Ramos-Buades}, A. and {Rana}, J. and {Rapagnani}, P. and {Rapol}, U.~D. and {Ray}, A. and {Raymond}, V. and {Raza}, N. and {Razzano}, M. and {Read}, J. and {Rees}, L.~A. and {Regimbau}, T. and {Rei}, L. and {Reid}, S. and {Reid}, S.~W. and {Reitze}, D.~H. and {Relton}, P. and {Renzini}, A. and {Rettegno}, P. and {Reza}, A. and {Rezac}, M. and {Ricci}, F. and {Richards}, D. and {Richardson}, J.~W. and {Richardson}, L. and {Riemenschneider}, G. and {Riles}, K. and {Rinaldi}, S. and {Rink}, K. and {Rizzo}, M. and {Robertson}, N.~A. and {Robie}, R. and {Robinet}, F. and {Rocchi}, A. and {Rodriguez}, S. and {Rolland}, L. and {Rollins}, J.~G. and {Romanelli}, M. and {Romano}, R. and {Romel}, C.~L. and {Romero-Rodr{\'\i}guez}, A. and {Romero-Shaw}, I.~M. and {Romie}, J.~H. and {Ronchini}, S. and {Rosa}, L. and {Rose}, C.~A. and {Rosell}, M.~J.~B. and {Rosi{\'n}ska}, D. and {Ross}, M.~P. and {Rowan}, S. and {Rowlinson}, S.~J. and {Roy}, S. and {Roy}, Santosh and {Roy}, Soumen and {Rozza}, D. and {Ruggi}, P. and {Ruiz-Rocha}, K. and {Ryan}, K. and {Sachdev}, S. and {Sadecki}, T. and {Sadiq}, J. and {Sakellariadou}, M. and {Salafia}, O.~S. and {Salconi}, L. and {Saleem}, M. and {Salemi}, F. and {Samajdar}, A. and {Sanchez}, E.~J. and {Sanchez}, J.~H. and {Sanchez}, L.~E. and {Sanchis-Gual}, N. and {Sanders}, J.~R. and {Sanuy}, A. and {Saravanan}, T.~R. and {Sarin}, N. and {Sassolas}, B. and {Satari}, H. and {Sauter}, O. and {Savage}, R.~L. and {Sawant}, D. and {Sawant}, H.~L. and {Sayah}, S. and {Schaetzl}, D. and {Scheel}, M. and {Scheuer}, J. and {Schiworski}, M. and {Schmidt}, P. and {Schmidt}, S. and {Schnabel}, R. and {Schneewind}, M. and {Schofield}, R.~M.~S. and {Sch{\"o}nbeck}, A. and {Schulte}, B.~W. and {Schutz}, B.~F. and {Schwartz}, E. and {Scott}, J. and {Scott}, S.~M. and {Seglar-Arroyo}, M. and {Sellers}, D. and {Sengupta}, A.~S. and {Sentenac}, D. and {Seo}, E.~G. and {Sequino}, V. and {Sergeev}, A. and {Setyawati}, Y. and {Shaffer}, T. and {Shahriar}, M.~S. and {Shams}, B. and {Sharma}, A. and {Sharma}, P. and {Shawhan}, P. and {Shcheblanov}, N.~S. and {Shikauchi}, M. and {Shoemaker}, D.~H. and {Shoemaker}, D.~M. and {ShyamSundar}, S. and {Sieniawska}, M. and {Sigg}, D. and {Singer}, L.~P. and {Singh}, D. and {Singh}, N. and {Singha}, A. and {Sintes}, A.~M. and {Sipala}, V. and {Skliris}, V. and {Slagmolen}, B.~J.~J. and {Slaven-Blair}, T.~J. and {Smetana}, J. and {Smith}, J.~R. and {Smith}, R.~J.~E. and {Soldateschi}, J. and {Somala}, S.~N. and {Son}, E.~J. and {Soni}, K. and {Soni}, S. and {Sordini}, V. and {Sorrentino}, F. and {Sorrentino}, N. and {Soulard}, R. and {Souradeep}, T. and {Sowell}, E. and {Spagnuolo}, V. and {Spencer}, A.~P. and {Spera}, M. and {Srinivasan}, R. and {Srivastava}, A.~K. and {Srivastava}, V. and {Staats}, K. and {Stachie}, C. and {Steer}, D.~A. and {Steinhoff}, J. and {Steinlechner}, J. and {Steinlechner}, S. and {Stevenson}, S. and {Stops}, D.~J. and {Stover}, M. and {Strain}, K.~A. and {Strang}, L.~C. and {Stratta}, G. and {Strunk}, A. and {Sturani}, R. and {Stuver}, A.~L. and {Sudhagar}, S. and {Sudhir}, V. and {Suh}, H.~G. and {Summerscales}, T.~Z. and {Sun}, H. and {Sun}, L. and {Sunil}, S. and {Sur}, A. and {Suresh}, J. and {Sutton}, P.~J. and {Swinkels}, B.~L. and {Szczepa{\'n}czyk}, M.~J. and {Szewczyk}, P. and {Tacca}, M. and {Tait}, S.~C. and {Talbot}, C.~J. and {Talbot}, C. and {Tanasijczuk}, A.~J. and {Tanner}, D.~B. and {Tao}, D. and {Tao}, L. and {Mart{\'\i}n}, E.~N. Tapia San and {Taranto}, C. and {Tasson}, J.~D. and {Tenorio}, R. and {Terhune}, J.~E. and {Terkowski}, L. and {Thirugnanasambandam}, M.~P. and {Thomas}, L. and {Thomas}, M. and {Thomas}, P. and {Thompson}, J.~E. and {Thondapu}, S.~R. and {Thorne}, K.~A. and {Thrane}, E. and {Tiwari}, Shubhanshu and {Tiwari}, Srishti and {Tiwari}, V. and {Toivonen}, A.~M. and {Toland}, K. and {Tolley}, A.~E. and {Tonelli}, M. and {Torres-Forn{\'e}}, A. and {Torrie}, C.~I. and {e Melo}, I. Tosta and {T{\"o}yr{\"a}}, D. and {Trapananti}, A. and {Travasso}, F. and {Traylor}, G. and {Trevor}, M. and {Tringali}, M.~C. and {Tripathee}, A. and {Troiano}, L. and {Trovato}, A. and {Trozzo}, L. and {Trudeau}, R.~J. and {Tsai}, D.~S. and {Tsai}, D. and {Tsang}, K.~W. and {Tse}, M. and {Tso}, R. and {Tsukada}, L. and {Tsuna}, D. and {Tsutsui}, T. and {Turbang}, K. and {Turconi}, M. and {Ubhi}, A.~S. and {Udall}, R.~P. and {Ueno}, K. and {Unnikrishnan}, C.~S. and {Urban}, A.~L. and {Utina}, A. and {Vahlbruch}, H. and {Vajente}, G. and {Vajpeyi}, A. and {Valdes}, G. and {Valentini}, M. and {Valsan}, V. and {van Bakel}, N. and {van Beuzekom}, M. and {van den Brand}, J.~F.~J. and {Van Den Broeck}, C. and {Vander-Hyde}, D.~C. and {van der Schaaf}, L. and {van Heijningen}, J.~V. and {Vanosky}, J. and {van Remortel}, N. and {Vardaro}, M. and {Vargas}, A.~F. and {Varma}, V. and {Vas{\'u}th}, M. and {Vecchio}, A. and {Vedovato}, G. and {Veitch}, J. and {Veitch}, P.~J. and {Venneberg}, J. and {Venugopalan}, G. and {Verkindt}, D. and {Verma}, P. and {Verma}, Y. and {Veske}, D. and {Vetrano}, F. and {Vicer{\'e}}, A. and {Vidyant}, S. and {Viets}, A.~D. and {Vijaykumar}, A. and {Villa-Ortega}, V. and {Vinet}, J. -Y. and {Virtuoso}, A. and {Vitale}, S. and {Vo}, T. and {Vocca}, H. and {von Reis}, E.~R.~G. and {von Wrangel}, J.~S.~A. and {Vorvick}, C. and {Vyatchanin}, S.~P. and {Wade}, L.~E. and {Wade}, M. and {Wagner}, K.~J. and {Walet}, R.~C. and {Walker}, M. and {Wallace}, G.~S. and {Wallace}, L. and {Walsh}, S. and {Wang}, J.~Z. and {Wang}, W.~H. and {Ward}, R.~L. and {Warner}, J. and {Was}, M. and {Washington}, N.~Y. and {Watchi}, J. and {Weaver}, B. and {Webster}, S.~A. and {Weinert}, M. and {Weinstein}, A.~J. and {Weiss}, R. and {Weller}, C.~M. and {Weller}, R. and {Wellmann}, F. and {Wen}, L. and {We{\ss}els}, P. and {Wette}, K. and {Whelan}, J.~T. and {White}, D.~D. and {Whiting}, B.~F. and {Whittle}, C. and {Wilken}, D. and {Williams}, D. and {Williams}, M.~J. and {Williamson}, A.~R. and {Willis}, J.~L. and {Willke}, B. and {Wilson}, D.~J. and {Winkler}, W. and {Wipf}, C.~C. and {Wlodarczyk}, T. and {Woan}, G. and {Woehler}, J. and {Wofford}, J.~K. and {Wong}, I.~C.~F. and {Wu}, D.~S. and {Wysocki}, D.~M. and {Xiao}, L. and {Yamamoto}, H. and {Yang}, F.~W. and {Yang}, L. and {Yang}, Yang and {Yang}, Z. and {Yap}, M.~J. and {Yeeles}, D.~W. and {Yelikar}, A.~B. and {Ying}, M. and {Yoo}, J. and {Yu}, Hang and {Yu}, Haocun and {Zadro{\.z}ny}, A. and {Zanolin}, M. and {Zelenova}, T. and {Zendri}, J. -P. and {Zevin}, M. and {Zhang}, J. and {Zhang}, L. and {Zhang}, T. and {Zhang}, Y. and {Zhao}, C. and {Zhao}, G. and {Zhao}, Yue and {Zhou}, R. and {Zhou}, Z. and {Zhu}, X.~J. and {Zimmerman}, A.~B. and {Zlochower}, Y. and {Zucker}, M.~E. and {Zweizig}, J. and {The LIGO Scientific Collaboration} and {the Virgo Collaboration}},
        title = "{GWTC-2.1: Deep extended catalog of compact binary coalescences observed by LIGO and Virgo during the first half of the third observing run}",
      journal = {\prd},
     keywords = {Experiments in gravity, cosmology, cosmic rays, General Relativity and Quantum Cosmology},
         year = 2024,
        month = jan,
       volume = {109},
       number = {2},
          eid = {022001},
        pages = {022001},
          doi = {10.1103/PhysRevD.109.022001},
archivePrefix = {arXiv},
       eprint = {2108.01045},
 primaryClass = {gr-qc},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024PhRvD.109b2001A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{abbottGWTC3,
       author = {{Abbott}, R. and {Abbott}, T.~D. and {Acernese}, F. and {Ackley}, K. and {Adams}, C. and {Adhikari}, N. and {Adhikari}, R.~X. and {Adya}, V.~B. and {Affeldt}, C. and {Agarwal}, D. and {Agathos}, M. and {Agatsuma}, K. and {Aggarwal}, N. and {Aguiar}, O.~D. and {Aiello}, L. and {Ain}, A. and {Ajith}, P. and {Akcay}, S. and {Akutsu}, T. and {Albanesi}, S. and {Allocca}, A. and {Altin}, P.~A. and {Amato}, A. and {Anand}, C. and {Anand}, S. and {Ananyeva}, A. and {Anderson}, S.~B. and {Anderson}, W.~G. and {Ando}, M. and {Andrade}, T. and {Andres}, N. and {Andri{\'c}}, T. and {Angelova}, S.~V. and {Ansoldi}, S. and {Antelis}, J.~M. and {Antier}, S. and {Appert}, S. and {Arai}, Koji and {Arai}, Koya and {Arai}, Y. and {Araki}, S. and {Araya}, A. and {Araya}, M.~C. and {Areeda}, J.~S. and {Ar{\`e}ne}, M. and {Aritomi}, N. and {Arnaud}, N. and {Zevin}, M. and {Zhan}, M. and {Zhang}, H. and {Zhang}, J. and {Zhang}, L. and {Zhang}, T. and {Zhang}, Y. and {Zhao}, C. and {Zhao}, G. and {Zhao}, Y. and {Zhao}, Yue and {Zheng}, Y. and {Zhou}, R. and {Zhou}, Z. and {Zhu}, X.~J. and {Zhu}, Z. -H. and {Zimmerman}, A.~B. and {Zlochower}, Y. and {Zucker}, M.~E. and {Zweizig}, J. and {Ligo Scientific Collaboration},, VIRGO Collaboration and {Kagra Collaboration}},
        title = "{GWTC-3: Compact Binary Coalescences Observed by LIGO and Virgo during the Second Part of the Third Observing Run}",
      journal = {Physical Review X},
     keywords = {General Relativity and Quantum Cosmology, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2023,
        month = oct,
       volume = {13},
       number = {4},
          eid = {041039},
        pages = {041039},
          doi = {10.1103/PhysRevX.13.041039},
archivePrefix = {arXiv},
       eprint = {2111.03606},
 primaryClass = {gr-qc},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023PhRvX..13d1039A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Hosokawa2016,
       author = {{Hosokawa}, Takashi and {Hirano}, Shingo and {Kuiper}, Rolf and {Yorke}, Harold W. and {Omukai}, Kazuyuki and {Yoshida}, Naoki},
        title = "{Formation of Massive Primordial Stars: Intermittent UV Feedback with Episodic Mass Accretion}",
      journal = {\apj},
     keywords = {accretion, accretion disks, cosmology: theory, early universe, galaxies: formation, stars: formation, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = jun,
       volume = {824},
       number = {2},
          eid = {119},
        pages = {119},
          doi = {10.3847/0004-637X/824/2/119},
archivePrefix = {arXiv},
       eprint = {1510.01407},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...824..119H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hirano2014,
       author = {{Hirano}, Shingo and {Hosokawa}, Takashi and {Yoshida}, Naoki and {Umeda}, Hideyuki and {Omukai}, Kazuyuki and {Chiaki}, Gen and {Yorke}, Harold W.},
        title = "{One Hundred First Stars: Protostellar Evolution and the Final Masses}",
      journal = {\apj},
     keywords = {accretion, accretion disks, early universe, stars: evolution, stars: formation, stars: population III, stars: pre-main sequence, Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - Galaxy Astrophysics},
         year = 2014,
        month = feb,
       volume = {781},
       number = {2},
          eid = {60},
        pages = {60},
          doi = {10.1088/0004-637X/781/2/60},
archivePrefix = {arXiv},
       eprint = {1308.4456},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...781...60H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chon2021,
       author = {{Chon}, Sunmyon and {Omukai}, Kazuyuki and {Schneider}, Raffaella},
        title = "{Transition of the initial mass function in the metal-poor environments}",
      journal = {\mnras},
     keywords = {binaries: general, stars: formation, stars: Population II, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = dec,
       volume = {508},
       number = {3},
        pages = {4175-4192},
          doi = {10.1093/mnras/stab2497},
archivePrefix = {arXiv},
       eprint = {2103.04997},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.508.4175C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ekstrom2008,
       author = {{Ekstr{\"o}m}, S. and {Meynet}, G. and {Chiappini}, C. and {Hirschi}, R. and {Maeder}, A.},
        title = "{Effects of rotation on the evolution of primordial stars}",
      journal = {\aap},
     keywords = {stars: evolution, stars: rotation, stars: chemically peculiar, stars:, supernovae: general, Astrophysics},
         year = 2008,
        month = oct,
       volume = {489},
       number = {2},
        pages = {685-698},
          doi = {10.1051/0004-6361:200809633},
archivePrefix = {arXiv},
       eprint = {0807.0573},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...489..685E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Murphy2021,
       author = {{Murphy}, Laura J. and {Groh}, Jose H. and {Ekstr{\"o}m}, Sylvia and {Meynet}, Georges and {Pezzotti}, Camila and {Georgy}, Cyril and {Choplin}, Arthur and {Eggenberger}, Patrick and {Farrell}, Eoin and {Haemmerl{\'e}}, Lionel and {Hirschi}, Raphael and {Maeder}, Andr{\'e} and {Martinet}, S{\'e}bastien},
        title = "{Grids of stellar models with rotation - V. Models from 1.7 to 120 M$_{{\ensuremath{\odot}}}$ at zero metallicity}",
      journal = {\mnras},
     keywords = {stars: evolution, stars: massive, stars: Population III, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = feb,
       volume = {501},
       number = {2},
        pages = {2745-2763},
          doi = {10.1093/mnras/staa3803},
archivePrefix = {arXiv},
       eprint = {2012.07420},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.501.2745M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Park2023,
       author = {{Park}, Jongwon and {Ricotti}, Massimo and {Sugimura}, Kazuyuki},
        title = "{Population III star formation in an X-ray background: III. Periodic radiative feedback and luminosity induced by elliptical orbits}",
      journal = {\mnras},
     keywords = {gravitational waves, binaries: general, stars: formation, stars: Population III, dark ages, reionization, first stars, X-rays: diffuse background, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2023,
        month = jun,
       volume = {521},
       number = {4},
        pages = {5334-5353},
          doi = {10.1093/mnras/stad895},
archivePrefix = {arXiv},
       eprint = {2212.04564},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023MNRAS.521.5334P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Prole2022,
       author = {{Prole}, Lewis R. and {Clark}, Paul C. and {Klessen}, Ralf S. and {Glover}, Simon C.~O.},
        title = "{Fragmentation-induced starvation in Population III star formation: a resolution study}",
      journal = {\mnras},
     keywords = {hydrodynamics, stars: formation, stars: luminosity function, mass function, stars: Population III, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = mar,
       volume = {510},
       number = {3},
        pages = {4019-4030},
          doi = {10.1093/mnras/stab3697},
archivePrefix = {arXiv},
       eprint = {2112.10800},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.510.4019P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stacy2016,
       author = {{Stacy}, Athena and {Bromm}, Volker and {Lee}, Aaron T.},
        title = "{Building up the Population III initial mass function from cosmological initial conditions}",
      journal = {\mnras},
     keywords = {stars: formation, stars: Population III, galaxies: formation, cosmology: theory, early Universe, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = oct,
       volume = {462},
       number = {2},
        pages = {1307-1328},
          doi = {10.1093/mnras/stw1728},
archivePrefix = {arXiv},
       eprint = {1603.09475},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.462.1307S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Smith2015,
       author = {{Smith}, Britton D. and {Wise}, John H. and {O'Shea}, Brian W. and {Norman}, Michael L. and {Khochfar}, Sadegh},
        title = "{The first Population II stars formed in externally enriched mini-haloes}",
      journal = {\mnras},
     keywords = {hydrodynamics, radiative transfer, methods: numerical, galaxies: star formation, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = sep,
       volume = {452},
       number = {3},
        pages = {2822-2836},
          doi = {10.1093/mnras/stv1509},
archivePrefix = {arXiv},
       eprint = {1504.07639},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.452.2822S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marchant2019,
       author = {{Marchant}, Pablo and {Renzo}, Mathieu and {Farmer}, Robert and {Pappas}, Kaliroe M.~W. and {Taam}, Ronald E. and {de Mink}, Selma E. and {Kalogera}, Vassiliki},
        title = "{Pulsational Pair-instability Supernovae in Very Close Binaries}",
      journal = {\apj},
     keywords = {binaries: close, stars: black holes, stars: massive, supernovae: general, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = sep,
       volume = {882},
       number = {1},
          eid = {36},
        pages = {36},
          doi = {10.3847/1538-4357/ab3426},
archivePrefix = {arXiv},
       eprint = {1810.13412},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...882...36M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vink2000,
       author = {{Vink}, J.~S. and {de Koter}, A. and {Lamers}, H.~J.~G.~L.~M.},
        title = "{New theoretical mass-loss rates of O and B stars}",
      journal = {\aap},
     keywords = {STARS: EARLY-TYPE, STARS: MASS-LOSS, STARS: SUPERGIANTS, STARS: WINDS, OUTFLOWS, STARS: EVOLUTION, Astrophysics},
         year = 2000,
        month = oct,
       volume = {362},
        pages = {295-309},
          doi = {10.48550/arXiv.astro-ph/0008183},
archivePrefix = {arXiv},
       eprint = {astro-ph/0008183},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&A...362..295V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reimers1975,
       author = {{Reimers}, D.},
        title = "{Circumstellar absorption lines and mass loss from red giants.}",
      journal = {Memoires of the Societe Royale des Sciences de Liege},
     keywords = {Absorption Spectra, Giant Stars, Line Spectra, M Stars, Stellar Envelopes, Stellar Mass Ejection, Doppler Effect, Ionization, K Lines, Spectral Line Width, Stellar Evolution, Stellar Spectra, Velocity Distribution, Astrophysics},
         year = 1975,
        month = jan,
       volume = {8},
        pages = {369-382},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1975MSRSL...8..369R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cranmer2011,
       author = {{Cranmer}, Steven R. and {Saar}, Steven H.},
        title = "{Testing a Predictive Theoretical Model for the Mass Loss Rates of Cool Stars}",
      journal = {\apj},
     keywords = {stars: coronae, stars: late-type, stars: magnetic field, stars: mass-loss, stars: winds, outflows, turbulence, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = nov,
       volume = {741},
       number = {1},
          eid = {54},
        pages = {54},
          doi = {10.1088/0004-637X/741/1/54},
archivePrefix = {arXiv},
       eprint = {1108.4369},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...741...54C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bloecker1995,
       author = {{Bloecker}, T.},
        title = "{Stellar evolution of low and intermediate-mass stars. I. Mass loss on the AGB and its consequences for stellar evolution.}",
      journal = {\aap},
     keywords = {STARS: EVOLUTION, STARS: MASS LOSS, STARS: AGB, POST-AGB},
         year = 1995,
        month = may,
       volume = {297},
        pages = {727},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995A&A...297..727B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bladh2019,
       author = {{Bladh}, S. and {Eriksson}, K. and {Marigo}, P. and {Liljegren}, S. and {Aringer}, B.},
        title = "{Carbon star wind models at solar and sub-solar metallicities: a comparative study. I. Mass loss and the properties of dust-driven winds}",
      journal = {\aap},
     keywords = {stars: AGB and post-AGB, stars: atmospheres, stars: carbon, stars: mass-loss, stars: evolution, stars: winds, outflows, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = mar,
       volume = {623},
          eid = {A119},
        pages = {A119},
          doi = {10.1051/0004-6361/201834778},
archivePrefix = {arXiv},
       eprint = {1902.05352},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...623A.119B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mattsson2010,
       author = {{Mattsson}, L. and {Wahlin}, R. and {H{\"o}fner}, S.},
        title = "{Dust driven mass loss from carbon stars as a function of stellar parameters . I. A grid of solar-metallicity wind models}",
      journal = {\aap},
     keywords = {stars: AGB and post-AGB, stars: atmospheres, stars: carbon, circumstellar matter, stars: evolution, stars: mass-loss, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = jan,
       volume = {509},
          eid = {A14},
        pages = {A14},
          doi = {10.1051/0004-6361/200912084},
archivePrefix = {arXiv},
       eprint = {0909.1513},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...509A..14M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eriksson2014,
       author = {{Eriksson}, K. and {Nowotny}, W. and {H{\"o}fner}, S. and {Aringer}, B. and {Wachter}, A.},
        title = "{Synthetic photometry for carbon-rich giants. IV. An extensive grid of dynamic atmosphere and wind models}",
      journal = {\aap},
     keywords = {stars: AGB and post-AGB, stars: atmospheres, stars: carbon, stars: variables: general, stars: mass-loss, circumstellar matter, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = jun,
       volume = {566},
          eid = {A95},
        pages = {A95},
          doi = {10.1051/0004-6361/201323241},
archivePrefix = {arXiv},
       eprint = {1404.7515},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...566A..95E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Marigo2020,
       author = {{Marigo}, Paola and {Cummings}, Jeffrey D. and {Curtis}, Jason Lee and {Kalirai}, Jason and {Chen}, Yang and {Tremblay}, Pier-Emmanuel and {Ramirez-Ruiz}, Enrico and {Bergeron}, Pierre and {Bladh}, Sara and {Bressan}, Alessandro and {Girardi}, L{\'e}o and {Pastorelli}, Giada and {Trabucchi}, Michele and {Cheng}, Sihao and {Aringer}, Bernhard and {Tio}, Piero Dal},
        title = "{Carbon star formation as seen through the non-monotonic initial-final mass relation}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = jul,
       volume = {4},
        pages = {1102-1110},
          doi = {10.1038/s41550-020-1132-1},
archivePrefix = {arXiv},
       eprint = {2007.04163},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020NatAs...4.1102M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pastorelli2020,
       author = {{Pastorelli}, Giada and {Marigo}, Paola and {Girardi}, L{\'e}o and {Aringer}, Bernhard and {Chen}, Yang and {Rubele}, Stefano and {Trabucchi}, Michele and {Bladh}, Sara and {Boyer}, Martha L. and {Bressan}, Alessandro and {Dalcanton}, Julianne J. and {Groenewegen}, Martin A.~T. and {Lebzelter}, Thomas and {Mowlavi}, Nami and {Chubb}, Katy L. and {Cioni}, Maria-Rosa L. and {de Grijs}, Richard and {Ivanov}, Valentin D. and {Nanni}, Ambra and {van Loon}, Jacco Th and {Zaggia}, Simone},
        title = "{Constraining the thermally pulsing asymptotic giant branch phase with resolved stellar populations in the Large Magellanic Cloud}",
      journal = {\mnras},
     keywords = {stars: AGB and post-AGB, stars: evolution, Magellanic Clouds, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = nov,
       volume = {498},
       number = {3},
        pages = {3283-3301},
          doi = {10.1093/mnras/staa2565},
archivePrefix = {arXiv},
       eprint = {2008.08595},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.498.3283P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AbbotGW190521.1,
       author = {{Abbott}, R. and {Abbott}, T.~D. and {Abraham}, S. and {Acernese}, F. and {Ackley}, K. and {Adams}, C. and {Adhikari}, R.~X. and {Adya}, V.~B. and {Affeldt}, C. and {Agathos}, M. and {Agatsuma}, K. and {Aggarwal}, N. and {Aguiar}, O.~D. and {Aich}, A. and {Aiello}, L. and {Ain}, A. and {Ajith}, P. and {Akcay}, S. and {Allen}, G. and {Allocca}, A. and {Altin}, P.~A. and {Amato}, A. and {Anand}, S. and {Ananyeva}, A. and {Anderson}, S.~B. and {Anderson}, W.~G. and {Angelova}, S.~V. and {Ansoldi}, S. and {Antier}, S. and {Appert}, S. and {Arai}, K. and {Araya}, M.~C. and {Areeda}, J.~S. and {Ar{\`e}ne}, M. and {Arnaud}, N. and {Aronson}, S.~M. and {Arun}, K.~G. and {Asali}, Y. and {Ascenzi}, S. and {Ashton}, G. and {Aston}, S.~M. and {Astone}, P. and {Aubin}, F. and {Aufmuth}, P. and {AultONeal}, K. and {Austin}, C. and {Avendano}, V. and {Babak}, S. and {Bacon}, P. and {Badaracco}, F. and {Bader}, M.~K.~M. and {Bae}, S. and {Baer}, A.~M. and {Baird}, J. and {Baldaccini}, F. and {Ballardin}, G. and {Ballmer}, S.~W. and {Bals}, A. and {Balsamo}, A. and {Baltus}, G. and {Banagiri}, S. and {Bankar}, D. and {Bankar}, R.~S. and {Barayoga}, J.~C. and {Barbieri}, C. and {Barish}, B.~C. and {Barker}, D. and {Barkett}, K. and {Barneo}, P. and {Barone}, F. and {Barr}, B. and {Barsotti}, L. and {Barsuglia}, M. and {Barta}, D. and {Bartlett}, J. and {Bartos}, I. and {Bassiri}, R. and {Basti}, A. and {Bawaj}, M. and {Bayley}, J.~C. and {Bazzan}, M. and {B{\'e}csy}, B. and {Bejger}, M. and {Belahcene}, I. and {Bell}, A.~S. and {Beniwal}, D. and {Benjamin}, M.~G. and {Bentley}, J.~D. and {Bergamin}, F. and {Berger}, B.~K. and {Bergmann}, G. and {Bernuzzi}, S. and {Berry}, C.~P.~L. and {Bersanetti}, D. and {Bertolini}, A. and {Betzwieser}, J. and {Bhandare}, R. and {Bhandari}, A.~V. and {Bidler}, J. and {Biggs}, E. and {Bilenko}, I.~A. and {Billingsley}, G. and {Birney}, R. and {Birnholtz}, O. and {Biscans}, S. and {Bischi}, M. and {Biscoveanu}, S. and {Bisht}, A. and {Bissenbayeva}, G. and {Bitossi}, M. and {Bizouard}, M.~A. and {Blackburn}, J.~K. and {Blackman}, J. and {Blair}, C.~D. and {Blair}, D.~G. and {Blair}, R.~M. and {Bobba}, F. and {Bode}, N. and {Boer}, M. and {Boetzel}, Y. and {Bogaert}, G. and {Bondu}, F. and {Bonilla}, E. and {Bonnand}, R. and {Booker}, P. and {Boom}, B.~A. and {Bork}, R. and {Boschi}, V. and {Bose}, S. and {Bossilkov}, V. and {Bosveld}, J. and {Bouffanais}, Y. and {Bozzi}, A. and {Bradaschia}, C. and {Brady}, P.~R. and {Bramley}, A. and {Branchesi}, M. and {Brau}, J.~E. and {Breschi}, M. and {Briant}, T. and {Briggs}, J.~H. and {Brighenti}, F. and {Brillet}, A. and {Brinkmann}, M. and {Brockill}, P. and {Brooks}, A.~F. and {Brooks}, J. and {Brown}, D.~D. and {Brunett}, S. and {Bruno}, G. and {Bruntz}, R. and {Buikema}, A. and {Bulik}, T. and {Bulten}, H.~J. and {Buonanno}, A. and {Buscicchio}, R. and {Buskulic}, D. and {Byer}, R.~L. and {Cabero}, M. and {Cadonati}, L. and {Cagnoli}, G. and {Cahillane}, C. and {Calder{\'o}n Bustillo}, J. and {Callaghan}, J.~D. and {Callister}, T.~A. and {Calloni}, E. and {Camp}, J.~B. and {Canepa}, M. and {Cannon}, K.~C. and {Cao}, H. and {Cao}, J. and {Carapella}, G. and {Carbognani}, F. and {Caride}, S. and {Carney}, M.~F. and {Carullo}, G. and {Casanueva Diaz}, J. and {Casentini}, C. and {Casta{\~n}eda}, J. and {Caudill}, S. and {Cavagli{\`a}}, M. and {Cavalier}, F. and {Cavalieri}, R. and {Cella}, G. and {Cerd{\'a}-Dur{\'a}n}, P. and {Cesarini}, E. and {Chaibi}, O. and {Chakravarti}, K. and {Chan}, C. and {Chan}, M. and {Chandra}, K. and {Chao}, S. and {Charlton}, P. and {Chase}, E.~A. and {Chassande-Mottin}, E. and {Chatterjee}, D. and {Chaturvedi}, M. and {Chatziioannou}, K. and {Chen}, H.~Y. and {Chen}, X. and {Chen}, Y. and {Cheng}, H. -P. and {Cheong}, C.~K. and {Chia}, H.~Y. and {Chiadini}, F. and {Chierici}, R. and {Chincarini}, A. and {Chiummo}, A. and {Cho}, G. and {Cho}, H.~S. and {Cho}, M. and {Christensen}, N. and {Chu}, Q. and {Chua}, S. and {Chung}, K.~W. and {Chung}, S. and {Ciani}, G. and {Ciecielag}, P. and {Cie{\'s}lar}, M. and {Ciobanu}, A.~A. and {Ciolfi}, R. and {Cipriano}, F. and {Cirone}, A. and {Clara}, F. and {Clark}, J.~A. and {Clearwater}, P. and {Clesse}, S. and {Cleva}, F. and {Coccia}, E. and {Cohadon}, P. -F. and {Cohen}, D. and {Colleoni}, M. and {Collette}, C.~G. and {Collins}, C. and {Colpi}, M. and {Constancio}, M. and {Conti}, L. and {Cooper}, S.~J. and {Corban}, P. and {Corbitt}, T.~R. and {Cordero-Carri{\'o}n}, I. and {Corezzi}, S. and {Corley}, K.~R. and {Cornish}, N. and {Corre}, D. and {Corsi}, A. and {Cortese}, S. and {Costa}, C.~A. and {Cotesta}, R. and {Coughlin}, M.~W. and {Coughlin}, S.~B. and {Coulon}, J. -P. and {Countryman}, S.~T. and {Couvares}, P. and {Covas}, P.~B. and {Coward}, D.~M. and {Cowart}, M.~J. and {Coyne}, D.~C. and {Coyne}, R. and {Creighton}, J.~D.~E. and {Creighton}, T.~D. and {Cripe}, J. and {Croquette}, M. and {Crowder}, S.~G. and {Cudell}, J. -R. and {Cullen}, T.~J. and {Cumming}, A. and {Cummings}, R. and {Cunningham}, L. and {Cuoco}, E. and {Curylo}, M. and {Canton}, T. Dal and {D{\'a}lya}, G. and {Dana}, A. and {Daneshgaran-Bajastani}, L.~M. and {D'Angelo}, B. and {Danilishin}, S.~L. and {D'Antonio}, S. and {Danzmann}, K. and {Darsow-Fromm}, C. and {Dasgupta}, A. and {Datrier}, L.~E.~H. and {Dattilo}, V. and {Dave}, I. and {Davier}, M. and {Davies}, G.~S. and {Davis}, D. and {Daw}, E.~J. and {DeBra}, D. and {Deenadayalan}, M. and {Degallaix}, J. and {De Laurentis}, M. and {Del{\'e}glise}, S. and {Delfavero}, M. and {De Lillo}, N. and {Del Pozzo}, W. and {DeMarchi}, L.~M. and {D'Emilio}, V. and {Demos}, N. and {Dent}, T. and {De Pietri}, R. and {De Rosa}, R. and {De Rossi}, C. and {DeSalvo}, R. and {de Varona}, O. and {Dhurandhar}, S. and {D{\'\i}az}, M.~C. and {Diaz-Ortiz}, M. and {Dietrich}, T. and {Di Fiore}, L. and {Di Fronzo}, C. and {Di Giorgio}, C. and {Di Giovanni}, F. and {Di Giovanni}, M. and {Di Girolamo}, T. and {Di Lieto}, A. and {Ding}, B. and {Di Pace}, S. and {Di Palma}, I. and {Di Renzo}, F. and {Divakarla}, A.~K. and {Dmitriev}, A. and {Doctor}, Z. and {Donovan}, F. and {Dooley}, K.~L. and {Doravari}, S. and {Dorrington}, I. and {Downes}, T.~P. and {Drago}, M. and {Driggers}, J.~C. and {Du}, Z. and {Ducoin}, J. -G. and {Dupej}, P. and {Durante}, O. and {D'Urso}, D. and {Dwyer}, S.~E. and {Easter}, P.~J. and {Eddolls}, G. and {Edelman}, B. and {Edo}, T.~B. and {Edy}, O. and {Effler}, A. and {Ehrens}, P. and {Eichholz}, J. and {Eikenberry}, S.~S. and {Eisenmann}, M. and {Eisenstein}, R.~A. and {Ejlli}, A. and {Errico}, L. and {Essick}, R.~C. and {Estelles}, H. and {Estevez}, D. and {Etienne}, Z.~B. and {Etzel}, T. and {Evans}, M. and {Evans}, T.~M. and {Ewing}, B.~E. and {Fafone}, V. and {Fairhurst}, S. and {Fan}, X. and {Farinon}, S. and {Farr}, B. and {Farr}, W.~M. and {Fauchon-Jones}, E.~J. and {Favata}, M. and {Fays}, M. and {Fazio}, M. and {Feicht}, J. and {Fejer}, M.~M. and {Feng}, F. and {Fenyvesi}, E. and {Ferguson}, D.~L. and {Fernandez-Galiana}, A. and {Ferrante}, I. and {Ferreira}, E.~C. and {Ferreira}, T.~A. and {Fidecaro}, F. and {Fiori}, I. and {Fiorucci}, D. and {Fishbach}, M. and {Fisher}, R.~P. and {Fittipaldi}, R. and {Fitz-Axen}, M. and {Fiumara}, V. and {Flaminio}, R. and {Floden}, E. and {Flynn}, E. and {Fong}, H. and {Font}, J.~A. and {Forsyth}, P.~W.~F. and {Fournier}, J. -D. and {Frasca}, S. and {Frasconi}, F. and {Frei}, Z. and {Freise}, A. and {Frey}, R. and {Frey}, V. and {Fritschel}, P. and {Frolov}, V.~V. and {Fronz{\`e}}, G. and {Fulda}, P. and {Fyffe}, M. and {Gabbard}, H.~A. and {Gadre}, B.~U. and {Gaebel}, S.~M. and {Gair}, J.~R. and {Galaudage}, S. and {Ganapathy}, D. and {Ganguly}, A. and {Gaonkar}, S.~G. and {Garc{\'\i}a-Quir{\'o}s}, C. and {Garufi}, F. and {Gateley}, B. and {Gaudio}, S. and {Gayathri}, V. and {Gemme}, G. and {Genin}, E. and {Gennai}, A. and {George}, D. and {George}, J. and {Gergely}, L. and {Ghonge}, S. and {Ghosh}, Abhirup and {Ghosh}, Archisman and {Ghosh}, S. and {Giacomazzo}, B. and {Giaime}, J.~A. and {Giardina}, K.~D. and {Gibson}, D.~R. and {Gier}, C. and {Gill}, K. and {Glanzer}, J. and {Gniesmer}, J. and {Godwin}, P. and {Goetz}, E. and {Goetz}, R. and {Gohlke}, N. and {Goncharov}, B. and {Gonz{\'a}lez}, G. and {Gopakumar}, A. and {Gossan}, S.~E. and {Gosselin}, M. and {Gouaty}, R. and {Grace}, B. and {Grado}, A. and {Granata}, M. and {Grant}, A. and {Gras}, S. and {Grassia}, P. and {Gray}, C. and {Gray}, R. and {Greco}, G. and {Green}, A.~C. and {Green}, R. and {Gretarsson}, E.~M. and {Griggs}, H.~L. and {Grignani}, G. and {Grimaldi}, A. and {Grimm}, S.~J. and {Grote}, H. and {Grunewald}, S. and {Gruning}, P. and {Guidi}, G.~M. and {Guimaraes}, A.~R. and {Guix{\'e}}, G. and {Gulati}, H.~K. and {Guo}, Y. and {Gupta}, A. and {Gupta}, Anchal and {Gupta}, P. and {Gustafson}, E.~K. and {Gustafson}, R. and {Haegel}, L. and {Halim}, O. and {Hall}, E.~D. and {Hamilton}, E.~Z. and {Hammond}, G. and {Haney}, M. and {Hanke}, M.~M. and {Hanks}, J. and {Hanna}, C. and {Hannam}, M.~D. and {Hannuksela}, O.~A. and {Hansen}, T.~J. and {Hanson}, J. and {Harder}, T. and {Hardwick}, T. and {Haris}, K. and {Harms}, J. and {Harry}, G.~M. and {Harry}, I.~W. and {Hasskew}, R.~K. and {Haster}, C. -J. and {Haughian}, K. and {Hayes}, F.~J. and {Healy}, J. and {Heidmann}, A. and {Heintze}, M.~C. and {Heinze}, J. and {Heitmann}, H. and {Hellman}, F. and {Hello}, P. and {Hemming}, G. and {Hendry}, M. and {Heng}, I.~S. and {Hennes}, E. and {Hennig}, J. and {Heurs}, M. and {Hild}, S. and {Hinderer}, T. and {Hoback}, S.~Y. and {Hochheim}, S. and {Hofgard}, E. and {Hofman}, D. and {Holgado}, A.~M. and {Holland}, N.~A. and {Holt}, K. and {Holz}, D.~E. and {Hopkins}, P. and {Horst}, C. and {Hough}, J. and {Howell}, E.~J. and {Hoy}, C.~G. and {Huang}, Y. and {H{\"u}bner}, M.~T. and {Huerta}, E.~A. and {Huet}, D. and {Hughey}, B. and {Hui}, V. and {Husa}, S. and {Huttner}, S.~H. and {Huxford}, R. and {Huynh-Dinh}, T. and {Idzkowski}, B. and {Iess}, A. and {Inchauspe}, H. and {Ingram}, C. and {Intini}, G. and {Isac}, J. -M. and {Isi}, M. and {Iyer}, B.~R. and {Jacqmin}, T. and {Jadhav}, S.~J. and {Jadhav}, S.~P. and {James}, A.~L. and {Jani}, K. and {Janthalur}, N.~N. and {Jaranowski}, P. and {Jariwala}, D. and {Jaume}, R. and {Jenkins}, A.~C. and {Jiang}, J. and {Johns}, G.~R. and {Johnson-McDaniel}, N.~K. and {Jones}, A.~W. and {Jones}, D.~I. and {Jones}, J.~D. and {Jones}, P. and {Jones}, R. and {Jonker}, R.~J.~G. and {Ju}, L. and {Junker}, J. and {Kalaghatgi}, C.~V. and {Kalogera}, V. and {Kamai}, B. and {Kandhasamy}, S. and {Kang}, G. and {Kanner}, J.~B. and {Kapadia}, S.~J. and {Karki}, S. and {Kashyap}, R. and {Kasprzack}, M. and {Kastaun}, W. and {Katsanevas}, S. and {Katsavounidis}, E. and {Katzman}, W. and {Kaufer}, S. and {Kawabe}, K. and {K{\'e}f{\'e}lian}, F. and {Keitel}, D. and {Keivani}, A. and {Kennedy}, R. and {Key}, J.~S. and {Khadka}, S. and {Khalili}, F.~Y. and {Khan}, I. and {Khan}, S. and {Khan}, Z.~A. and {Khazanov}, E.~A. and {Khetan}, N. and {Khursheed}, M. and {Kijbunchoo}, N. and {Kim}, Chunglee and {Kim}, G.~J. and {Kim}, J.~C. and {Kim}, K. and {Kim}, W. and {Kim}, W.~S. and {Kim}, Y. -M. and {Kimball}, C. and {King}, P.~J. and {Kinley-Hanlon}, M. and {Kirchhoff}, R. and {Kissel}, J.~S. and {Kleybolte}, L. and {Klimenko}, S. and {Knowles}, T.~D. and {Knyazev}, E. and {Koch}, P. and {Koehlenbeck}, S.~M. and {Koekoek}, G. and {Koley}, S. and {Kondrashov}, V. and {Kontos}, A. and {Koper}, N. and {Korobko}, M. and {Korth}, W.~Z. and {Kovalam}, M. and {Kozak}, D.~B. and {Kringel}, V. and {Krishnendu}, N.~V. and {Kr{\'o}lak}, A. and {Krupinski}, N. and {Kuehn}, G. and {Kumar}, A. and {Kumar}, P. and {Kumar}, Rahul and {Kumar}, Rakesh and {Kumar}, S. and {Kuo}, L. and {Kutynia}, A. and {Lackey}, B.~D. and {Laghi}, D. and {Lalande}, E. and {Lam}, T.~L. and {Lamberts}, A. and {Landry}, M. and {Lane}, B.~B. and {Lang}, R.~N. and {Lange}, J. and {Lantz}, B. and {Lanza}, R.~K. and {La Rosa}, I. and {Lartaux-Vollard}, A. and {Lasky}, P.~D. and {Laxen}, M. and {Lazzarini}, A. and {Lazzaro}, C. and {Leaci}, P. and {Leavey}, S. and {Lecoeuche}, Y.~K. and {Lee}, C.~H. and {Lee}, H.~M. and {Lee}, H.~W. and {Lee}, J. and {Lee}, K. and {Lehmann}, J. and {Leroy}, N. and {Letendre}, N. and {Levin}, Y. and {Li}, A.~K.~Y. and {Li}, J. and {li}, K. and {Li}, T.~G.~F. and {Li}, X. and {Linde}, F. and {Linker}, S.~D. and {Linley}, J.~N. and {Littenberg}, T.~B. and {Liu}, J. and {Liu}, X. and {Llorens-Monteagudo}, M. and {Lo}, R.~K.~L. and {Lockwood}, A. and {London}, L.~T. and {Longo}, A. and {Lorenzini}, M. and {Loriette}, V. and {Lormand}, M. and {Losurdo}, G. and {Lough}, J.~D. and {Lousto}, C.~O. and {Lovelace}, G. and {L{\"u}ck}, H. and {Lumaca}, D. and {Lundgren}, A.~P. and {Ma}, Y. and {Macas}, R. and {Macfoy}, S. and {MacInnis}, M. and {Macleod}, D.~M. and {MacMillan}, I.~A.~O. and {Macquet}, A. and {Maga{\~n}a Hernandez}, I. and {Maga{\~n}a-Sandoval}, F. and {Magee}, R.~M. and {Majorana}, E. and {Maksimovic}, I. and {Malik}, A. and {Man}, N. and {Mandic}, V. and {Mangano}, V. and {Mansell}, G.~L. and {Manske}, M. and {Mantovani}, M. and {Mapelli}, M. and {Marchesoni}, F. and {Marion}, F. and {M{\'a}rka}, S. and {M{\'a}rka}, Z. and {Markakis}, C. and {Markosyan}, A.~S. and {Markowitz}, A. and {Maros}, E. and {Marquina}, A. and {Marsat}, S. and {Martelli}, F. and {Martin}, I.~W. and {Martin}, R.~M. and {Martinez}, V. and {Martynov}, D.~V. and {Masalehdan}, H. and {Mason}, K. and {Massera}, E. and {Masserot}, A. and {Massinger}, T.~J. and {Masso-Reid}, M. and {Mastrogiovanni}, S. and {Matas}, A. and {Matichard}, F. and {Mavalvala}, N. and {Maynard}, E. and {McCann}, J.~J. and {McCarthy}, R. and {McClelland}, D.~E. and {McCormick}, S. and {McCuller}, L. and {McGuire}, S.~C. and {McIsaac}, C. and {McIver}, J. and {McManus}, D.~J. and {McRae}, T. and {McWilliams}, S.~T. and {Meacher}, D. and {Meadors}, G.~D. and {Mehmet}, M. and {Mehta}, A.~K. and {Mejuto Villa}, E. and {Melatos}, A. and {Mendell}, G. and {Mercer}, R.~A. and {Mereni}, L. and {Merfeld}, K. and {Merilh}, E.~L. and {Merritt}, J.~D. and {Merzougui}, M. and {Meshkov}, S. and {Messenger}, C. and {Messick}, C. and {Metzdorff}, R. and {Meyers}, P.~M. and {Meylahn}, F. and {Mhaske}, A. and {Miani}, A. and {Miao}, H. and {Michaloliakos}, I. and {Michel}, C. and {Middleton}, H. and {Milano}, L. and {Miller}, A.~L. and {Millhouse}, M. and {Mills}, J.~C. and {Milotti}, E. and {Milovich-Goff}, M.~C. and {Minazzoli}, O. and {Minenkov}, Y. and {Mishkin}, A. and {Mishra}, C. and {Mistry}, T. and {Mitra}, S. and {Mitrofanov}, V.~P. and {Mitselmakher}, G. and {Mittleman}, R. and {Mo}, G. and {Mogushi}, K. and {Mohapatra}, S.~R.~P. and {Mohite}, S.~R. and {Molina-Ruiz}, M. and {Mondin}, M. and {Montani}, M. and {Moore}, C.~J. and {Moraru}, D. and {Morawski}, F. and {Moreno}, G. and {Morisaki}, S. and {Mours}, B. and {Mow-Lowry}, C.~M. and {Mozzon}, S. and {Muciaccia}, F. and {Mukherjee}, Arunava and {Mukherjee}, D. and {Mukherjee}, S. and {Mukherjee}, Subroto and {Mukund}, N. and {Mullavey}, A. and {Munch}, J. and {Mu{\~n}iz}, E.~A. and {Murray}, P.~G. and {Nagar}, A. and {Nardecchia}, I. and {Naticchioni}, L. and {Nayak}, R.~K. and {Neil}, B.~F. and {Neilson}, J. and {Nelemans}, G. and {Nelson}, T.~J.~N. and {Nery}, M. and {Neunzert}, A. and {Ng}, K.~Y. and {Ng}, S. and {Nguyen}, C. and {Nguyen}, P. and {Nichols}, D. and {Nichols}, S.~A. and {Nissanke}, S. and {Nitz}, A. and {Nocera}, F. and {Noh}, M. and {North}, C. and {Nothard}, D. and {Nuttall}, L.~K. and {Oberling}, J. and {O'Brien}, B.~D. and {Oganesyan}, G. and {Ogin}, G.~H. and {Oh}, J.~J. and {Oh}, S.~H. and {Ohme}, F. and {Ohta}, H. and {Okada}, M.~A. and {Oliver}, M. and {Olivetto}, C. and {Oppermann}, P. and {Oram}, Richard J. and {O'Reilly}, B. and {Ormiston}, R.~G. and {Ortega}, L.~F. and {O'Shaughnessy}, R. and {Ossokine}, S. and {Osthelder}, C. and {Ottaway}, D.~J. and {Overmier}, H. and {Owen}, B.~J. and {Pace}, A.~E. and {Pagano}, G. and {Page}, M.~A. and {Pagliaroli}, G. and {Pai}, A. and {Pai}, S.~A. and {Palamos}, J.~R. and {Palashov}, O. and {Palomba}, C. and {Pan}, H. and {Panda}, P.~K. and {Pang}, P.~T.~H. and {Pankow}, C. and {Pannarale}, F. and {Pant}, B.~C. and {Paoletti}, F. and {Paoli}, A. and {Parida}, A. and {Parker}, W. and {Pascucci}, D. and {Pasqualetti}, A. and {Passaquieti}, R. and {Passuello}, D. and {Patricelli}, B. and {Payne}, E. and {Pearlstone}, B.~L. and {Pechsiri}, T.~C. and {Pedersen}, A.~J. and {Pedraza}, M. and {Pele}, A. and {Penn}, S. and {Perego}, A. and {Perez}, C.~J. and {P{\'e}rigois}, C. and {Perreca}, A. and {Perri{\`e}s}, S. and {Petermann}, J. and {Pfeiffer}, H.~P. and {Phelps}, M. and {Phukon}, K.~S. and {Piccinni}, O.~J. and {Pichot}, M. and {Piendibene}, M. and {Piergiovanni}, F. and {Pierro}, V. and {Pillant}, G. and {Pinard}, L. and {Pinto}, I.~M. and {Piotrzkowski}, K. and {Pirello}, M. and {Pitkin}, M. and {Plastino}, W. and {Poggiani}, R. and {Pong}, D.~Y.~T. and {Ponrathnam}, S. and {Popolizio}, P. and {Porter}, E.~K. and {Powell}, J. and {Prajapati}, A.~K. and {Prasai}, K. and {Prasanna}, R. and {Pratten}, G. and {Prestegard}, T. and {Principe}, M. and {Prodi}, G.~A. and {Prokhorov}, L. and {Punturo}, M. and {Puppo}, P. and {P{\"u}rrer}, M. and {Qi}, H. and {Quetschke}, V. and {Quinonez}, P.~J. and {Raab}, F.~J. and {Raaijmakers}, G. and {Radkins}, H. and {Radulesco}, N. and {Raffai}, P. and {Rafferty}, H. and {Raja}, S. and {Rajan}, C. and {Rajbhandari}, B. and {Rakhmanov}, M. and {Ramirez}, K.~E. and {Ramos-Buades}, A. and {Rana}, Javed and {Rao}, K. and {Rapagnani}, P. and {Raymond}, V. and {Razzano}, M. and {Read}, J. and {Regimbau}, T. and {Rei}, L. and {Reid}, S. and {Reitze}, D.~H. and {Rettegno}, P. and {Ricci}, F. and {Richardson}, C.~J. and {Richardson}, J.~W. and {Ricker}, P.~M. and {Riemenschneider}, G. and {Riles}, K. and {Rizzo}, M. and {Robertson}, N.~A. and {Robinet}, F. and {Rocchi}, A. and {Rodriguez-Soto}, R.~D. and {Rolland}, L. and {Rollins}, J.~G. and {Roma}, V.~J. and {Romanelli}, M. and {Romano}, R. and {Romel}, C.~L. and {Romero-Shaw}, I.~M. and {Romie}, J.~H. and {Rose}, C.~A. and {Rose}, D. and {Rose}, K. and {Rosi{\'n}ska}, D. and {Rosofsky}, S.~G. and {Ross}, M.~P. and {Rowan}, S. and {Rowlinson}, S.~J. and {Roy}, P.~K. and {Roy}, Santosh and {Roy}, Soumen and {Ruggi}, P. and {Rutins}, G. and {Ryan}, K. and {Sachdev}, S. and {Sadecki}, T. and {Sakellariadou}, M. and {Salafia}, O.~S. and {Salconi}, L. and {Saleem}, M. and {Salemi}, F. and {Samajdar}, A. and {Sanchez}, E.~J. and {Sanchez}, L.~E. and {Sanchis-Gual}, N. and {Sanders}, J.~R. and {Santiago}, K.~A. and {Santos}, E. and {Sarin}, N. and {Sassolas}, B. and {Sathyaprakash}, B.~S. and {Sauter}, O. and {Savage}, R.~L. and {Savant}, V. and {Sawant}, D. and {Sayah}, S. and {Schaetzl}, D. and {Schale}, P. and {Scheel}, M. and {Scheuer}, J. and {Schmidt}, P. and {Schnabel}, R. and {Schofield}, R.~M.~S. and {Sch{\"o}nbeck}, A. and {Schreiber}, E. and {Schulte}, B.~W. and {Schutz}, B.~F. and {Schwarm}, O. and {Schwartz}, E. and {Scott}, J. and {Scott}, S.~M. and {Seidel}, E. and {Sellers}, D. and {Sengupta}, A.~S. and {Sennett}, N. and {Sentenac}, D. and {Sequino}, V. and {Sergeev}, A. and {Setyawati}, Y. and {Shaddock}, D.~A. and {Shaffer}, T. and {Sharifi}, S. and {Shahriar}, M.~S. and {Sharma}, A. and {Sharma}, P. and {Shawhan}, P. and {Shen}, H. and {Shikauchi}, M. and {Shink}, R. and {Shoemaker}, D.~H. and {Shoemaker}, D.~M. and {Shukla}, K. and {ShyamSundar}, S. and {Siellez}, K. and {Sieniawska}, M. and {Sigg}, D. and {Singer}, L.~P. and {Singh}, D. and {Singh}, N. and {Singha}, A. and {Singhal}, A. and {Sintes}, A.~M. and {Sipala}, V. and {Skliris}, V. and {Slagmolen}, B.~J.~J. and {Slaven-Blair}, T.~J. and {Smetana}, J. and {Smith}, J.~R. and {Smith}, R.~J.~E. and {Somala}, S. and {Son}, E.~J. and {Soni}, S. and {Sorazu}, B. and {Sordini}, V. and {Sorrentino}, F. and {Souradeep}, T. and {Sowell}, E. and {Spencer}, A.~P. and {Spera}, M. and {Srivastava}, A.~K. and {Srivastava}, V. and {Staats}, K. and {Stachie}, C. and {Standke}, M. and {Steer}, D.~A. and {Steinke}, M. and {Steinlechner}, J. and {Steinlechner}, S. and {Steinmeyer}, D. and {Stevenson}, S. and {Stocks}, D. and {Stops}, D.~J. and {Stover}, M. and {Strain}, K.~A. and {Stratta}, G. and {Strunk}, A. and {Sturani}, R. and {Stuver}, A.~L. and {Sudhagar}, S. and {Sudhir}, V. and {Summerscales}, T.~Z. and {Sun}, L. and {Sunil}, S. and {Sur}, A. and {Suresh}, J. and {Sutton}, P.~J. and {Swinkels}, B.~L. and {Szczepa{\'n}czyk}, M.~J. and {Tacca}, M. and {Tait}, S.~C. and {Talbot}, C. and {Tanasijczuk}, A.~J. and {Tanner}, D.~B. and {Tao}, D. and {T{\'a}pai}, M. and {Tapia}, A. and {Tapia San Martin}, E.~N. and {Tasson}, J.~D. and {Taylor}, R. and {Tenorio}, R. and {Terkowski}, L. and {Thirugnanasambandam}, M.~P. and {Thomas}, M. and {Thomas}, P. and {Thompson}, J.~E. and {Thondapu}, S.~R. and {Thorne}, K.~A. and {Thrane}, E. and {Tinsman}, C.~L. and {Saravanan}, T.~R. and {Tiwari}, Shubhanshu and {Tiwari}, S. and {Tiwari}, V. and {Toland}, K. and {Tonelli}, M. and {Tornasi}, Z. and {Torres-Forn{\'e}}, A. and {Torrie}, C.~I. and {Tosta e Melo}, I. and {T{\"o}yr{\"a}}, D. and {Travasso}, F. and {Traylor}, G. and {Tringali}, M.~C. and {Tripathee}, A. and {Trovato}, A. and {Trudeau}, R.~J. and {Tsang}, K.~W. and {Tse}, M. and {Tso}, R. and {Tsukada}, L. and {Tsuna}, D. and {Tsutsui}, T. and {Turconi}, M. and {Ubhi}, A.~S. and {Udall}, R. and {Ueno}, K. and {Ugolini}, D. and {Unnikrishnan}, C.~S. and {Urban}, A.~L. and {Usman}, S.~A. and {Utina}, A.~C. and {Vahlbruch}, H. and {Vajente}, G. and {Valdes}, G. and {Valentini}, M. and {van Bakel}, N. and {van Beuzekom}, M. and {van den Brand}, J.~F.~J. and {Van Den Broeck}, C. and {Vander-Hyde}, D.~C. and {van der Schaaf}, L. and {Van Heijningen}, J.~V. and {van Veggel}, A.~A. and {Vardaro}, M. and {Varma}, V. and {Vass}, S. and {Vas{\'u}th}, M. and {Vecchio}, A. and {Vedovato}, G. and {Veitch}, J. and {Veitch}, P.~J. and {Venkateswara}, K. and {Venugopalan}, G. and {Verkindt}, D. and {Veske}, D. and {Vetrano}, F. and {Vicer{\'e}}, A. and {Viets}, A.~D. and {Vinciguerra}, S. and {Vine}, D.~J. and {Vinet}, J. -Y. and {Vitale}, S. and {Vivanco}, Francisco Hernandez and {Vo}, T. and {Vocca}, H. and {Vorvick}, C. and {Vyatchanin}, S.~P. and {Wade}, A.~R. and {Wade}, L.~E. and {Wade}, M. and {Walet}, R. and {Walker}, M. and {Wallace}, G.~S. and {Wallace}, L. and {Walsh}, S. and {Wang}, J.~Z. and {Wang}, S. and {Wang}, W.~H. and {Ward}, R.~L. and {Warden}, Z.~A. and {Warner}, J. and {Was}, M. and {Watchi}, J. and {Weaver}, B. and {Wei}, L. -W. and {Weinert}, M. and {Weinstein}, A.~J. and {Weiss}, R. and {Wellmann}, F. and {Wen}, L. and {We{\ss}els}, P. and {Westhouse}, J.~W. and {Wette}, K. and {Whelan}, J.~T. and {Whiting}, B.~F. and {Whittle}, C. and {Wilken}, D.~M. and {Williams}, D. and {Willis}, J.~L. and {Willke}, B. and {Winkler}, W. and {Wipf}, C.~C. and {Wittel}, H. and {Woan}, G. and {Woehler}, J. and {Wofford}, J.~K. and {Wong}, I.~C.~F. and {Wright}, J.~L. and {Wu}, D.~S. and {Wysocki}, D.~M. and {Xiao}, L. and {Yamamoto}, H. and {Yang}, L. and {Yang}, Y. and {Yang}, Z. and {Yap}, M.~J. and {Yazback}, M. and {Yeeles}, D.~W. and {Yu}, Hang and {Yu}, Haocun and {Yuen}, S.~H.~R. and {Zadro{\.Z}ny}, A.~K. and {Zadro{\.Z}ny}, A. and {Zanolin}, M. and {Zelenova}, T. and {Zendri}, J. -P. and {Zevin}, M. and {Zhang}, J. and {Zhang}, L. and {Zhang}, T. and {Zhao}, C. and {Zhao}, G. and {Zhou}, M. and {Zhou}, Z. and {Zhu}, X.~J. and {Zimmerman}, A.~B. and {Zucker}, M.~E. and {Zweizig}, J. and {LIGO Scientific Collaboration} and {Virgo Collaboration}},
        title = "{GW190521: A Binary Black Hole Merger with a Total Mass of 150 M$_{{\ensuremath{\odot}}}$}",
      journal = {\prl},
     keywords = {General Relativity and Quantum Cosmology, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = sep,
       volume = {125},
       number = {10},
          eid = {101102},
        pages = {101102},
          doi = {10.1103/PhysRevLett.125.101102},
archivePrefix = {arXiv},
       eprint = {2009.01075},
 primaryClass = {gr-qc},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020PhRvL.125j1102A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Abbot2020GW190521.2,
       author = {{Abbott}, R. and {Abbott}, T.~D. and {Abraham}, S. and {Acernese}, F. and {Ackley}, K. and {Adams}, C. and {Adhikari}, R.~X. and {Adya}, V.~B. and {Affeldt}, C. and {Agathos}, M. and {Agatsuma}, K. and {Aggarwal}, N. and {Aguiar}, O.~D. and {Aich}, A. and {Aiello}, L. and {Ain}, A. and {Ajith}, P. and {Akcay}, S. and {Allen}, G. and {Allocca}, A. and {Altin}, P.~A. and {Amato}, A. and {Anand}, S. and {Ananyeva}, A. and {Anderson}, S.~B. and {Anderson}, W.~G. and {Angelova}, S.~V. and {Ansoldi}, S. and {Antier}, S. and {Appert}, S. and {Arai}, K. and {Araya}, M.~C. and {Areeda}, J.~S. and {Ar{\`e}ne}, M. and {Arnaud}, N. and {Aronson}, S.~M. and {Arun}, K.~G. and {Asali}, Y. and {Ascenzi}, S. and {Ashton}, G. and {Aston}, S.~M. and {Astone}, P. and {Aubin}, F. and {Aufmuth}, P. and {AultONeal}, K. and {Austin}, C. and {Avendano}, V. and {Babak}, S. and {Bacon}, P. and {Badaracco}, F. and {Bader}, M.~K.~M. and {Bae}, S. and {Baer}, A.~M. and {Baird}, J. and {Baldaccini}, F. and {Ballardin}, G. and {Ballmer}, S.~W. and {Bals}, A. and {Balsamo}, A. and {Baltus}, G. and {Banagiri}, S. and {Bankar}, D. and {Bankar}, R.~S. and {Barayoga}, J.~C. and {Barbieri}, C. and {Barish}, B.~C. and {Barker}, D. and {Barkett}, K. and {Barneo}, P. and {Barone}, F. and {Barr}, B. and {Barsotti}, L. and {Barsuglia}, M. and {Barta}, D. and {Bartlett}, J. and {Bartos}, I. and {Bassiri}, R. and {Basti}, A. and {Bawaj}, M. and {Bayley}, J.~C. and {Bazzan}, M. and {B{\'e}csy}, B. and {Bejger}, M. and {Belahcene}, I. and {Bell}, A.~S. and {Beniwal}, D. and {Benjamin}, M.~G. and {Bentley}, J.~D. and {Bergamin}, F. and {Berger}, B.~K. and {Bergmann}, G. and {Bernuzzi}, S. and {Berry}, C.~P.~L. and {Bersanetti}, D. and {Bertolini}, A. and {Betzwieser}, J. and {Bhandare}, R. and {Bhandari}, A.~V. and {Bidler}, J. and {Biggs}, E. and {Bilenko}, I.~A. and {Billingsley}, G. and {Birney}, R. and {Birnholtz}, O. and {Biscans}, S. and {Bischi}, M. and {Biscoveanu}, S. and {Bisht}, A. and {Bissenbayeva}, G. and {Bitossi}, M. and {Bizouard}, M.~A. and {Blackburn}, J.~K. and {Blackman}, J. and {Blair}, C.~D. and {Blair}, D.~G. and {Blair}, R.~M. and {Bobba}, F. and {Bode}, N. and {Boer}, M. and {Boetzel}, Y. and {Bogaert}, G. and {Bondu}, F. and {Bonilla}, E. and {Bonnand}, R. and {Booker}, P. and {Boom}, B.~A. and {Bork}, R. and {Boschi}, V. and {Bose}, S. and {Bossilkov}, V. and {Bosveld}, J. and {Bouffanais}, Y. and {Bozzi}, A. and {Bradaschia}, C. and {Brady}, P.~R. and {Bramley}, A. and {Branchesi}, M. and {Brau}, J.~E. and {Breschi}, M. and {Briant}, T. and {Briggs}, J.~H. and {Brighenti}, F. and {Brillet}, A. and {Brinkmann}, M. and {Brockill}, P. and {Brooks}, A.~F. and {Brooks}, J. and {Brown}, D.~D. and {Brunett}, S. and {Bruno}, G. and {Bruntz}, R. and {Buikema}, A. and {Bulik}, T. and {Bulten}, H.~J. and {Buonanno}, A. and {Buscicchio}, R. and {Buskulic}, D. and {Byer}, R.~L. and {Cabero}, M. and {Cadonati}, L. and {Cagnoli}, G. and {Cahillane}, C. and {Bustillo}, J. Calder{\'o}n and {Callaghan}, J.~D. and {Callister}, T.~A. and {Calloni}, E. and {Camp}, J.~B. and {Canepa}, M. and {Cannon}, K.~C. and {Cao}, H. and {Cao}, J. and {Carapella}, G. and {Carbognani}, F. and {Caride}, S. and {Carney}, M.~F. and {Carullo}, G. and {Diaz}, J. Casanueva and {Casentini}, C. and {Casta{\~n}eda}, J. and {Caudill}, S. and {Cavagli{\`a}}, M. and {Cavalier}, F. and {Cavalieri}, R. and {Cella}, G. and {Cerd{\'a}-Dur{\'a}n}, P. and {Cesarini}, E. and {Chaibi}, O. and {Chakravarti}, K. and {Chan}, C. and {Chan}, M. and {Chao}, S. and {Charlton}, P. and {Chase}, E.~A. and {Chassande-Mottin}, E. and {Chatterjee}, D. and {Chaturvedi}, M. and {Chatziioannou}, K. and {Chen}, H.~Y. and {Chen}, X. and {Chen}, Y. and {Cheng}, H. -P. and {Cheong}, C.~K. and {Chia}, H.~Y. and {Chiadini}, F. and {Chierici}, R. and {Chincarini}, A. and {Chiummo}, A. and {Cho}, G. and {Cho}, H.~S. and {Cho}, M. and {Christensen}, N. and {Chu}, Q. and {Chua}, S. and {Chung}, K.~W. and {Chung}, S. and {Ciani}, G. and {Ciecielag}, P. and {Cie{\'s}lar}, M. and {Ciobanu}, A.~A. and {Ciolfi}, R. and {Cipriano}, F. and {Cirone}, A. and {Clara}, F. and {Clark}, J.~A. and {Clearwater}, P. and {Clesse}, S. and {Cleva}, F. and {Coccia}, E. and {Cohadon}, P. -F. and {Cohen}, D. and {Colleoni}, M. and {Collette}, C.~G. and {Collins}, C. and {Colpi}, M. and {Constancio}, M., Jr. and {Conti}, L. and {Cooper}, S.~J. and {Corban}, P. and {Corbitt}, T.~R. and {Cordero-Carri{\'o}n}, I. and {Corezzi}, S. and {Corley}, K.~R. and {Cornish}, N. and {Corre}, D. and {Corsi}, A. and {Cortese}, S. and {Costa}, C.~A. and {Cotesta}, R. and {Coughlin}, M.~W. and {Coughlin}, S.~B. and {Coulon}, J. -P. and {Countryman}, S.~T. and {Couvares}, P. and {Covas}, P.~B. and {Coward}, D.~M. and {Cowart}, M.~J. and {Coyne}, D.~C. and {Coyne}, R. and {Creighton}, J.~D.~E. and {Creighton}, T.~D. and {Cripe}, J. and {Croquette}, M. and {Crowder}, S.~G. and {Cudell}, J. -R. and {Cullen}, T.~J. and {Cumming}, A. and {Cummings}, R. and {Cunningham}, L. and {Cuoco}, E. and {Curylo}, M. and {Canton}, T. Dal and {D{\'a}lya}, G. and {Dana}, A. and {Daneshgaran-Bajastani}, L.~M. and {D'Angelo}, B. and {Danilishin}, S.~L. and {D'Antonio}, S. and {Danzmann}, K. and {Darsow-Fromm}, C. and {Dasgupta}, A. and {Datrier}, L.~E.~H. and {Dattilo}, V. and {Dave}, I. and {Davier}, M. and {Davies}, G.~S. and {Davis}, D. and {Daw}, E.~J. and {DeBra}, D. and {Deenadayalan}, M. and {Degallaix}, J. and {De Laurentis}, M. and {Del{\'e}glise}, S. and {Delfavero}, M. and {De Lillo}, N. and {Del Pozzo}, W. and {DeMarchi}, L.~M. and {D'Emilio}, V. and {Demos}, N. and {Dent}, T. and {De Pietri}, R. and {De Rosa}, R. and {De Rossi}, C. and {DeSalvo}, R. and {de Varona}, O. and {Dhurandhar}, S. and {D{\'\i}az}, M.~C. and {Diaz-Ortiz}, M., Jr. and {Dietrich}, T. and {Di Fiore}, L. and {Di Fronzo}, C. and {Di Giorgio}, C. and {Di Giovanni}, F. and {Di Giovanni}, M. and {Di Girolamo}, T. and {Di Lieto}, A. and {Ding}, B. and {Di Pace}, S. and {Di Palma}, I. and {Di Renzo}, F. and {Divakarla}, A.~K. and {Dmitriev}, A. and {Doctor}, Z. and {Donovan}, F. and {Dooley}, K.~L. and {Doravari}, S. and {Dorrington}, I. and {Downes}, T.~P. and {Drago}, M. and {Driggers}, J.~C. and {Du}, Z. and {Ducoin}, J. -G. and {Dupej}, P. and {Durante}, O. and {D'Urso}, D. and {Dwyer}, S.~E. and {Easter}, P.~J. and {Eddolls}, G. and {Edelman}, B. and {Edo}, T.~B. and {Edy}, O. and {Effler}, A. and {Ehrens}, P. and {Eichholz}, J. and {Eikenberry}, S.~S. and {Eisenmann}, M. and {Eisenstein}, R.~A. and {Ejlli}, A. and {Errico}, L. and {Essick}, R.~C. and {Estelles}, H. and {Estevez}, D. and {Etienne}, Z.~B. and {Etzel}, T. and {Evans}, M. and {Evans}, T.~M. and {Ewing}, B.~E. and {Fafone}, V. and {Fairhurst}, S. and {Fan}, X. and {Farinon}, S. and {Farr}, B. and {Farr}, W.~M. and {Fauchon-Jones}, E.~J. and {Favata}, M. and {Fays}, M. and {Fazio}, M. and {Feicht}, J. and {Fejer}, M.~M. and {Feng}, F. and {Fenyvesi}, E. and {Ferguson}, D.~L. and {Fernandez-Galiana}, A. and {Ferrante}, I. and {Ferreira}, E.~C. and {Ferreira}, T.~A. and {Fidecaro}, F. and {Fiori}, I. and {Fiorucci}, D. and {Fishbach}, M. and {Fisher}, R.~P. and {Fittipaldi}, R. and {Fitz-Axen}, M. and {Fiumara}, V. and {Flaminio}, R. and {Floden}, E. and {Flynn}, E. and {Fong}, H. and {Font}, J.~A. and {Forsyth}, P.~W.~F. and {Fournier}, J. -D. and {Frasca}, S. and {Frasconi}, F. and {Frei}, Z. and {Freise}, A. and {Frey}, R. and {Frey}, V. and {Fritschel}, P. and {Frolov}, V.~V. and {Fronz{\`e}}, G. and {Fulda}, P. and {Fyffe}, M. and {Gabbard}, H.~A. and {Gadre}, B.~U. and {Gaebel}, S.~M. and {Gair}, J.~R. and {Galaudage}, S. and {Ganapathy}, D. and {Gaonkar}, S.~G. and {Garc{\'\i}a-Quir{\'o}s}, C. and {Garufi}, F. and {Gateley}, B. and {Gaudio}, S. and {Gayathri}, V. and {Gemme}, G. and {Genin}, E. and {Gennai}, A. and {George}, D. and {George}, J. and {Gergely}, L. and {Ghonge}, S. and {Ghosh}, Abhirup and {Ghosh}, Archisman and {Ghosh}, S. and {Giacomazzo}, B. and {Giaime}, J.~A. and {Giardina}, K.~D. and {Gibson}, D.~R. and {Gier}, C. and {Gill}, K. and {Glanzer}, J. and {Gniesmer}, J. and {Godwin}, P. and {Goetz}, E. and {Goetz}, R. and {Gohlke}, N. and {Goncharov}, B. and {Gonz{\'a}lez}, G. and {Gopakumar}, A. and {Gossan}, S.~E. and {Gosselin}, M. and {Gouaty}, R. and {Grace}, B. and {Grado}, A. and {Granata}, M. and {Grant}, A. and {Gras}, S. and {Grassia}, P. and {Gray}, C. and {Gray}, R. and {Greco}, G. and {Green}, A.~C. and {Green}, R. and {Gretarsson}, E.~M. and {Griggs}, H.~L. and {Grignani}, G. and {Grimaldi}, A. and {Grimm}, S.~J. and {Grote}, H. and {Grunewald}, S. and {Gruning}, P. and {Guidi}, G.~M. and {Guimaraes}, A.~R. and {Guix{\'e}}, G. and {Gulati}, H.~K. and {Guo}, Y. and {Gupta}, A. and {Gupta}, Anchal and {Gupta}, P. and {Gustafson}, E.~K. and {Gustafson}, R. and {Haegel}, L. and {Halim}, O. and {Hall}, E.~D. and {Hamilton}, E.~Z. and {Hammond}, G. and {Haney}, M. and {Hanke}, M.~M. and {Hanks}, J. and {Hanna}, C. and {Hannam}, M.~D. and {Hannuksela}, O.~A. and {Hansen}, T.~J. and {Hanson}, J. and {Harder}, T. and {Hardwick}, T. and {Haris}, K. and {Harms}, J. and {Harry}, G.~M. and {Harry}, I.~W. and {Hasskew}, R.~K. and {Haster}, C. -J. and {Haughian}, K. and {Hayes}, F.~J. and {Healy}, J. and {Heidmann}, A. and {Heintze}, M.~C. and {Heinze}, J. and {Heitmann}, H. and {Hellman}, F. and {Hello}, P. and {Hemming}, G. and {Hendry}, M. and {Heng}, I.~S. and {Hennes}, E. and {Hennig}, J. and {Heurs}, M. and {Hild}, S. and {Hinderer}, T. and {Hoback}, S.~Y. and {Hochheim}, S. and {Hofgard}, E. and {Hofman}, D. and {Holgado}, A.~M. and {Holland}, N.~A. and {Holt}, K. and {Holz}, D.~E. and {Hopkins}, P. and {Horst}, C. and {Hough}, J. and {Howell}, E.~J. and {Hoy}, C.~G. and {Huang}, Y. and {H{\"u}bner}, M.~T. and {Huerta}, E.~A. and {Huet}, D. and {Hughey}, B. and {Hui}, V. and {Husa}, S. and {Huttner}, S.~H. and {Huxford}, R. and {Huynh-Dinh}, T. and {Idzkowski}, B. and {Iess}, A. and {Inchauspe}, H. and {Ingram}, C. and {Intini}, G. and {Isac}, J. -M. and {Isi}, M. and {Iyer}, B.~R. and {Jacqmin}, T. and {Jadhav}, S.~J. and {Jadhav}, S.~P. and {James}, A.~L. and {Jani}, K. and {Janthalur}, N.~N. and {Jaranowski}, P. and {Jariwala}, D. and {Jaume}, R. and {Jenkins}, A.~C. and {Jiang}, J. and {Johns}, G.~R. and {Johnson-McDaniel}, N.~K. and {Jones}, A.~W. and {Jones}, D.~I. and {Jones}, J.~D. and {Jones}, P. and {Jones}, R. and {Jonker}, R.~J.~G. and {Ju}, L. and {Junker}, J. and {Kalaghatgi}, C.~V. and {Kalogera}, V. and {Kamai}, B. and {Kandhasamy}, S. and {Kang}, G. and {Kanner}, J.~B. and {Kapadia}, S.~J. and {Karki}, S. and {Kashyap}, R. and {Kasprzack}, M. and {Kastaun}, W. and {Katsanevas}, S. and {Katsavounidis}, E. and {Katzman}, W. and {Kaufer}, S. and {Kawabe}, K. and {K{\'e}f{\'e}lian}, F. and {Keitel}, D. and {Keivani}, A. and {Kennedy}, R. and {Key}, J.~S. and {Khadka}, S. and {Khalili}, F.~Y. and {Khan}, I. and {Khan}, S. and {Khan}, Z.~A. and {Khazanov}, E.~A. and {Khetan}, N. and {Khursheed}, M. and {Kijbunchoo}, N. and {Kim}, Chunglee and {Kim}, G.~J. and {Kim}, J.~C. and {Kim}, K. and {Kim}, W. and {Kim}, W.~S. and {Kim}, Y. -M. and {Kimball}, C. and {King}, P.~J. and {Kinley-Hanlon}, M. and {Kirchhoff}, R. and {Kissel}, J.~S. and {Kleybolte}, L. and {Klimenko}, S. and {Knowles}, T.~D. and {Knyazev}, E. and {Koch}, P. and {Koehlenbeck}, S.~M. and {Koekoek}, G. and {Koley}, S. and {Kondrashov}, V. and {Kontos}, A. and {Koper}, N. and {Korobko}, M. and {Korth}, W.~Z. and {Kovalam}, M. and {Kozak}, D.~B. and {Kringel}, V. and {Krishnendu}, N.~V. and {Kr{\'o}lak}, A. and {Krupinski}, N. and {Kuehn}, G. and {Kumar}, A. and {Kumar}, P. and {Kumar}, Rahul and {Kumar}, Rakesh and {Kumar}, S. and {Kuo}, L. and {Kutynia}, A. and {Lackey}, B.~D. and {Laghi}, D. and {Lalande}, E. and {Lam}, T.~L. and {Lamberts}, A. and {Landry}, M. and {Lane}, B.~B. and {Lang}, R.~N. and {Lange}, J. and {Lantz}, B. and {Lanza}, R.~K. and {La Rosa}, I. and {Lartaux-Vollard}, A. and {Lasky}, P.~D. and {Laxen}, M. and {Lazzarini}, A. and {Lazzaro}, C. and {Leaci}, P. and {Leavey}, S. and {Lecoeuche}, Y.~K. and {Lee}, C.~H. and {Lee}, H.~M. and {Lee}, H.~W. and {Lee}, J. and {Lee}, K. and {Lehmann}, J. and {Leroy}, N. and {Letendre}, N. and {Levin}, Y. and {Li}, A.~K.~Y. and {Li}, J. and {li}, K. and {Li}, T.~G.~F. and {Li}, X. and {Linde}, F. and {Linker}, S.~D. and {Linley}, J.~N. and {Littenberg}, T.~B. and {Liu}, J. and {Liu}, X. and {Llorens-Monteagudo}, M. and {Lo}, R.~K.~L. and {Lockwood}, A. and {London}, L.~T. and {Longo}, A. and {Lorenzini}, M. and {Loriette}, V. and {Lormand}, M. and {Losurdo}, G. and {Lough}, J.~D. and {Lousto}, C.~O. and {Lovelace}, G. and {L{\"u}ck}, H. and {Lumaca}, D. and {Lundgren}, A.~P. and {Ma}, Y. and {Macas}, R. and {Macfoy}, S. and {MacInnis}, M. and {Macleod}, D.~M. and {MacMillan}, I.~A.~O. and {Macquet}, A. and {Hernandez}, I. Maga{\~n}a and {Maga{\~n}a-Sandoval}, F. and {Magee}, R.~M. and {Majorana}, E. and {Maksimovic}, I. and {Malik}, A. and {Man}, N. and {Mandic}, V. and {Mangano}, V. and {Mansell}, G.~L. and {Manske}, M. and {Mantovani}, M. and {Mapelli}, M. and {Marchesoni}, F. and {Marion}, F. and {M{\'a}rka}, S. and {M{\'a}rka}, Z. and {Markakis}, C. and {Markosyan}, A.~S. and {Markowitz}, A. and {Maros}, E. and {Marquina}, A. and {Marsat}, S. and {Martelli}, F. and {Martin}, I.~W. and {Martin}, R.~M. and {Martinez}, V. and {Martynov}, D.~V. and {Masalehdan}, H. and {Mason}, K. and {Massera}, E. and {Masserot}, A. and {Massinger}, T.~J. and {Masso-Reid}, M. and {Mastrogiovanni}, S. and {Matas}, A. and {Matichard}, F. and {Mavalvala}, N. and {Maynard}, E. and {McCann}, J.~J. and {McCarthy}, R. and {McClelland}, D.~E. and {McCormick}, S. and {McCuller}, L. and {McGuire}, S.~C. and {McIsaac}, C. and {McIver}, J. and {McManus}, D.~J. and {McRae}, T. and {McWilliams}, S.~T. and {Meacher}, D. and {Meadors}, G.~D. and {Mehmet}, M. and {Mehta}, A.~K. and {Villa}, E. Mejuto and {Melatos}, A. and {Mendell}, G. and {Mercer}, R.~A. and {Mereni}, L. and {Merfeld}, K. and {Merilh}, E.~L. and {Merritt}, J.~D. and {Merzougui}, M. and {Meshkov}, S. and {Messenger}, C. and {Messick}, C. and {Metzdorff}, R. and {Meyers}, P.~M. and {Meylahn}, F. and {Mhaske}, A. and {Miani}, A. and {Miao}, H. and {Michaloliakos}, I. and {Michel}, C. and {Middleton}, H. and {Milano}, L. and {Miller}, A.~L. and {Millhouse}, M. and {Mills}, J.~C. and {Milotti}, E. and {Milovich-Goff}, M.~C. and {Minazzoli}, O. and {Minenkov}, Y. and {Mishkin}, A. and {Mishra}, C. and {Mistry}, T. and {Mitra}, S. and {Mitrofanov}, V.~P. and {Mitselmakher}, G. and {Mittleman}, R. and {Mo}, G. and {Mogushi}, K. and {Mohapatra}, S.~R.~P. and {Mohite}, S.~R. and {Molina-Ruiz}, M. and {Mondin}, M. and {Montani}, M. and {Moore}, C.~J. and {Moraru}, D. and {Morawski}, F. and {Moreno}, G. and {Morisaki}, S. and {Mours}, B. and {Mow-Lowry}, C.~M. and {Mozzon}, S. and {Muciaccia}, F. and {Mukherjee}, Arunava and {Mukherjee}, D. and {Mukherjee}, S. and {Mukherjee}, Subroto and {Mukund}, N. and {Mullavey}, A. and {Munch}, J. and {Mu{\~n}iz}, E.~A. and {Murray}, P.~G. and {Nagar}, A. and {Nardecchia}, I. and {Naticchioni}, L. and {Nayak}, R.~K. and {Neil}, B.~F. and {Neilson}, J. and {Nelemans}, G. and {Nelson}, T.~J.~N. and {Nery}, M. and {Neunzert}, A. and {Ng}, K.~Y. and {Ng}, S. and {Nguyen}, C. and {Nguyen}, P. and {Nichols}, D. and {Nichols}, S.~A. and {Nissanke}, S. and {Nocera}, F. and {Noh}, M. and {North}, C. and {Nothard}, D. and {Nuttall}, L.~K. and {Oberling}, J. and {O'Brien}, B.~D. and {Oganesyan}, G. and {Ogin}, G.~H. and {Oh}, J.~J. and {Oh}, S.~H. and {Ohme}, F. and {Ohta}, H. and {Okada}, M.~A. and {Oliver}, M. and {Olivetto}, C. and {Oppermann}, P. and {Oram}, Richard J. and {O'Reilly}, B. and {Ormiston}, R.~G. and {Ortega}, L.~F. and {O'Shaughnessy}, R. and {Ossokine}, S. and {Osthelder}, C. and {Ottaway}, D.~J. and {Overmier}, H. and {Owen}, B.~J. and {Pace}, A.~E. and {Pagano}, G. and {Page}, M.~A. and {Pagliaroli}, G. and {Pai}, A. and {Pai}, S.~A. and {Palamos}, J.~R. and {Palashov}, O. and {Palomba}, C. and {Pan}, H. and {Panda}, P.~K. and {Pang}, P.~T.~H. and {Pankow}, C. and {Pannarale}, F. and {Pant}, B.~C. and {Paoletti}, F. and {Paoli}, A. and {Parida}, A. and {Parker}, W. and {Pascucci}, D. and {Pasqualetti}, A. and {Passaquieti}, R. and {Passuello}, D. and {Patricelli}, B. and {Payne}, E. and {Pearlstone}, B.~L. and {Pechsiri}, T.~C. and {Pedersen}, A.~J. and {Pedraza}, M. and {Pele}, A. and {Penn}, S. and {Perego}, A. and {Perez}, C.~J. and {P{\'e}rigois}, C. and {Perreca}, A. and {Perri{\`e}s}, S. and {Petermann}, J. and {Pfeiffer}, H.~P. and {Phelps}, M. and {Phukon}, K.~S. and {Piccinni}, O.~J. and {Pichot}, M. and {Piendibene}, M. and {Piergiovanni}, F. and {Pierro}, V. and {Pillant}, G. and {Pinard}, L. and {Pinto}, I.~M. and {Piotrzkowski}, K. and {Pirello}, M. and {Pitkin}, M. and {Plastino}, W. and {Poggiani}, R. and {Pong}, D.~Y.~T. and {Ponrathnam}, S. and {Popolizio}, P. and {Porter}, E.~K. and {Powell}, J. and {Prajapati}, A.~K. and {Prasai}, K. and {Prasanna}, R. and {Pratten}, G. and {Prestegard}, T. and {Principe}, M. and {Prodi}, G.~A. and {Prokhorov}, L. and {Punturo}, M. and {Puppo}, P. and {P{\"u}rrer}, M. and {Qi}, H. and {Quetschke}, V. and {Quinonez}, P.~J. and {Raab}, F.~J. and {Raaijmakers}, G. and {Radkins}, H. and {Radulesco}, N. and {Raffai}, P. and {Rafferty}, H. and {Raja}, S. and {Rajan}, C. and {Rajbhandari}, B. and {Rakhmanov}, M. and {Ramirez}, K.~E. and {Ramos-Buades}, A. and {Rana}, Javed and {Rao}, K. and {Rapagnani}, P. and {Raymond}, V. and {Razzano}, M. and {Read}, J. and {Regimbau}, T. and {Rei}, L. and {Reid}, S. and {Reitze}, D.~H. and {Rettegno}, P. and {Ricci}, F. and {Richardson}, C.~J. and {Richardson}, J.~W. and {Ricker}, P.~M. and {Riemenschneider}, G. and {Riles}, K. and {Rizzo}, M. and {Robertson}, N.~A. and {Robinet}, F. and {Rocchi}, A. and {Rodriguez-Soto}, R.~D. and {Rolland}, L. and {Rollins}, J.~G. and {Roma}, V.~J. and {Romanelli}, M. and {Romano}, R. and {Romel}, C.~L. and {Romero-Shaw}, I.~M. and {Romie}, J.~H. and {Rose}, C.~A. and {Rose}, D. and {Rose}, K. and {Rosi{\'n}ska}, D. and {Rosofsky}, S.~G. and {Ross}, M.~P. and {Rowan}, S. and {Rowlinson}, S.~J. and {Roy}, P.~K. and {Roy}, Santosh and {Roy}, Soumen and {Ruggi}, P. and {Rutins}, G. and {Ryan}, K. and {Sachdev}, S. and {Sadecki}, T. and {Sakellariadou}, M. and {Salafia}, O.~S. and {Salconi}, L. and {Saleem}, M. and {Samajdar}, A. and {Sanchez}, E.~J. and {Sanchez}, L.~E. and {Sanchis-Gual}, N. and {Sanders}, J.~R. and {Santiago}, K.~A. and {Santos}, E. and {Sarin}, N. and {Sassolas}, B. and {Sathyaprakash}, B.~S. and {Sauter}, O. and {Savage}, R.~L. and {Savant}, V. and {Sawant}, D. and {Sayah}, S. and {Schaetzl}, D. and {Schale}, P. and {Scheel}, M. and {Scheuer}, J. and {Schmidt}, P. and {Schnabel}, R. and {Schofield}, R.~M.~S. and {Sch{\"o}nbeck}, A. and {Schreiber}, E. and {Schulte}, B.~W. and {Schutz}, B.~F. and {Schwarm}, O. and {Schwartz}, E. and {Scott}, J. and {Scott}, S.~M. and {Seidel}, E. and {Sellers}, D. and {Sengupta}, A.~S. and {Sennett}, N. and {Sentenac}, D. and {Sequino}, V. and {Sergeev}, A. and {Setyawati}, Y. and {Shaddock}, D.~A. and {Shaffer}, T. and {Shahriar}, M.~S. and {Sharifi}, S. and {Sharma}, A. and {Sharma}, P. and {Shawhan}, P. and {Shen}, H. and {Shikauchi}, M. and {Shink}, R. and {Shoemaker}, D.~H. and {Shoemaker}, D.~M. and {Shukla}, K. and {ShyamSundar}, S. and {Siellez}, K. and {Sieniawska}, M. and {Sigg}, D. and {Singer}, L.~P. and {Singh}, D. and {Singh}, N. and {Singha}, A. and {Singhal}, A. and {Sintes}, A.~M. and {Sipala}, V. and {Skliris}, V. and {Slagmolen}, B.~J.~J. and {Slaven-Blair}, T.~J. and {Smetana}, J. and {Smith}, J.~R. and {Smith}, R.~J.~E. and {Somala}, S. and {Son}, E.~J. and {Soni}, S. and {Sorazu}, B. and {Sordini}, V. and {Sorrentino}, F. and {Souradeep}, T. and {Sowell}, E. and {Spencer}, A.~P. and {Spera}, M. and {Srivastava}, A.~K. and {Srivastava}, V. and {Staats}, K. and {Stachie}, C. and {Standke}, M. and {Steer}, D.~A. and {Steinke}, M. and {Steinlechner}, J. and {Steinlechner}, S. and {Steinmeyer}, D. and {Stevenson}, S. and {Stocks}, D. and {Stops}, D.~J. and {Stover}, M. and {Strain}, K.~A. and {Stratta}, G. and {Strunk}, A. and {Sturani}, R. and {Stuver}, A.~L. and {Sudhagar}, S. and {Sudhir}, V. and {Summerscales}, T.~Z. and {Sun}, L. and {Sunil}, S. and {Sur}, A. and {Suresh}, J. and {Sutton}, P.~J. and {Swinkels}, B.~L. and {Szczepa{\'n}czyk}, M.~J. and {Tacca}, M. and {Tait}, S.~C. and {Talbot}, C. and {Tanasijczuk}, A.~J. and {Tanner}, D.~B. and {Tao}, D. and {T{\'a}pai}, M. and {Tapia}, A. and {San Martin}, E.~N. Tapia and {Tasson}, J.~D. and {Taylor}, R. and {Tenorio}, R. and {Terkowski}, L. and {Thirugnanasambandam}, M.~P. and {Thomas}, M. and {Thomas}, P. and {Thompson}, J.~E. and {Thondapu}, S.~R. and {Thorne}, K.~A. and {Thrane}, E. and {Tinsman}, C.~L. and {Saravanan}, T.~R. and {Tiwari}, Shubhanshu and {Tiwari}, S. and {Tiwari}, V. and {Toland}, K. and {Tonelli}, M. and {Tornasi}, Z. and {Torres-Forn{\'e}}, A. and {Torrie}, C.~I. and {Tosta e Melo}, I. and {T{\"o}yr{\"a}}, D. and {Trail}, E.~A. and {Travasso}, F. and {Traylor}, G. and {Tringali}, M.~C. and {Tripathee}, A. and {Trovato}, A. and {Trudeau}, R.~J. and {Tsang}, K.~W. and {Tse}, M. and {Tso}, R. and {Tsukada}, L. and {Tsuna}, D. and {Tsutsui}, T. and {Turconi}, M. and {Ubhi}, A.~S. and {Udall}, R. and {Ueno}, K. and {Ugolini}, D. and {Unnikrishnan}, C.~S. and {Urban}, A.~L. and {Usman}, S.~A. and {Utina}, A.~C. and {Vahlbruch}, H. and {Vajente}, G. and {Valdes}, G. and {Valentini}, M. and {van Bakel}, N. and {van Beuzekom}, M. and {van den Brand}, J.~F.~J. and {Van Den Broeck}, C. Den and {Vander-Hyde}, D.~C. and {van der Schaaf}, L. and {Van Heijningen}, J.~V. and {van Veggel}, A.~A. and {Vardaro}, M. and {Varma}, V. and {Vass}, S. and {Vas{\'u}th}, M. and {Vecchio}, A. and {Vedovato}, G. and {Veitch}, J. and {Veitch}, P.~J. and {Venkateswara}, K. and {Venugopalan}, G. and {Verkindt}, D. and {Veske}, D. and {Vetrano}, F. and {Vicer{\'e}}, A. and {Viets}, A.~D. and {Vinciguerra}, S. and {Vine}, D.~J. and {Vinet}, J. -Y. and {Vitale}, S. and {Vivanco}, Francisco Hernandez and {Vo}, T. and {Vocca}, H. and {Vorvick}, C. and {Vyatchanin}, S.~P. and {Wade}, A.~R. and {Wade}, L.~E. and {Wade}, M. and {Walet}, R. and {Walker}, M. and {Wallace}, G.~S. and {Wallace}, L. and {Walsh}, S. and {Wang}, J.~Z. and {Wang}, S. and {Wang}, W.~H. and {Ward}, R.~L. and {Warden}, Z.~A. and {Warner}, J. and {Was}, M. and {Watchi}, J. and {Weaver}, B. and {Wei}, L. -W. and {Weinert}, M. and {Weinstein}, A.~J. and {Weiss}, R. and {Wellmann}, F. and {Wen}, L. and {We{\ss}els}, P. and {Westhouse}, J.~W. and {Wette}, K. and {Whelan}, J.~T. and {Whiting}, B.~F. and {Whittle}, C. and {Wilken}, D.~M. and {Williams}, D. and {Willis}, J.~L. and {Willke}, B. and {Winkler}, W. and {Wipf}, C.~C. and {Wittel}, H. and {Woan}, G. and {Woehler}, J. and {Wofford}, J.~K. and {Wong}, C. and {Wright}, J.~L. and {Wu}, D.~S. and {Wysocki}, D.~M. and {Xiao}, L. and {Yamamoto}, H. and {Yang}, L. and {Yang}, Y. and {Yang}, Z. and {Yap}, M.~J. and {Yazback}, M. and {Yeeles}, D.~W. and {Yu}, Hang and {Yu}, Haocun and {Yuen}, S.~H.~R. and {Zadro{\.z}ny}, A.~K. and {Zadro{\.z}ny}, A. and {Zanolin}, M. and {Zelenova}, T. and {Zendri}, J. -P. and {Zevin}, M. and {Zhang}, J. and {Zhang}, L. and {Zhang}, T. and {Zhao}, C. and {Zhao}, G. and {Zhou}, M. and {Zhou}, Z. and {Zhu}, X.~J. and {Zimmerman}, A.~B. and {Zlochower}, Y. and {Zucker}, M.~E. and {Zweizig}, J. and {LIGO Scientific Collaboration} and {Virgo Collaboration}},
        title = "{Properties and Astrophysical Implications of the 150 M$_{{\ensuremath{\odot}}}$ Binary Black Hole Merger GW190521}",
      journal = {\apjl},
     keywords = {Astrophysical black holes, High energy astrophysics, Gravitational collapse, Gravitation, Gravitational wave astronomy, Gravitational wave sources, LIGO, Stellar mass black holes, Stellar populations, Intermediate-mass black holes, 98, 739, 662, 661, 675, 677, 920, 611, 1622, 816, Astrophysics - High Energy Astrophysical Phenomena, General Relativity and Quantum Cosmology},
         year = 2020,
        month = sep,
       volume = {900},
       number = {1},
          eid = {L13},
        pages = {L13},
          doi = {10.3847/2041-8213/aba493},
archivePrefix = {arXiv},
       eprint = {2009.01190},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...900L..13A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Agrawal2022,
       author = {{Agrawal}, Poojan and {Sz{\'e}csi}, Dorottya and {Stevenson}, Simon and {Eldridge}, Jan J. and {Hurley}, Jarrod},
        title = "{Explaining the differences in massive star models from various simulations}",
      journal = {\mnras},
     keywords = {gravitational waves, stars: evolution, stars: formation, stars: massive, galaxies: stellar content, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = jun,
       volume = {512},
       number = {4},
        pages = {5717-5725},
          doi = {10.1093/mnras/stac930},
archivePrefix = {arXiv},
       eprint = {2112.02800},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.512.5717A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Addari2024,
       author = {{Addari}, Francesco and {Marigo}, Paola and {Bressan}, Alessandro and {Costa}, Guglielmo and {Shepherd}, Kendall and {Volpato}, Guglielmo},
        title = "{The Role of the Third Dredge-up and Mass Loss in Shaping the Initial{\textendash}Final Mass Relation of White Dwarfs}",
      journal = {\apj},
     keywords = {Asymptotic giant branch stars, Carbon stars, White dwarf stars, Stellar winds, Stellar convective zones, 2100, 199, 1799, 1636, 301, Astrophysics - Solar and Stellar Astrophysics},
         year = 2024,
        month = mar,
       volume = {964},
       number = {1},
          eid = {51},
        pages = {51},
          doi = {10.3847/1538-4357/ad2067},
archivePrefix = {arXiv},
       eprint = {2401.09812},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024ApJ...964...51A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Bohm-Vitense1958,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {{B{\"{o}}hm-Vitense}, E.},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
isbn = {9788578110796},
issn = {1098-6596},
journal = {\zap},
pages = {108},
pmid = {25246403},
title = "{{{\{}{\"{U}}{\}}ber die Wasserstoffkonvektionszone in Sternen verschiedener Effektivtemperaturen und Leuchtkr{\{}{\"{a}}{\}}fte. Mit 5 Textabbildungen}}",
url = {https://ui.adsabs.harvard.edu//?bbbRedirect=1{\#}abs/1958ZA.....46..108B/abstract},
volume = {46},
year = {1958}
}

@ARTICLE{Bressan2012,
       author = {{Bressan}, Alessandro and {Marigo}, Paola and {Girardi}, L{\'e}o. and {Salasnich}, Bernardo and {Dal Cero}, Claudia and {Rubele}, Stefano and {Nanni}, Ambra},
        title = "{PARSEC: stellar tracks and isochrones with the PAdova and TRieste Stellar Evolution Code}",
      journal = {\mnras},
     keywords = {stars: evolution, Hertzsprung{\ensuremath{-}}Russell and colour magnitude diagrams, stars: interiors, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = nov,
       volume = {427},
       number = {1},
        pages = {127-145},
          doi = {10.1111/j.1365-2966.2012.21948.x},
archivePrefix = {arXiv},
       eprint = {1208.4498},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.427..127B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bertelli1984,
       author = {{Bertelli}, G. and {Bressan}, A.~G. and {Chiosi}, C.},
        title = "{The HR diagram of massive stars : widening of the main sequence band and WR formation.}",
      journal = {\aap},
     keywords = {Hertzsprung-Russell Diagram, Main Sequence Stars, Stellar Evolution, Supergiant Stars, Wolf-Rayet Stars, Stellar Luminosity, Stellar Spectra, Stellar Temperature, Stellar Winds, Astrophysics},
         year = 1984,
        month = jan,
       volume = {130},
        pages = {279-293},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1984A&A...130..279B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Bressan1981,
       author = {{Bressan}, A.~G. and {Chiosi}, C. and {Bertelli}, G.},
        title = "{Mass loss and overshooting in massive stars}",
      journal = {\aap},
     keywords = {Astrophysics, Stellar Evolution, Stellar Mass Ejection, Supermassive Stars, Hertzsprung-Russell Diagram, Mixing Length Flow Theory, Stellar Models, Stellar Winds, Supergiant Stars, Astrophysics},
         year = 1981,
        month = sep,
       volume = {102},
       number = {1},
        pages = {25-30},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1981A&A...102...25B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Bromm2004,
       author = {{Bromm}, Volker and {Larson}, Richard B.},
        title = "{The First Stars}",
      journal = {\araa},
     keywords = {Astrophysics},
         year = 2004,
        month = sep,
       volume = {42},
       number = {1},
        pages = {79-118},
          doi = {10.1146/annurev.astro.42.053102.134034},
archivePrefix = {arXiv},
       eprint = {astro-ph/0311019},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ARA&A..42...79B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Becker2013,
       author = {{Becker}, George D. and {Bolton}, James S.},
        title = "{New measurements of the ionizing ultraviolet background over 2 < z < 5 and implications for hydrogen reionization}",
      journal = {\mnras},
     keywords = {galaxies: high-redshift, intergalactic medium, quasars: absorption lines, cosmic background radiation, cosmology: observations, dark ages, reionization, first stars, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = dec,
       volume = {436},
       number = {2},
        pages = {1023-1039},
          doi = {10.1093/mnras/stt1610},
archivePrefix = {arXiv},
       eprint = {1307.2259},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.436.1023B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bestenlehner2020,
       author = {{Bestenlehner}, Joachim M. and {Crowther}, Paul A. and {Caballero-Nieves}, Saida M. and {Schneider}, Fabian R.~N. and {Sim{\'o}n-D{\'\i}az}, Sergio and {Brands}, Sarah A. and {de Koter}, Alex and {Gr{\"a}fener}, G{\"o}tz and {Herrero}, Artemio and {Langer}, Norbert and {Lennon}, Daniel J. and {Ma{\'\i}z Apell{\'a}niz}, Jesus and {Puls}, Joachim and {Vink}, Jorick S.},
        title = "{The R136 star cluster dissected with Hubble Space Telescope/STIS - II. Physical properties of the most massive stars in R136}",
      journal = {\mnras},
     keywords = {stars: early-type, stars: evolution, stars: fundamental parameters, stars: massive, galaxies: clusters: individual: R136, Magellanic Clouds, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = dec,
       volume = {499},
       number = {2},
        pages = {1918-1936},
          doi = {10.1093/mnras/staa2801},
archivePrefix = {arXiv},
       eprint = {2009.05136},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.499.1918B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Brands2022,
       author = {{Brands}, Sarah A. and {de Koter}, Alex and {Bestenlehner}, Joachim M. and {Crowther}, Paul A. and {Sundqvist}, Jon O. and {Puls}, Joachim and {Caballero-Nieves}, Saida M. and {Abdul-Masih}, Michael and {Driessen}, Florian A. and {Garc{\'\i}a}, Miriam and {Geen}, Sam and {Gr{\"a}fener}, G{\"o}tz and {Hawcroft}, Calum and {Kaper}, Lex and {Keszthelyi}, Zsolt and {Langer}, Norbert and {Sana}, Hugues and {Schneider}, Fabian R.~N. and {Shenar}, Tomer and {Vink}, Jorick S.},
        title = "{The R136 star cluster dissected with Hubble Space Telescope/STIS. III. The most massive stars and their clumped winds}",
      journal = {\aap},
     keywords = {stars: massive, stars: mass-loss, stars: winds, outflows, stars: fundamental parameters, Magellanic Clouds, galaxies: star clusters: individual: R136, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = jul,
       volume = {663},
          eid = {A36},
        pages = {A36},
          doi = {10.1051/0004-6361/202142742},
archivePrefix = {arXiv},
       eprint = {2202.11080},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A&A...663A..36B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Bressan2023,
       author = {{Bressan}, A. and {Costa}, G. and {Goswami}, S. and {Grisoni}, V. and {Shepherd}, K.~G. and {Silva}, L. and {Addari}, F. and {Marigo}, P.},
        title = "{Very massive stars chemical enrichment in extremely metal-poor galaxies}",
     keywords = {Stars: abundances, Stars: massive, Stars: rotation, Stars: Population III, Galaxy: abundances, galaxies: starburst, galaxies: formation},
    booktitle = {Memorie della Societa Astronomica Italiana},
         year = 2023,
       volume = {94},
        month = sep,
        pages = {91},
          doi = {10.36116/MEMSAIT_94N2.2023.91},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023MmSAI..94b..91B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bellm2019,
       author = {{Bellm}, Eric C. and {Kulkarni}, Shrinivas R. and {Graham}, Matthew J. and {Dekany}, Richard and {Smith}, Roger M. and {Riddle}, Reed and {Masci}, Frank J. and {Helou}, George and {Prince}, Thomas A. and {Adams}, Scott M. and {Barbarino}, C. and {Barlow}, Tom and {Bauer}, James and {Beck}, Ron and {Belicki}, Justin and {Biswas}, Rahul and {Blagorodnova}, Nadejda and {Bodewits}, Dennis and {Bolin}, Bryce and {Brinnel}, Valery and {Brooke}, Tim and {Bue}, Brian and {Bulla}, Mattia and {Burruss}, Rick and {Cenko}, S. Bradley and {Chang}, Chan-Kao and {Connolly}, Andrew and {Coughlin}, Michael and {Cromer}, John and {Cunningham}, Virginia and {De}, Kishalay and {Delacroix}, Alex and {Desai}, Vandana and {Duev}, Dmitry A. and {Eadie}, Gwendolyn and {Farnham}, Tony L. and {Feeney}, Michael and {Feindt}, Ulrich and {Flynn}, David and {Franckowiak}, Anna and {Frederick}, S. and {Fremling}, C. and {Gal-Yam}, Avishay and {Gezari}, Suvi and {Giomi}, Matteo and {Goldstein}, Daniel A. and {Golkhou}, V. Zach and {Goobar}, Ariel and {Groom}, Steven and {Hacopians}, Eugean and {Hale}, David and {Henning}, John and {Ho}, Anna Y.~Q. and {Hover}, David and {Howell}, Justin and {Hung}, Tiara and {Huppenkothen}, Daniela and {Imel}, David and {Ip}, Wing-Huen and {Ivezi{\'c}}, {\v{Z}}eljko and {Jackson}, Edward and {Jones}, Lynne and {Juric}, Mario and {Kasliwal}, Mansi M. and {Kaspi}, S. and {Kaye}, Stephen and {Kelley}, Michael S.~P. and {Kowalski}, Marek and {Kramer}, Emily and {Kupfer}, Thomas and {Landry}, Walter and {Laher}, Russ R. and {Lee}, Chien-De and {Lin}, Hsing Wen and {Lin}, Zhong-Yi and {Lunnan}, Ragnhild and {Giomi}, Matteo and {Mahabal}, Ashish and {Mao}, Peter and {Miller}, Adam A. and {Monkewitz}, Serge and {Murphy}, Patrick and {Ngeow}, Chow-Choong and {Nordin}, Jakob and {Nugent}, Peter and {Ofek}, Eran and {Patterson}, Maria T. and {Penprase}, Bryan and {Porter}, Michael and {Rauch}, Ludwig and {Rebbapragada}, Umaa and {Reiley}, Dan and {Rigault}, Mickael and {Rodriguez}, Hector and {van Roestel}, Jan and {Rusholme}, Ben and {van Santen}, Jakob and {Schulze}, S. and {Shupe}, David L. and {Singer}, Leo P. and {Soumagnac}, Maayane T. and {Stein}, Robert and {Surace}, Jason and {Sollerman}, Jesper and {Szkody}, Paula and {Taddia}, F. and {Terek}, Scott and {Van Sistine}, Angela and {van Velzen}, Sjoert and {Vestrand}, W. Thomas and {Walters}, Richard and {Ward}, Charlotte and {Ye}, Quan-Zhi and {Yu}, Po-Chieh and {Yan}, Lin and {Zolkower}, Jeffry},
        title = "{The Zwicky Transient Facility: System Overview, Performance, and First Results}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = jan,
       volume = {131},
       number = {995},
        pages = {018002},
          doi = {10.1088/1538-3873/aaecbe},
archivePrefix = {arXiv},
       eprint = {1902.01932},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PASP..131a8002B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


% -------------------------- C --------------------------
@ARTICLE{Crowther2010,
       author = {{Crowther}, Paul A. and {Schnurr}, Olivier and {Hirschi}, Raphael and {Yusof}, Norhasliza and {Parker}, Richard J. and {Goodwin}, Simon P. and {Kassim}, Hasan Abu},
        title = "{The R136 star cluster hosts several stars whose individual masses greatly exceed the accepted 150M$_{solar}$ stellar mass limit}",
      journal = {\mnras},
     keywords = {binaries: general, stars: early-type, stars: fundamental parameters, stars: Wolf-Rayet, galaxies: star clusters: individual: R136, galaxies: star clusters: individual: NGC 3603, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Galaxy Astrophysics},
         year = 2010,
        month = oct,
       volume = {408},
       number = {2},
        pages = {731-751},
          doi = {10.1111/j.1365-2966.2010.17167.x},
archivePrefix = {arXiv},
       eprint = {1007.3284},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.408..731C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cyburt2010,
       author = {{Cyburt}, Richard H. and {Amthor}, A. Matthew and {Ferguson}, Ryan and {Meisel}, Zach and {Smith}, Karl and {Warren}, Scott and {Heger}, Alexander and {Hoffman}, R.~D. and {Rauscher}, Thomas and {Sakharuk}, Alexander and {Schatz}, Hendrik and {Thielemann}, F.~K. and {Wiescher}, Michael},
        title = "{The JINA REACLIB Database: Its Recent Updates and Impact on Type-I X-ray Bursts}",
      journal = {\apjs},
     keywords = {nuclear reactions, nucleosynthesis, abundances, X-rays: bursts},
         year = 2010,
        month = jul,
       volume = {189},
       number = {1},
        pages = {240-252},
          doi = {10.1088/0067-0049/189/1/240},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJS..189..240C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Caffau2011,
       author = {{Caffau}, E. and {Ludwig}, H. -G. and {Steffen}, M. and {Freytag}, B. and {Bonifacio}, P.},
        title = "{Solar Chemical Abundances Determined with a CO5BOLD 3D Model Atmosphere}",
      journal = {\solphys},
     keywords = {Sun: abundances, Sun: photosphere, Line: formation, Hydrodynamics, Convection, Radiative transfer, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = feb,
       volume = {268},
       number = {2},
        pages = {255-269},
          doi = {10.1007/s11207-010-9541-4},
archivePrefix = {arXiv},
       eprint = {1003.1190},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011SoPh..268..255C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Chen2015,
       author = {{Chen}, Yang and {Bressan}, Alessandro and {Girardi}, L{\'e}o and {Marigo}, Paola and {Kong}, Xu and {Lanza}, Antonio},
        title = "{PARSEC evolutionary tracks of massive stars up to 350 M$_{{\ensuremath{\odot}}}$ at metallicities 0.0001 {\ensuremath{\leq}} Z {\ensuremath{\leq}} 0.04}",
      journal = {\mnras},
     keywords = {stars: evolution, Hertzsprung-Russell and colour-magnitude diagrams, stars: massive, stars: mass-loss, supergiants, stars: Wolf-Rayet, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = sep,
       volume = {452},
       number = {1},
        pages = {1068-1080},
          doi = {10.1093/mnras/stv1281},
archivePrefix = {arXiv},
       eprint = {1506.01681},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.452.1068C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Costa2019a,
       author = {{Costa}, Guglielmo and {Girardi}, L{\'e}o and {Bressan}, Alessandro and {Marigo}, Paola and {Rodrigues}, Tha{\'\i}se S. and {Chen}, Yang and {Lanza}, Antonio and {Goudfrooij}, Paul},
        title = "{Mixing by overshooting and rotation in intermediate-mass stars}",
      journal = {\mnras},
     keywords = {convection, binaries: eclipsing, stars: evolution, stars: fundamental parameters, stars: interiors, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = jun,
       volume = {485},
       number = {4},
        pages = {4641-4657},
          doi = {10.1093/mnras/stz728},
archivePrefix = {arXiv},
       eprint = {1903.04368},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.485.4641C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Costa2021,
       author = {{Costa}, Guglielmo and {Bressan}, Alessandro and {Mapelli}, Michela and {Marigo}, Paola and {Iorio}, Giuliano and {Spera}, Mario},
        title = "{Formation of GW190521 from stellar evolution: the impact of the hydrogen-rich envelope, dredge-up, and $^{12}$C({\ensuremath{\alpha}}, {\ensuremath{\gamma}})$^{16}$O rate on the pair-instability black hole mass gap}",
      journal = {\mnras},
     keywords = {convection, stars: black holes, stars: evolution, stars: interiors, stars: massive, stars: mass-loss, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = mar,
       volume = {501},
       number = {3},
        pages = {4514-4533},
          doi = {10.1093/mnras/staa3916},
archivePrefix = {arXiv},
       eprint = {2010.02242},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.501.4514C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Costa2019b,
       author = {{Costa}, Guglielmo and {Girardi}, L{\'e}o and {Bressan}, Alessandro and {Chen}, Yang and {Goudfrooij}, Paul and {Marigo}, Paola and {Rodrigues}, Tha{\'\i}se S. and {Lanza}, Antonio},
        title = "{Multiple stellar populations in NGC 1866. New clues from Cepheids and colour-magnitude diagram}",
      journal = {\aap},
     keywords = {Hertzsprung-Russell and C-M diagrams, stars: evolution, stars: rotation, stars: variables: Cepheids, galaxies: star clusters: individual: NGC 1866, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = nov,
       volume = {631},
          eid = {A128},
        pages = {A128},
          doi = {10.1051/0004-6361/201936409},
archivePrefix = {arXiv},
       eprint = {1909.01907},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...631A.128C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Costa2022,
       author = {{Costa}, Guglielmo and {Ballone}, Alessandro and {Mapelli}, Michela and {Bressan}, Alessandro},
        title = "{Formation of black holes in the pair-instability mass gap: Evolution of a post-collision star}",
      journal = {\mnras},
     keywords = {black hole physics, stars: black holes, stars: evolution, stars: massive, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2022,
        month = oct,
       volume = {516},
       number = {1},
        pages = {1072-1080},
          doi = {10.1093/mnras/stac2222},
archivePrefix = {arXiv},
       eprint = {2204.03492},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.516.1072C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Chieffi2013,
       author = {{Chieffi}, Alessandro and {Limongi}, Marco},
        title = "{Pre-supernova Evolution of Rotating Solar Metallicity Stars in the Mass Range 13-120 M $_{{\ensuremath{\odot}}}$ and their Explosive Yields}",
      journal = {\apj},
     keywords = {stars: evolution, stars: interiors, stars: massive, stars: rotation, supernovae: general},
         year = 2013,
        month = feb,
       volume = {764},
       number = {1},
          eid = {21},
        pages = {21},
          doi = {10.1088/0004-637X/764/1/21},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...764...21C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Chen2014,
       author = {{Chen}, Yang and {Girardi}, L{\'e}o and {Bressan}, Alessandro and {Marigo}, Paola and {Barbieri}, Mauro and {Kong}, Xu},
        title = "{Improving PARSEC models for very low mass stars}",
      journal = {\mnras},
     keywords = {stars: evolution, Hertzsprung-Russell and colour-magnitude diagrams, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = nov,
       volume = {444},
       number = {3},
        pages = {2525-2543},
          doi = {10.1093/mnras/stu1605},
archivePrefix = {arXiv},
       eprint = {1409.0322},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.444.2525C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Choi2016,
       author = {{Choi}, Jieun and {Dotter}, Aaron and {Conroy}, Charlie and {Cantiello}, Matteo and {Paxton}, Bill and {Johnson}, Benjamin D.},
        title = "{Mesa Isochrones and Stellar Tracks (MIST). I. Solar-scaled Models}",
      journal = {\apj},
     keywords = {stars: evolution, stars: general, stars: interiors, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = jun,
       volume = {823},
       number = {2},
          eid = {102},
        pages = {102},
          doi = {10.3847/0004-637X/823/2/102},
archivePrefix = {arXiv},
       eprint = {1604.08592},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...823..102C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Chen2019,
       author = {{Chen}, Yang and {Girardi}, L{\'e}o and {Fu}, Xiaoting and {Bressan}, Alessandro and {Aringer}, Bernhard and {Dal Tio}, Piero and {Pastorelli}, Giada and {Marigo}, Paola and {Costa}, Guglielmo and {Zhang}, Xing},
        title = "{YBC: a stellar bolometric corrections database with variable extinction coefficients. Application to PARSEC isochrones}",
      journal = {\aap},
     keywords = {Hertzsprung-Russell and C-M diagrams, astronomical databases: miscellaneous, dust, extinction, open clusters and associations: individual: NGC 2425, open clusters and associations: individual: Mellotte 22, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = dec,
       volume = {632},
          eid = {A105},
        pages = {A105},
          doi = {10.1051/0004-6361/201936612},
archivePrefix = {arXiv},
       eprint = {1910.09037},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...632A.105C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


% -------------------------- D --------------------------
@ARTICLE{deJager1988,
       author = {{de Jager}, C. and {Nieuwenhuijden}, H. and {van der Hucht}, K.~A.},
        title = "{Mass Loss Rates in the Hertzprung-Russell Diagram}",
      journal = {Bulletin d'Information du Centre de Donnees Stellaires},
         year = 1988,
        month = dec,
       volume = {35},
        pages = {141},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988BICDS..35..141D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{deMink2014,
       author = {{de Mink}, S.~E. and {Sana}, H. and {Langer}, N. and {Izzard}, R.~G. and {Schneider}, F.~R.~N.},
        title = "{The Incidence of Stellar Mergers and Mass Gainers among Massive Stars}",
      journal = {\apj},
     keywords = {binaries: close, Galaxy: stellar content, stars: early-type, stars: massive, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = feb,
       volume = {782},
       number = {1},
          eid = {7},
        pages = {7},
          doi = {10.1088/0004-637X/782/1/7},
archivePrefix = {arXiv},
       eprint = {1312.3650},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...782....7D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{DiCarlo2019,
       author = {{Di Carlo}, Ugo N. and {Giacobbo}, Nicola and {Mapelli}, Michela and {Pasquato}, Mario and {Spera}, Mario and {Wang}, Long and {Haardt}, Francesco},
        title = "{Merging black holes in young star clusters}",
      journal = {\mnras},
     keywords = {black hole physics, gravitational waves, methods: numerical, binaries: general, stars: kinematics and dynamics, galaxies: star clusters: general, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = aug,
       volume = {487},
       number = {2},
        pages = {2947-2960},
          doi = {10.1093/mnras/stz1453},
archivePrefix = {arXiv},
       eprint = {1901.00863},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.487.2947D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{DeLuca2021,
       author = {{De Luca}, V. and {Desjacques}, V. and {Franciolini}, G. and {Pani}, P. and {Riotto}, A.},
        title = "{GW190521 Mass Gap Event and the Primordial Black Hole Scenario}",
      journal = {\prl},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Phenomenology},
         year = 2021,
        month = feb,
       volume = {126},
       number = {5},
          eid = {051101},
        pages = {051101},
          doi = {10.1103/PhysRevLett.126.051101},
archivePrefix = {arXiv},
       eprint = {2009.01728},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021PhRvL.126e1101D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


% -------------------------- E --------------------------
@ARTICLE{Eggenberger2008,
       author = {{Eggenberger}, P. and {Meynet}, G. and {Maeder}, A. and {Hirschi}, R. and {Charbonnel}, C. and {Talon}, S. and {Ekstr{\"o}m}, S.},
        title = "{The Geneva stellar evolution code}",
      journal = {\apss},
     keywords = {Stars: evolution},
         year = 2008,
        month = aug,
       volume = {316},
       number = {1-4},
        pages = {43-54},
          doi = {10.1007/s10509-007-9511-y},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008Ap&SS.316...43E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Evans2011,
       author = {{Evans}, C.~J. and {Taylor}, W.~D. and {H{\'e}nault-Brunet}, V. and {Sana}, H. and {de Koter}, A. and {Sim{\'o}n-D{\'\i}az}, S. and {Carraro}, G. and {Bagnoli}, T. and {Bastian}, N. and {Bestenlehner}, J.~M. and {Bonanos}, A.~Z. and {Bressert}, E. and {Brott}, I. and {Campbell}, M.~A. and {Cantiello}, M. and {Clark}, J.~S. and {Costa}, E. and {Crowther}, P.~A. and {de Mink}, S.~E. and {Doran}, E. and {Dufton}, P.~L. and {Dunstall}, P.~R. and {Friedrich}, K. and {Garcia}, M. and {Gieles}, M. and {Gr{\"a}fener}, G. and {Herrero}, A. and {Howarth}, I.~D. and {Izzard}, R.~G. and {Langer}, N. and {Lennon}, D.~J. and {Ma{\'\i}z Apell{\'a}niz}, J. and {Markova}, N. and {Najarro}, F. and {Puls}, J. and {Ramirez}, O.~H. and {Sab{\'\i}n-Sanjuli{\'a}n}, C. and {Smartt}, S.~J. and {Stroud}, V.~E. and {van Loon}, J. Th. and {Vink}, J.~S. and {Walborn}, N.~R.},
        title = "{The VLT-FLAMES Tarantula Survey. I. Introduction and observational overview}",
      journal = {\aap},
     keywords = {open clusters and associations: individual: 30 Doradus, stars: early-type, stars: fundamental parameters, binaries: spectroscopic, stars: Wolf-Rayet, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = jun,
       volume = {530},
          eid = {A108},
        pages = {A108},
          doi = {10.1051/0004-6361/201116782},
archivePrefix = {arXiv},
       eprint = {1103.5386},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...530A.108E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ekstrom2012,
       author = {{Ekstr{\"o}m}, S. and {Georgy}, C. and {Eggenberger}, P. and {Meynet}, G. and {Mowlavi}, N. and {Wyttenbach}, A. and {Granada}, A. and {Decressin}, T. and {Hirschi}, R. and {Frischknecht}, U. and {Charbonnel}, C. and {Maeder}, A.},
        title = "{Grids of stellar models with rotation. I. Models from 0.8 to 120 M$_{{\ensuremath{\odot}}}$ at solar metallicity (Z = 0.014)}",
      journal = {\aap},
     keywords = {stars: general, stars: evolution, stars: massive, stars: low-mass, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = jan,
       volume = {537},
          eid = {A146},
        pages = {A146},
          doi = {10.1051/0004-6361/201117751},
archivePrefix = {arXiv},
       eprint = {1110.5049},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...537A.146E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{El-badry2024,
       author = {{El-Badry}, Kareem},
        title = "{On the formation of a 33 solar-mass black hole in a low-metallicity binary}",
      journal = {The Open Journal of Astrophysics},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2024,
        month = may,
       volume = {7},
          eid = {38},
        pages = {38},
          doi = {10.33232/001c.117652},
archivePrefix = {arXiv},
       eprint = {2404.13047},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024OJAp....7E..38E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



% -------------------------- F --------------------------
@ARTICLE{Fryer1999,
       author = {{Fryer}, Chris L.},
        title = "{Mass Limits For Black Hole Formation}",
      journal = {\apj},
     keywords = {BLACK HOLE PHYSICS, STARS: EVOLUTION, STARS: INTERIORS, STARS: SUPERNOVAE: GENERAL, Black Hole Physics, Stars: Evolution, Stars: Interiors, Stars: Supernovae: General, Astrophysics},
         year = 1999,
        month = sep,
       volume = {522},
       number = {1},
        pages = {413-418},
          doi = {10.1086/307647},
archivePrefix = {arXiv},
       eprint = {astro-ph/9902315},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...522..413F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Frebel2007,
       author = {{Frebel}, Anna and {Johnson}, Jarrett L. and {Bromm}, Volker},
        title = "{Probing the formation of the first low-mass stars with stellar archaeology}",
      journal = {\mnras},
     keywords = {techniques: spectroscopic, stars: abundances, stars: Population II, Galaxy: halo, Galaxy: stellar content, early Universe, Astrophysics},
         year = 2007,
        month = sep,
       volume = {380},
       number = {1},
        pages = {L40-L44},
          doi = {10.1111/j.1745-3933.2007.00344.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0701395},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007MNRAS.380L..40F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Frebel2015,
       author = {{Frebel}, Anna and {Norris}, John E.},
        title = "{Near-Field Cosmology with Extremely Metal-Poor Stars}",
      journal = {\araa},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = aug,
       volume = {53},
        pages = {631-688},
          doi = {10.1146/annurev-astro-082214-122423},
archivePrefix = {arXiv},
       eprint = {1501.06921},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ARA&A..53..631F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Fu2018,
       author = {{Fu}, Xiaoting and {Bressan}, Alessandro and {Marigo}, Paola and {Girardi}, L{\'e}o and {Montalb{\'a}n}, Josefina and {Chen}, Yang and {Nanni}, Ambra},
        title = "{New PARSEC data base of {\ensuremath{\alpha}}-enhanced stellar evolutionary tracks and isochrones - I. Calibration with 47 Tuc (NGC 104) and the improvement on RGB bump}",
      journal = {\mnras},
     keywords = {stars: evolution, Hertzsprung-Russell and colour-magnitude diagrams, stars: interiors, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = may,
       volume = {476},
       number = {1},
        pages = {496-511},
          doi = {10.1093/mnras/sty235},
archivePrefix = {arXiv},
       eprint = {1801.07137},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.476..496F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Fernandez2018,
    author = {Fernández, Rodrigo and Quataert, Eliot and Kashiyama, Kazumi and Coughlin, Eric R},
    title = "{Mass ejection in failed supernovae: variation with stellar progenitor}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {476},
    number = {2},
    pages = {2366-2383},
    year = {2018},
    month = {02},
    abstract = "{}",
    issn = {0035-8711},
    doi = {10.1093/mnras/sty306},
    url = {https://doi.org/10.1093/mnras/sty306},
    eprint = {https://academic.oup.com/mnras/article-pdf/476/2/2366/24395619/sty306.pdf},
}
@ARTICLE{Farmer2019,
       author = {{Farmer}, R. and {Renzo}, M. and {de Mink}, S.~E. and {Marchant}, P. and {Justham}, S.},
        title = "{Mind the Gap: The Location of the Lower Edge of the Pair-instability Supernova Black Hole Mass Gap}",
      journal = {\apj},
     keywords = {Massive stars, Stellar mass loss, Supernovae, Astrophysical black holes, Stellar mass black holes, Stellar evolution, 732, 1613, 1668, 98, 1611, 1599, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = dec,
       volume = {887},
       number = {1},
          eid = {53},
        pages = {53},
          doi = {10.3847/1538-4357/ab518b10.48550/arXiv.1910.12874},
archivePrefix = {arXiv},
       eprint = {1910.12874},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...887...53F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
% -------------------------- G --------------------------
@ARTICLE{Grafener2008,
       author = {{Gr{\"a}fener}, G. and {Hamann}, W. -R.},
        title = "{Mass loss from late-type WN stars and its Z-dependence. Very massive stars approaching the Eddington limit}",
      journal = {\aap},
     keywords = {stars: Wolf-Rayet, stars: early-type, stars: atmospheres, stars: mass-loss, stars: winds, outflows, stars: individual: WR 22, Astrophysics},
         year = 2008,
        month = may,
       volume = {482},
       number = {3},
        pages = {945-960},
          doi = {10.1051/0004-6361:20066176},
archivePrefix = {arXiv},
       eprint = {0803.0866},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...482..945G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Georgy2013,
       author = {{Georgy}, C. and {Ekstr{\"o}m}, S. and {Eggenberger}, P. and {Meynet}, G. and {Haemmerl{\'e}}, L. and {Maeder}, A. and {Granada}, A. and {Groh}, J.~H. and {Hirschi}, R. and {Mowlavi}, N. and {Yusof}, N. and {Charbonnel}, C. and {Decressin}, T. and {Barblan}, F.},
        title = "{Grids of stellar models with rotation. III. Models from 0.8 to 120 M$_{{\ensuremath{\odot}}}$ at a metallicity Z = 0.002}",
      journal = {\aap},
     keywords = {stars: general, stars: evolution, stars: rotation, stars: massive, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = oct,
       volume = {558},
          eid = {A103},
        pages = {A103},
          doi = {10.1051/0004-6361/201322178},
archivePrefix = {arXiv},
       eprint = {1308.2914},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...558A.103G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Goswami2021,
       author = {{Goswami}, S. and {Slemer}, A. and {Marigo}, P. and {Bressan}, A. and {Silva}, L. and {Spera}, M. and {Boco}, L. and {Grisoni}, V. and {Pantoni}, L. and {Lapi}, A.},
        title = "{The effects of the initial mass function on Galactic chemical enrichment}",
      journal = {\aap},
     keywords = {stars: abundances, stars: massive, Galaxy: abundances, Galaxy: disk, solar neighborhood, Galaxy: evolution, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = jun,
       volume = {650},
          eid = {A203},
        pages = {A203},
          doi = {10.1051/0004-6361/202039842},
archivePrefix = {arXiv},
       eprint = {2104.05680},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...650A.203G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Gaia2024,
       author = {{Gaia Collaboration} and {Panuzzo}, P. and {Mazeh}, T. and {Arenou}, F. and {Holl}, B. and {Caffau}, E. and {Jorissen}, A. and {Babusiaux}, C. and {Gavras}, P. and {Sahlmann}, J. and {Bastian}, U. and {Wyrzykowski}, {\L}. and {Eyer}, L. and {Leclerc}, N. and {Bauchet}, N. and {Bombrun}, A. and {Mowlavi}, N. and {Seabroke}, G.~M. and {Teyssier}, D. and {Balbinot}, E. and {Helmi}, A. and {Brown}, A.~G.~A. and {Vallenari}, A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Barbier}, A. and {Biermann}, M. and {Creevey}, O.~L. and {Ducourant}, C. and {Evans}, D.~W. and {Guerra}, R. and {Hutton}, A. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Nicolas}, C. and {Randich}, S. and {Sartoretti}, P. and {Smiljanic}, R. and {Tanga}, P. and {Walton}, N.~A. and {Aerts}, C. and {Bailer-Jones}, C.~A.~L. and {Cropper}, M. and {Drimmel}, R. and {Jansen}, F. and {Katz}, D. and {Lattanzi}, M.~G. and {Soubiran}, C. and {Th{\'e}venin}, F. and {van Leeuwen}, F. and {Andrae}, R. and {Audard}, M. and {Bakker}, J. and {Blomme}, R. and {Casta{\~n}eda}, J. and {De Angeli}, F. and {Fabricius}, C. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Galluccio}, L. and {Guerrier}, A. and {Heiter}, U. and {Masana}, E. and {Messineo}, R. and {Nienartowicz}, K. and {Pailler}, F. and {Riclet}, F. and {Roux}, W. and {Sordo}, R. and {Gracia-Abril}, G. and {Portell}, J. and {Altmann}, M. and {Benson}, K. and {Berthier}, J. and {Burgess}, P.~W. and {Busonero}, D. and {Busso}, G. and {Cacciari}, C. and {C{\'a}novas}, H. and {Carrasco}, J.~M. and {Carry}, B. and {Cellino}, A. and {Cheek}, N. and {Clementini}, G. and {Damerdji}, Y. and {Davidson}, M. and {de Teodoro}, P. and {Delchambre}, L. and {Dell'Oro}, A. and {Fraile Garcia}, E. and {Garabato}, D. and {Garc{\'\i}a-Lario}, P. and {Haigron}, R. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hatzidimitriou}, D. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Jamal}, S. and {Jevardat de Fombelle}, G. and {Jordan}, S. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {L{\"o}ffler}, W. and {Lorca}, A. and {Marchal}, O. and {Marrese}, P.~M. and {Moitinho}, A. and {Muinonen}, K. and {Nu{\~n}ez Campos}, M. and {Oreshina-Slezak}, I. and {Osborne}, P. and {Pancino}, E. and {Pauwels}, T. and {Recio-Blanco}, A. and {Riello}, M. and {Rimoldini}, L. and {Robin}, A.~C. and {Roegiers}, T. and {Sarro}, L.~M. and {Schultheis}, M. and {Smith}, M. and {Sozzetti}, A. and {Utrilla}, E. and {van Leeuwen}, M. and {Weingrill}, K. and {Abbas}, U. and {{\'A}brah{\'a}m}, P. and {Abreu Aramburu}, A. and {Ahmed}, S. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Anders}, F. and {Anderson}, R.~I. and {Anglada Varela}, E. and {Antoja}, T. and {Baig}, S. and {Baines}, D. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balog}, Z. and {Barache}, C. and {Barros}, M. and {Barstow}, M.~A. and {Bartolom{\'e}}, S. and {Bashi}, D. and {Bassilana}, J. -L. and {Baudeau}, N. and {Becciani}, U. and {Bedin}, L.~R. and {Bellas-Velidis}, I. and {Bellazzini}, M. and {Beordo}, W. and {Bernet}, M. and {Bertolotto}, C. and {Bertone}, S. and {Bianchi}, L. and {Binnenfeld}, A. and {Blanco-Cuaresma}, S. and {Bland-Hawthorn}, J. and {Blazere}, A. and {Boch}, T. and {Bossini}, D. and {Bouquillon}, S. and {Bragaglia}, A. and {Braine}, J. and {Bratsolis}, E. and {Breedt}, E. and {Bressan}, A. and {Brouillet}, N. and {Brugaletta}, E. and {Bucciarelli}, B. and {Butkevich}, A.~G. and {Buzzi}, R. and {Camut}, A. and {Cancelliere}, R. and {Cantat-Gaudin}, T. and {Capilla Guilarte}, D. and {Carballo}, R. and {Carlucci}, T. and {Carnerero}, M.~I. and {Carretero}, J. and {Carton}, S. and {Casamiquela}, L. and {Casey}, A. and {Castellani}, M. and {Castro-Ginard}, A. and {Ceraj}, L. and {Cesare}, V. and {Charlot}, P. and {Chaudet}, C. and {Chemin}, L. and {Chiavassa}, A. and {Chornay}, N. and {Chosson}, D. and {Cooper}, W.~J. and {Cornez}, T. and {Cowell}, S. and {Crosta}, M. and {Crowley}, C. and {Cruz Reyes}, M. and {Dafonte}, C. and {Dal Ponte}, M. and {David}, M. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {de Torres}, A. and {del Peloso}, E.~F. and {Delbo}, M. and {Delgado}, A. and {Delisle}, J. -B. and {Demouchy}, C. and {Denis}, E. and {Dharmawardena}, T.~E. and {Di Giacomo}, F. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and {Dsilva}, K. and {Enke}, H. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Fatovi{\'c}}, M. and {Fedorets}, G. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fernique}, P. and {Figueras}, F. and {Fouron}, C. and {Fragkoudi}, F. and {Gai}, M. and {Galinier}, M. and {Garcia-Serrano}, A. and {Garc{\'\i}a-Torres}, M. and {Garofalo}, A. and {Gerlach}, E. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomboc}, A. and {Gomez}, A. and {Gonz{\'a}lez-Santamar{\'\i}a}, I. and {Gosset}, E. and {Granvik}, M. and {Gregori Barrera}, V. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Haywood}, M. and {Helmer}, A. and {Hidalgo}, S.~L. and {Hilger}, T. and {Hobbs}, D. and {Hottier}, C. and {Huckle}, H.~E. and {Jim{\'e}nez-Arranz}, {\'O}. and {Juaristi Campillo}, J. and {Kaczmarek}, Z. and {Kervella}, P. and {Khanna}, S. and {Kontizas}, M. and {Kordopatis}, G. and {Korn}, A.~J. and {K{\'o}sp{\'a}l}, {\'A}. and {Kostrzewa-Rutkowska}, Z. and {Kruszy{\'n}ska}, K. and {Kun}, M. and {Lambert}, S. and {Lanza}, A.~F. and {Lebreton}, Y. and {Lebzelter}, T. and {Leccia}, S. and {Lecoutre}, G. and {Liao}, S. and {Liberato}, L. and {Licata}, E. and {Livanou}, E. and {Lobel}, A. and {L{\'o}pez-Miralles}, J. and {Loup}, C. and {Madar{\'a}sz}, M. and {Mahy}, L. and {Mann}, R.~G. and {Manteiga}, M. and {Marcellino}, C.~P. and {Marchant}, J.~M. and {Marconi}, M. and {Mar{\'\i}n Pina}, D. and {Marinoni}, S. and {Marshall}, D.~J. and {Mart{\'\i}n Lozano}, J. and {Martin Polo}, L. and {Mart{\'\i}n-Fleitas}, J.~M. and {Marton}, G. and {Mascarenhas}, D. and {Masip}, A. and {Mastrobuono-Battisti}, A. and {McMillan}, P.~J. and {Meichsner}, J. and {Merc}, J. and {Messina}, S. and {Millar}, N.~R. and {Mints}, A. and {Mohamed}, D. and {Molina}, D. and {Molinaro}, R. and {Moln{\'a}r}, L. and {Mongui{\'o}}, M. and {Montegriffo}, P. and {Monti}, L. and {Mora}, A. and {Morbidelli}, R. and {Morris}, D. and {Mudimadugula}, R. and {Muraveva}, T. and {Musella}, I. and {Nagy}, Z. and {Nardetto}, N. and {Navarrete}, C. and {Oh}, S. and {Ordenovic}, C. and {Orenstein}, O. and {Pagani}, C. and {Pagano}, I. and {Palaversa}, L. and {Palicio}, P.~A. and {Pallas-Quintela}, L. and {Pawlak}, M. and {Penttil{\"a}}, A. and {Pesciullesi}, P. and {Pinamonti}, M. and {Plachy}, E. and {Planquart}, L. and {Plum}, G. and {Poggio}, E. and {Pourbaix}, D. and {Price-Whelan}, A.~M. and {Pulone}, L. and {Rabin}, V. and {Rainer}, M. and {Raiteri}, C.~M. and {Ramos}, P. and {Ramos-Lerate}, M. and {Ratajczak}, M. and {Re Fiorentin}, P. and {Regibo}, S. and {Reyl{\'e}}, C. and {Ripepi}, V. and {Riva}, A. and {Rix}, H. -W. and {Rixon}, G. and {Robert}, G. and {Robichon}, N. and {Robin}, C. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Ruz Mieres}, D. and {Rybicki}, K.~A. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, A. and {Sanna}, N. and {Santove{\~n}a}, R. and {Sarasso}, M. and {Sarmiento}, M.~H. and {Sarrate Riera}, C. and {Sciacca}, E. and {S{\'e}gransan}, D. and {Semczuk}, M. and {Shahaf}, S. and {Siebert}, A. and {Slezak}, E. and {Smart}, R.~L. and {Snaith}, O.~N. and {Solano}, E. and {Solitro}, F. and {Souami}, D. and {Souchay}, J. and {Spitoni}, E. and {Spoto}, F. and {Squillante}, L.~A. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Surdej}, J. and {Szabados}, L. and {Taris}, F. and {Taylor}, M.~B. and {Teixeira}, R. and {Tepper-Garcia}, T. and {Thuillot}, W. and {Tolomei}, L. and {Tonello}, N. and {Torra}, F. and {Torralba Elipe}, G. and {Trabucchi}, M. and {Trentin}, E. and {Tsantaki}, M. and {Turon}, C. and {Ulla}, A. and {Unger}, N. and {Valtchanov}, I. and {Vanel}, O. and {Vecchiato}, A. and {Vicente}, D. and {Villar}, E. and {Weiler}, M. and {Zhao}, H. and {Zorec}, J. and {Zucker}, S. and {{\v{Z}}upi{\'c}}, A. and {Zwitter}, T.},
        title = "{Discovery of a dormant 33 solar-mass black hole in pre-release Gaia astrometry}",
      journal = {\aap},
     keywords = {astrometry, binaries: spectroscopic, stars: black holes, stars: evolution, stars: massive, stars: Population II, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2024,
        month = jun,
       volume = {686},
          eid = {L2},
        pages = {L2},
          doi = {10.1051/0004-6361/202449763},
archivePrefix = {arXiv},
       eprint = {2404.10486},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024A&A...686L...2G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




% -------------------------- H --------------------------
@ARTICLE{Haft1994,
       author = {{Haft}, Martin and {Raffelt}, Georg and {Weiss}, Achim},
        title = "{Standard and Nonstandard Plasma Neutrino Emission Revisited}",
      journal = {\apj},
     keywords = {Computational Astrophysics, Emission Spectra, Magnetic Dispersion, Neutrinos, Numerical Analysis, Plasmas (Physics), Quantum Electrodynamics, Approximation, Magnetic Dipoles, Stellar Cores, Stellar Evolution, Astrophysics, ELEMENTARY PARTICLES, PLASMAS, RADIATION MECHANISMS: MISCELLANEOUS, STARS: GIANTS, STARS: INTERIORS, Astrophysics},
         year = 1994,
        month = apr,
       volume = {425},
        pages = {222},
          doi = {10.1086/173978},
archivePrefix = {arXiv},
       eprint = {astro-ph/9309014},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994ApJ...425..222H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Heger2000,
       author = {{Heger}, A. and {Langer}, N. and {Woosley}, S.~E.},
        title = "{Presupernova Evolution of Rotating Massive Stars. I. Numerical Method and Evolution of the Internal Stellar Structure}",
      journal = {\apj},
     keywords = {HYDRODYNAMICS, METHODS: NUMERICAL, STARS EARLY-TYPE, STARS: EVOLUTION, STARS: INTERIORS, STARS ROTATION, Hydrodynamics, Methods: Numerical, stars early-type, Stars: Evolution, Stars: Interiors, stars rotation, Astrophysics},
         year = 2000,
        month = jan,
       volume = {528},
       number = {1},
        pages = {368-396},
          doi = {10.1086/308158},
archivePrefix = {arXiv},
       eprint = {astro-ph/9904132},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...528..368H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{HegerWoosley2002,
       author = {{Heger}, A. and {Woosley}, S.~E.},
        title = "{The Nucleosynthetic Signature of Population III}",
      journal = {\apj},
     keywords = {Nuclear Reactions, Nucleosynthesis, Abundances, Stars: Early-Type, Stars: Supernovae: General, Astrophysics},
         year = 2002,
        month = mar,
       volume = {567},
       number = {1},
        pages = {532-543},
          doi = {10.1086/338487},
archivePrefix = {arXiv},
       eprint = {astro-ph/0107037},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...567..532H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Heger2002,
       author = {{Heger}, Alexander and {Woosley}, Stan and {Baraffe}, Isabelle and {Abel}, Tom},
        title = "{Evolution and Explosion of Very Massive Primordial Stars}",
     keywords = {Astrophysics},
    booktitle = {Lighthouses of the Universe: The Most Luminous Celestial Objects and Their Use for Cosmology},
         year = 2002,
       editor = {{Gilfanov}, Marat and {Sunyeav}, Rashid and {Churazov}, Eugene},
        month = jan,
        pages = {369},
          doi = {10.1007/10856495_57},
archivePrefix = {arXiv},
       eprint = {astro-ph/0112059},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002luml.conf..369H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Heger2003,
       author = {{Heger}, A. and {Fryer}, C.~L. and {Woosley}, S.~E. and {Langer}, N. and {Hartmann}, D.~H.},
        title = "{How Massive Single Stars End Their Life}",
      journal = {\apj},
     keywords = {Black Hole Physics, Gamma Rays: Bursts, Stars: Early-Type, Stars: Neutron, Stars: Supernovae: General, Astrophysics},
         year = 2003,
        month = jul,
       volume = {591},
       number = {1},
        pages = {288-300},
          doi = {10.1086/375341},
archivePrefix = {arXiv},
       eprint = {astro-ph/0212469},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...591..288H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Haehnelt2001,
       author = {{Haehnelt}, Martin G. and {Madau}, Piero and {Kudritzki}, Rolf and {Haardt}, Francesco},
        title = "{An Ionizing Ultraviolet Background Dominated by Massive Stars}",
      journal = {\apjl},
     keywords = {Cosmology: Theory, Galaxies: Intergalactic Medium, Galaxies: Quasars: Absorption Lines, Astrophysics},
         year = 2001,
        month = mar,
       volume = {549},
       number = {2},
        pages = {L151-L154},
          doi = {10.1086/319170},
archivePrefix = {arXiv},
       eprint = {astro-ph/0010631},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...549L.151H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Hirschi2005,
       author = {{Hirschi}, R. and {Meynet}, G. and {Maeder}, A.},
        title = "{Yields of rotating stars at solar metallicity}",
      journal = {\aap},
     keywords = {stars: abundances, stars: evolution, stars: rotation, stars: Wolf-Rayet, stars: supernovae: general, Astrophysics},
         year = 2005,
        month = apr,
       volume = {433},
       number = {3},
        pages = {1013-1022},
          doi = {10.1051/0004-6361:20041554},
archivePrefix = {arXiv},
       eprint = {astro-ph/0412454},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A&A...433.1013H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



% -------------------------- I --------------------------
@ARTICLE{Itoh2008,
       author = {{Itoh}, Naoki and {Uchida}, Shinsuke and {Sakamoto}, Yu and {Kohyama}, Yasuharu and {Nozawa}, Satoshi},
        title = "{The Second Born Corrections to the Electrical and Thermal Conductivities of Dense Matter in the Liquid Metal Phase}",
      journal = {\apj},
     keywords = {atomic processes, dense matter, stars: neutron, white dwarfs, Astrophysics},
         year = 2008,
        month = apr,
       volume = {677},
       number = {1},
        pages = {495-502},
          doi = {10.1086/529367},
archivePrefix = {arXiv},
       eprint = {0708.2967},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...677..495I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Iglesias1996,
       author = {{Iglesias}, Carlos A. and {Rogers}, Forrest J.},
        title = "{Updated Opal Opacities}",
      journal = {\apj},
     keywords = {ATOMIC DATA, ATOMIC PROCESSES, STARS: INTERIORS},
         year = 1996,
        month = jun,
       volume = {464},
        pages = {943},
          doi = {10.1086/177381},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...464..943I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{ItohKohyama1983,
       author = {{Itoh}, N. and {Kohyama}, Y.},
        title = "{Neutrino-pair bremsstrahlung in dense stars. I. Liquid metal case.}",
      journal = {\apj},
     keywords = {Bremsstrahlung, Neutrinos, Neutron Stars, Pair Production, Stellar Models, White Dwarf Stars, Coulomb Collisions, Density Distribution, Liquid Metals, Stellar Temperature, Astrophysics, Bremsstrahlung:Degenerate Stars, Degenerate Stars:Bremsstrahlung, Dense Matter:Neutrinos, Neutrinos:Dense Matter, Neutron Stars:Radiative Transfer, Radiative Transfer:Neutron Stars, Radiative Transfer:White Dwarfs, White Dwarfs:Radiative Transfer},
         year = 1983,
        month = dec,
       volume = {275},
        pages = {858-866},
          doi = {10.1086/161579},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1983ApJ...275..858I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ivezic2019,
       author = {{Ivezi{\'c}}, {\v{Z}}eljko and {Kahn}, Steven M. and {Tyson}, J. Anthony and {Abel}, Bob and {Acosta}, Emily and {Allsman}, Robyn and {Alonso}, David and {AlSayyad}, Yusra and {Anderson}, Scott F. and {Andrew}, John and {Angel}, James Roger P. and {Angeli}, George Z. and {Ansari}, Reza and {Antilogus}, Pierre and {Araujo}, Constanza and {Armstrong}, Robert and {Arndt}, Kirk T. and {Astier}, Pierre and {Aubourg}, {\'E}ric and {Auza}, Nicole and {Axelrod}, Tim S. and {Bard}, Deborah J. and {Barr}, Jeff D. and {Barrau}, Aurelian and {Bartlett}, James G. and {Bauer}, Amanda E. and {Bauman}, Brian J. and {Baumont}, Sylvain and {Bechtol}, Ellen and {Bechtol}, Keith and {Becker}, Andrew C. and {Becla}, Jacek and {Beldica}, Cristina and {Bellavia}, Steve and {Bianco}, Federica B. and {Biswas}, Rahul and {Blanc}, Guillaume and {Blazek}, Jonathan and {Blandford}, Roger D. and {Bloom}, Josh S. and {Bogart}, Joanne and {Bond}, Tim W. and {Booth}, Michael T. and {Borgland}, Anders W. and {Borne}, Kirk and {Bosch}, James F. and {Boutigny}, Dominique and {Brackett}, Craig A. and {Bradshaw}, Andrew and {Brandt}, William Nielsen and {Brown}, Michael E. and {Bullock}, James S. and {Burchat}, Patricia and {Burke}, David L. and {Cagnoli}, Gianpietro and {Calabrese}, Daniel and {Callahan}, Shawn and {Callen}, Alice L. and {Carlin}, Jeffrey L. and {Carlson}, Erin L. and {Chandrasekharan}, Srinivasan and {Charles-Emerson}, Glenaver and {Chesley}, Steve and {Cheu}, Elliott C. and {Chiang}, Hsin-Fang and {Chiang}, James and {Chirino}, Carol and {Chow}, Derek and {Ciardi}, David R. and {Claver}, Charles F. and {Cohen-Tanugi}, Johann and {Cockrum}, Joseph J. and {Coles}, Rebecca and {Connolly}, Andrew J. and {Cook}, Kem H. and {Cooray}, Asantha and {Covey}, Kevin R. and {Cribbs}, Chris and {Cui}, Wei and {Cutri}, Roc and {Daly}, Philip N. and {Daniel}, Scott F. and {Daruich}, Felipe and {Daubard}, Guillaume and {Daues}, Greg and {Dawson}, William and {Delgado}, Francisco and {Dellapenna}, Alfred and {de Peyster}, Robert and {de Val-Borro}, Miguel and {Digel}, Seth W. and {Doherty}, Peter and {Dubois}, Richard and {Dubois-Felsmann}, Gregory P. and {Durech}, Josef and {Economou}, Frossie and {Eifler}, Tim and {Eracleous}, Michael and {Emmons}, Benjamin L. and {Fausti Neto}, Angelo and {Ferguson}, Henry and {Figueroa}, Enrique and {Fisher-Levine}, Merlin and {Focke}, Warren and {Foss}, Michael D. and {Frank}, James and {Freemon}, Michael D. and {Gangler}, Emmanuel and {Gawiser}, Eric and {Geary}, John C. and {Gee}, Perry and {Geha}, Marla and {Gessner}, Charles J.~B. and {Gibson}, Robert R. and {Gilmore}, D. Kirk and {Glanzman}, Thomas and {Glick}, William and {Goldina}, Tatiana and {Goldstein}, Daniel A. and {Goodenow}, Iain and {Graham}, Melissa L. and {Gressler}, William J. and {Gris}, Philippe and {Guy}, Leanne P. and {Guyonnet}, Augustin and {Haller}, Gunther and {Harris}, Ron and {Hascall}, Patrick A. and {Haupt}, Justine and {Hernandez}, Fabio and {Herrmann}, Sven and {Hileman}, Edward and {Hoblitt}, Joshua and {Hodgson}, John A. and {Hogan}, Craig and {Howard}, James D. and {Huang}, Dajun and {Huffer}, Michael E. and {Ingraham}, Patrick and {Innes}, Walter R. and {Jacoby}, Suzanne H. and {Jain}, Bhuvnesh and {Jammes}, Fabrice and {Jee}, M. James and {Jenness}, Tim and {Jernigan}, Garrett and {Jevremovi{\'c}}, Darko and {Johns}, Kenneth and {Johnson}, Anthony S. and {Johnson}, Margaret W.~G. and {Jones}, R. Lynne and {Juramy-Gilles}, Claire and {Juri{\'c}}, Mario and {Kalirai}, Jason S. and {Kallivayalil}, Nitya J. and {Kalmbach}, Bryce and {Kantor}, Jeffrey P. and {Karst}, Pierre and {Kasliwal}, Mansi M. and {Kelly}, Heather and {Kessler}, Richard and {Kinnison}, Veronica and {Kirkby}, David and {Knox}, Lloyd and {Kotov}, Ivan V. and {Krabbendam}, Victor L. and {Krughoff}, K. Simon and {Kub{\'a}nek}, Petr and {Kuczewski}, John and {Kulkarni}, Shri and {Ku}, John and {Kurita}, Nadine R. and {Lage}, Craig S. and {Lambert}, Ron and {Lange}, Travis and {Langton}, J. Brian and {Le Guillou}, Laurent and {Levine}, Deborah and {Liang}, Ming and {Lim}, Kian-Tat and {Lintott}, Chris J. and {Long}, Kevin E. and {Lopez}, Margaux and {Lotz}, Paul J. and {Lupton}, Robert H. and {Lust}, Nate B. and {MacArthur}, Lauren A. and {Mahabal}, Ashish and {Mandelbaum}, Rachel and {Markiewicz}, Thomas W. and {Marsh}, Darren S. and {Marshall}, Philip J. and {Marshall}, Stuart and {May}, Morgan and {McKercher}, Robert and {McQueen}, Michelle and {Meyers}, Joshua and {Migliore}, Myriam and {Miller}, Michelle and {Mills}, David J. and {Miraval}, Connor and {Moeyens}, Joachim and {Moolekamp}, Fred E. and {Monet}, David G. and {Moniez}, Marc and {Monkewitz}, Serge and {Montgomery}, Christopher and {Morrison}, Christopher B. and {Mueller}, Fritz and {Muller}, Gary P. and {Mu{\~n}oz Arancibia}, Freddy and {Neill}, Douglas R. and {Newbry}, Scott P. and {Nief}, Jean-Yves and {Nomerotski}, Andrei and {Nordby}, Martin and {O'Connor}, Paul and {Oliver}, John and {Olivier}, Scot S. and {Olsen}, Knut and {O'Mullane}, William and {Ortiz}, Sandra and {Osier}, Shawn and {Owen}, Russell E. and {Pain}, Reynald and {Palecek}, Paul E. and {Parejko}, John K. and {Parsons}, James B. and {Pease}, Nathan M. and {Peterson}, J. Matt and {Peterson}, John R. and {Petravick}, Donald L. and {Libby Petrick}, M.~E. and {Petry}, Cathy E. and {Pierfederici}, Francesco and {Pietrowicz}, Stephen and {Pike}, Rob and {Pinto}, Philip A. and {Plante}, Raymond and {Plate}, Stephen and {Plutchak}, Joel P. and {Price}, Paul A. and {Prouza}, Michael and {Radeka}, Veljko and {Rajagopal}, Jayadev and {Rasmussen}, Andrew P. and {Regnault}, Nicolas and {Reil}, Kevin A. and {Reiss}, David J. and {Reuter}, Michael A. and {Ridgway}, Stephen T. and {Riot}, Vincent J. and {Ritz}, Steve and {Robinson}, Sean and {Roby}, William and {Roodman}, Aaron and {Rosing}, Wayne and {Roucelle}, Cecille and {Rumore}, Matthew R. and {Russo}, Stefano and {Saha}, Abhijit and {Sassolas}, Benoit and {Schalk}, Terry L. and {Schellart}, Pim and {Schindler}, Rafe H. and {Schmidt}, Samuel and {Schneider}, Donald P. and {Schneider}, Michael D. and {Schoening}, William and {Schumacher}, German and {Schwamb}, Megan E. and {Sebag}, Jacques and {Selvy}, Brian and {Sembroski}, Glenn H. and {Seppala}, Lynn G. and {Serio}, Andrew and {Serrano}, Eduardo and {Shaw}, Richard A. and {Shipsey}, Ian and {Sick}, Jonathan and {Silvestri}, Nicole and {Slater}, Colin T. and {Smith}, J. Allyn and {Smith}, R. Chris and {Sobhani}, Shahram and {Soldahl}, Christine and {Storrie-Lombardi}, Lisa and {Stover}, Edward and {Strauss}, Michael A. and {Street}, Rachel A. and {Stubbs}, Christopher W. and {Sullivan}, Ian S. and {Sweeney}, Donald and {Swinbank}, John D. and {Szalay}, Alexander and {Takacs}, Peter and {Tether}, Stephen A. and {Thaler}, Jon J. and {Thayer}, John Gregg and {Thomas}, Sandrine and {Thornton}, Adam J. and {Thukral}, Vaikunth and {Tice}, Jeffrey and {Trilling}, David E. and {Turri}, Max and {Van Berg}, Richard and {Vanden Berk}, Daniel and {Vetter}, Kurt and {Virieux}, Francoise and {Vucina}, Tomislav and {Wahl}, William and {Walkowicz}, Lucianne and {Walsh}, Brian and {Walter}, Christopher W. and {Wang}, Daniel L. and {Wang}, Shin-Yawn and {Warner}, Michael and {Wiecha}, Oliver and {Willman}, Beth and {Winters}, Scott E. and {Wittman}, David and {Wolff}, Sidney C. and {Wood-Vasey}, W. Michael and {Wu}, Xiuqin and {Xin}, Bo and {Yoachim}, Peter and {Zhan}, Hu},
        title = "{LSST: From Science Drivers to Reference Design and Anticipated Data Products}",
      journal = {\apj},
     keywords = {astrometry, cosmology: observations, Galaxy: general, methods: observational, stars: general, surveys, Astrophysics},
         year = 2019,
        month = mar,
       volume = {873},
       number = {2},
          eid = {111},
        pages = {111},
          doi = {10.3847/1538-4357/ab042c},
archivePrefix = {arXiv},
       eprint = {0805.2366},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...873..111I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Iorio2024,
       author = {{Iorio}, Giuliano and {Torniamenti}, Stefano and {Mapelli}, Michela and {Dall'Amico}, Marco and {Trani}, Alessandro A. and {Rastello}, Sara and {Sgalletta}, Cecilia and {Rinaldi}, Stefano and {Costa}, Guglielmo and {Dahl-Lahtinen}, Bera A. and {Escobar}, Gast{\'o}n J. and {Korb}, Erika and {Vaccaro}, M. Paola and {Lacchin}, Elena and {Mestichelli}, Benedetta and {Di Carlo}, Ugo N. and {Spera}, Mario and {Arca Sedda}, Manuel},
        title = "{The boring history of Gaia BH3 from isolated binary evolution}",
      journal = {\aap},
     keywords = {methods: numerical, binaries: general, stars: black holes, stars: massive, Galaxy: halo, Galaxy: stellar content, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2024,
        month = oct,
       volume = {690},
          eid = {A144},
        pages = {A144},
          doi = {10.1051/0004-6361/202450531},
archivePrefix = {arXiv},
       eprint = {2404.17568},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024A&A...690A.144I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




% -------------------------- J --------------------------
@ARTICLE{Johnson2013,
       author = {{Johnson}, Jarrett L. and {Dalla Vecchia}, Claudio and {Khochfar}, Sadegh},
        title = "{The First Billion Years project: the impact of stellar radiation on the co-evolution of Populations II and III}",
      journal = {\mnras},
     keywords = {molecular processes, galaxies: formation, galaxies: high-redshift, intergalactic medium, cosmology: theory, early Universe, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = jan,
       volume = {428},
       number = {3},
        pages = {1857-1872},
          doi = {10.1093/mnras/sts011},
archivePrefix = {arXiv},
       eprint = {1206.5824},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.428.1857J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


% -------------------------- K --------------------------
@ARTICLE{Komatsu2011,
       author = {{Komatsu}, E. and {Smith}, K.~M. and {Dunkley}, J. and {Bennett}, C.~L. and {Gold}, B. and {Hinshaw}, G. and {Jarosik}, N. and {Larson}, D. and {Nolta}, M.~R. and {Page}, L. and {Spergel}, D.~N. and {Halpern}, M. and {Hill}, R.~S. and {Kogut}, A. and {Limon}, M. and {Meyer}, S.~S. and {Odegard}, N. and {Tucker}, G.~S. and {Weiland}, J.~L. and {Wollack}, E. and {Wright}, E.~L.},
        title = "{Seven-year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Cosmological Interpretation}",
      journal = {\apjs},
     keywords = {cosmic background radiation, cosmology: observations, dark matter, early universe, space vehicles, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2011,
        month = feb,
       volume = {192},
       number = {2},
          eid = {18},
        pages = {18},
          doi = {10.1088/0067-0049/192/2/18},
archivePrefix = {arXiv},
       eprint = {1001.4538},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJS..192...18K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kremer2020,
       author = {{Kremer}, Kyle and {Spera}, Mario and {Becker}, Devin and {Chatterjee}, Sourav and {Di Carlo}, Ugo N. and {Fragione}, Giacomo and {Rodriguez}, Carl L. and {Ye}, Claire S. and {Rasio}, Frederic A.},
        title = "{Populating the Upper Black Hole Mass Gap through Stellar Collisions in Young Star Clusters}",
      journal = {\apj},
     keywords = {Stellar mass black holes, Gravitational waves, Globular star clusters, 1611, 678, 656, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = nov,
       volume = {903},
       number = {1},
          eid = {45},
        pages = {45},
          doi = {10.3847/1538-4357/abb945},
archivePrefix = {arXiv},
       eprint = {2006.10771},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...903...45K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Klessen2023,
       author = {{Klessen}, Ralf S. and {Glover}, Simon C.~O.},
        title = "{The First Stars: Formation, Properties, and Impact}",
      journal = {\araa},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2023,
        month = aug,
       volume = {61},
        pages = {65-130},
          doi = {10.1146/annurev-astro-071221-053453},
archivePrefix = {arXiv},
       eprint = {2303.12500},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023ARA&A..61...65K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Koutsouridou2023,
       author = {{Koutsouridou}, Ioanna and {Salvadori}, Stefania and {Sk{\'u}lad{\'o}ttir}, {\'A}sa},
        title = "{True PISN descendant: implications for the mass distribution of the first stars}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2023,
        month = dec,
          eid = {arXiv:2312.05309},
        pages = {arXiv:2312.05309},
          doi = {10.48550/arXiv.2312.05309},
archivePrefix = {arXiv},
       eprint = {2312.05309},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023arXiv231205309K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


% -------------------------- L --------------------------
@ARTICLE{Limongi2003,
       author = {{Limongi}, Marco and {Chieffi}, Alessandro},
        title = "{Evolution, Explosion, and Nucleosynthesis of Core-Collapse Supernovae}",
      journal = {\apj},
     keywords = {Nuclear Reactions, Nucleosynthesis, Abundances, Stars: Evolution, Stars: Interiors, Stars: Supernovae: General, Astrophysics},
         year = 2003,
        month = jul,
       volume = {592},
       number = {1},
        pages = {404-433},
          doi = {10.1086/375703},
archivePrefix = {arXiv},
       eprint = {astro-ph/0304185},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...592..404L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@misc{LSSTsciencecollaboration2009,
      title={LSST Science Book, Version 2.0}, 
      author={LSST Science Collaboration and Paul A. Abell and Julius Allison and Scott F. Anderson and John R. Andrew and J. Roger P. Angel and Lee Armus and David Arnett and S. J. Asztalos and Tim S. Axelrod and Stephen Bailey and D. R. Ballantyne and Justin R. Bankert and Wayne A. Barkhouse and Jeffrey D. Barr and L. Felipe Barrientos and Aaron J. Barth and James G. Bartlett and Andrew C. Becker and Jacek Becla and Timothy C. Beers and Joseph P. Bernstein and Rahul Biswas and Michael R. Blanton and Joshua S. Bloom and John J. Bochanski and Pat Boeshaar and Kirk D. Borne and Marusa Bradac and W. N. Brandt and Carrie R. Bridge and Michael E. Brown and Robert J. Brunner and James S. Bullock and Adam J. Burgasser and James H. Burge and David L. Burke and Phillip A. Cargile and Srinivasan Chandrasekharan and George Chartas and Steven R. Chesley and You-Hua Chu and David Cinabro and Mark W. Claire and Charles F. Claver and Douglas Clowe and A. J. Connolly and Kem H. Cook and Jeff Cooke and Asantha Cooray and Kevin R. Covey and Christopher S. Culliton and Roelof de Jong and Willem H. de Vries and Victor P. Debattista and Francisco Delgado and Ian P. Dell'Antonio and Saurav Dhital and Rosanne Di Stefano and Mark Dickinson and Benjamin Dilday and S. G. Djorgovski and Gregory Dobler and Ciro Donalek and Gregory Dubois-Felsmann and Josef Durech and Ardis Eliasdottir and Michael Eracleous and Laurent Eyer and Emilio E. Falco and Xiaohui Fan and Christopher D. Fassnacht and Harry C. Ferguson and Yanga R. Fernandez and Brian D. Fields and Douglas Finkbeiner and Eduardo E. Figueroa and Derek B. Fox and Harold Francke and James S. Frank and Josh Frieman and Sebastien Fromenteau and Muhammad Furqan and Gaspar Galaz and A. Gal-Yam and Peter Garnavich and Eric Gawiser and John Geary and Perry Gee and Robert R. Gibson and Kirk Gilmore and Emily A. Grace and Richard F. Green and William J. Gressler and Carl J. Grillmair and Salman Habib and J. S. Haggerty and Mario Hamuy and Alan W. Harris and Suzanne L. Hawley and Alan F. Heavens and Leslie Hebb and Todd J. Henry and Edward Hileman and Eric J. Hilton and Keri Hoadley and J. B. Holberg and Matt J. Holman and Steve B. Howell and Leopoldo Infante and Zeljko Ivezic and Suzanne H. Jacoby and Bhuvnesh Jain and R and Jedicke and M. James Jee and J. Garrett Jernigan and Saurabh W. Jha and Kathryn V. Johnston and R. Lynne Jones and Mario Juric and Mikko Kaasalainen and Styliani and Kafka and Steven M. Kahn and Nathan A. Kaib and Jason Kalirai and Jeff Kantor and Mansi M. Kasliwal and Charles R. Keeton and Richard Kessler and Zoran Knezevic and Adam Kowalski and Victor L. Krabbendam and K. Simon Krughoff and Shrinivas Kulkarni and Stephen Kuhlman and Mark Lacy and Sebastien Lepine and Ming Liang and Amy Lien and Paulina Lira and Knox S. Long and Suzanne Lorenz and Jennifer M. Lotz and R. H. Lupton and Julie Lutz and Lucas M. Macri and Ashish A. Mahabal and Rachel Mandelbaum and Phil Marshall and Morgan May and Peregrine M. McGehee and Brian T. Meadows and Alan Meert and Andrea Milani and Christopher J. Miller and Michelle Miller and David Mills and Dante Minniti and David Monet and Anjum S. Mukadam and Ehud Nakar and Douglas R. Neill and Jeffrey A. Newman and Sergei Nikolaev and Martin Nordby and Paul O'Connor and Masamune Oguri and John Oliver and Scot S. Olivier and Julia K. Olsen and Knut Olsen and Edward W. Olszewski and Hakeem Oluseyi and Nelson D. Padilla and Alex Parker and Joshua Pepper and John R. Peterson and Catherine Petry and Philip A. Pinto and James L. Pizagno and Bogdan Popescu and Andrej Prsa and Veljko Radcka and M. Jordan Raddick and Andrew Rasmussen and Arne Rau and Jeonghee Rho and James E. Rhoads and Gordon T. Richards and Stephen T. Ridgway and Brant E. Robertson and Rok Roskar and Abhijit Saha and Ata Sarajedini and Evan Scannapieco and Terry Schalk and Rafe Schindler and Samuel Schmidt and Sarah Schmidt and Donald P. Schneider and German Schumacher and Ryan Scranton and Jacques Sebag and Lynn G. Seppala and Ohad Shemmer and Joshua D. Simon and M. Sivertz and Howard A. Smith and J. Allyn Smith and Nathan Smith and Anna H. Spitz and Adam Stanford and Keivan G. Stassun and Jay Strader and Michael A. Strauss and Christopher W. Stubbs and Donald W. Sweeney and Alex Szalay and Paula Szkody and Masahiro Takada and Paul Thorman and David E. Trilling and Virginia Trimble and Anthony Tyson and Richard Van Berg and Daniel Vanden Berk and Jake VanderPlas and Licia Verde and Bojan Vrsnak and Lucianne M. Walkowicz and Benjamin D. Wandelt and Sheng Wang and Yun Wang and Michael Warner and Risa H. Wechsler and Andrew A. West and Oliver Wiecha and Benjamin F. Williams and Beth Willman and David Wittman and Sidney C. Wolff and W. Michael Wood-Vasey and Przemek Wozniak and Patrick Young and Andrew Zentner and Hu Zhan},
      year={2009},
      eprint={0912.0201},
      archivePrefix={arXiv},
      primaryClass={astro-ph.IM}
}

@ARTICLE{Limongi2018,
       author = {{Limongi}, Marco and {Chieffi}, Alessandro},
        title = "{Presupernova Evolution and Explosive Nucleosynthesis of Rotating Massive Stars in the Metallicity Range -3 {\ensuremath{\leq}} [Fe/H] {\ensuremath{\leq}} 0}",
      journal = {\apjs},
     keywords = {stars: evolution, stars: interiors, stars: massive, stars: rotation, supernovae: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = jul,
       volume = {237},
       number = {1},
          eid = {13},
        pages = {13},
          doi = {10.3847/1538-4365/aacb24},
archivePrefix = {arXiv},
       eprint = {1805.09640},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..237...13L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{LIGO2023,
  title = {Population of Merging Compact Binaries Inferred Using Gravitational Waves through GWTC-3},
  author = {Abbott, R. and Abbott, T. D. and Acernese, F. and Ackley, K. and Adams, C. and Adhikari, N. and Adhikari, R. X. and Adya, V. B. and Affeldt, C. and Agarwal, D. and Agathos, M. and Agatsuma, K. and Aggarwal, N. and Aguiar, O. D. and Aiello, L. and Ain, A. and Ajith, P. and Akutsu, T. and de Alarc\'on, P. F. and Akcay, S. and Albanesi, S. and Allocca, A. and Altin, P. A. and Amato, A. and Anand, C. and Anand, S. and Ananyeva, A. and Anderson, S. B. and Anderson, W. G. and Ando, M. and Andrade, T. and Andres, N. and Andri\ifmmode \acute{c}\else \'{c}\fi{}, T. and Angelova, S. V. and Ansoldi, S. and Antelis, J. M. and Antier, S. and Antonini, F. and Appert, S. and Arai, Koji and Arai, Koya and Arai, Y. and Araki, S. and Araya, A. and Araya, M. C. and Areeda, J. S. and Ar\`ene, M. and Aritomi, N. and Arnaud, N. and Arogeti, M. and Aronson, S. M. and Arun, K. G. and Asada, H. and Asali, Y. and Ashton, G. and Aso, Y. and Assiduo, M. and Aston, S. M. and Astone, P. and Aubin, F. and Austin, C. and Babak, S. and Badaracco, F. and Bader, M. K. M. and Badger, C. and Bae, S. and Bae, Y. and Baer, A. M. and Bagnasco, S. and Bai, Y. and Baiotti, L. and Baird, J. and Bajpai, R. and Ball, M. and Ballardin, G. and Ballmer, S. W. and Balsamo, A. and Baltus, G. and Banagiri, S. and Bankar, D. and Barayoga, J. C. and Barbieri, C. and Barish, B. C. and Barker, D. and Barneo, P. and Barone, F. and Barr, B. and Barsotti, L. and Barsuglia, M. and Barta, D. and Bartlett, J. and Barton, M. A. and Bartos, I. and Bassiri, R. and Basti, A. and Bawaj, M. and Bayley, J. C. and Baylor, A. C. and Bazzan, M. and B\'ecsy, B. and Bedakihale, V. M. and Bejger, M. and Belahcene, I. and Benedetto, V. and Beniwal, D. and Bennett, T. F. and Bentley, J. D. and BenYaala, M. and Bergamin, F. and Berger, B. K. and Bernuzzi, S. and Berry, C. P. L. and Bersanetti, D. and Bertolini, A. and Betzwieser, J. and Beveridge, D. and Bhandare, R. and Bhardwaj, U. and Bhattacharjee, D. and Bhaumik, S. and Bilenko, I. A. and Billingsley, G. and Bini, S. and Birney, R. and Birnholtz, O. and Biscans, S. and Bischi, M. and Biscoveanu, S. and Bisht, A. and Biswas, B. and Bitossi, M. and Bizouard, M.-A. and Blackburn, J. K. and Blair, C. D. and Blair, D. G. and Blair, R. M. and Bobba, F. and Bode, N. and Boer, M. and Bogaert, G. and Boldrini, M. and Bonavena, L. D. and Bondu, F. and Bonilla, E. and Bonnand, R. and Booker, P. and Boom, B. A. and Bork, R. and Boschi, V. and Bose, N. and Bose, S. and Bossilkov, V. and Boudart, V. and Bouffanais, Y. and Bozzi, A. and Bradaschia, C. and Brady, P. R. and Bramley, A. and Branch, A. and Branchesi, M. and Brandt, J. and Brau, J. E. and Breschi, M. and Briant, T. and Briggs, J. H. and Brillet, A. and Brinkmann, M. and Brockill, P. and Brooks, A. F. and Brooks, J. and Brown, D. D. and Brunett, S. and Bruno, G. and Bruntz, R. and Bryant, J. and Bulik, T. and Bulten, H. J. and Buonanno, A. and Buscicchio, R. and Buskulic, D. and Buy, C. and Byer, R. L. and Cadonati, L. and Cagnoli, G. and Cahillane, C. and Bustillo, J. Calder\'on and Callaghan, J. D. and Callister, T. A. and Calloni, E. and Cameron, J. and Camp, J. B. and Canepa, M. and Canevarolo, S. and Cannavacciuolo, M. and Cannon, K. C. and Cao, H. and Cao, Z. and Capocasa, E. and Capote, E. and Carapella, G. and Carbognani, F. and Carlin, J. B. and Carney, M. F. and Carpinelli, M. and Carrillo, G. and Carullo, G. and Carver, T. L. and Diaz, J. Casanueva and Casentini, C. and Castaldi, G. and Caudill, S. and Cavagli\`a, M. and Cavalier, F. and Cavalieri, R. and Ceasar, M. and Cella, G. and Cerd\'a-Dur\'an, P. and Cesarini, E. and Chaibi, W. and Chakravarti, K. and Subrahmanya, S. Chalathadka and Champion, E. and Chan, C.-H. and Chan, C. and Chan, C. L. and Chan, K. and Chan, M. and Chandra, K. and Chanial, P. and Chao, S. and Chapman-Bird, C. E. A. and Charlton, P. and Chase, E. A. and Chassande-Mottin, E. and Chatterjee, C. and Chatterjee, Debarati and Chatterjee, Deep and Chaturvedi, M. and Chaty, S. and Chatziioannou, K. and Chen, C. and Chen, H. Y. and Chen, J. and Chen, K. and Chen, X. and Chen, Y.-B. and Chen, Y.-R. and Chen, Z. and Cheng, H. and Cheong, C. K. and Cheung, H. Y. and Chia, H. Y. and Chiadini, F. and Chiang, C-Y. and Chiarini, G. and Chierici, R. and Chincarini, A. and Chiofalo, M. L. and Chiummo, A. and Cho, G. and Cho, H. S. and Choudhary, R. K. and Choudhary, S. and Christensen, N. and Chu, H. and Chu, Q. and Chu, Y-K. and Chua, S. and Chung, K. W. and Ciani, G. and Ciecielag, P. and Cie\ifmmode \acute{s}\else \'{s}\fi{}lar, M. and Cifaldi, M. and Ciobanu, A. A. and Ciolfi, R. and Cipriano, F. and Cirone, A. and Clara, F. and Clark, E. N. and Clark, J. A. and Clarke, L. and Clearwater, P. and Clesse, S. and Cleva, F. and Coccia, E. and Codazzo, E. and Cohadon, P.-F. and Cohen, D. E. and Cohen, L. and Colleoni, M. and Collette, C. G. and Colombo, A. and Colpi, M. and Compton, C. M. and Constancio, M. and Conti, L. and Cooper, S. J. and Corban, P. and Corbitt, T. R. and Cordero-Carri\'on, I. and Corezzi, S. and Corley, K. R. and Cornish, N. and Corre, D. and Corsi, A. and Cortese, S. and Costa, C. A. and Cotesta, R. and Coughlin, M. W. and Coulon, J.-P. and Countryman, S. T. and Cousins, B. and Couvares, P. and Coward, D. M. and Cowart, M. J. and Coyne, D. C. and Coyne, R. and Creighton, J. D. E. and Creighton, T. D. and Criswell, A. W. and Croquette, M. and Crowder, S. G. and Cudell, J. R. and Cullen, T. J. and Cumming, A. and Cummings, R. and Cunningham, L. and Cuoco, E. and Cury\l{}o, M. and Dabadie, P. and Canton, T. Dal and Dall'Osso, S. and D\'alya, G. and Dana, A. and DaneshgaranBajastani, L. M. and D'Angelo, B. and Danila, B. and Danilishin, S. and D'Antonio, S. and Danzmann, K. and Darsow-Fromm, C. and Dasgupta, A. and Datrier, L. E. H. and Datta, S. and Dattilo, V. and Dave, I. and Davier, M. and Davies, G. S. and Davis, D. and Davis, M. C. and Daw, E. J. and Dean, R. and DeBra, D. and Deenadayalan, M. and Degallaix, J. and De Laurentis, M. and Del\'eglise, S. and Del Favero, V. and De Lillo, F. and De Lillo, N. and Del Pozzo, W. and DeMarchi, L. M. and De Matteis, F. and D'Emilio, V. and Demos, N. and Dent, T. and Depasse, A. and De Pietri, R. and De Rosa, R. and De Rossi, C. and DeSalvo, R. and De Simone, R. and Dhurandhar, S. and D\'{\i}az, M. C. and Diaz-Ortiz, M. and Didio, N. A. and Dietrich, T. and Di Fiore, L. and Di Fronzo, C. and Di Giorgio, C. and Di Giovanni, F. and Di Giovanni, M. and Di Girolamo, T. and Di Lieto, A. and Ding, B. and Di Pace, S. and Di Palma, I. and Di Renzo, F. and Divakarla, A. K. and Dmitriev, A. and Doctor, Z. and D'Onofrio, L. and Donovan, F. and Dooley, K. L. and Doravari, S. and Dorrington, I. and Drago, M. and Driggers, J. C. and Drori, Y. and Ducoin, J.-G. and Dupej, P. and Durante, O. and D'Urso, D. and Duverne, P.-A. and Dwyer, S. E. and Eassa, C. and Easter, P. J. and Ebersold, M. and Eckhardt, T. and Eddolls, G. and Edelman, B. and Edo, T. B. and Edy, O. and Effler, A. and Eguchi, S. and Eichholz, J. and Eikenberry, S. S. and Eisenmann, M. and Eisenstein, R. A. and Ejlli, A. and Engelby, E. and Enomoto, Y. and Errico, L. and Essick, R. C. and Estell\'es, H. and Estevez, D. and Etienne, Z. and Etzel, T. and Evans, M. and Evans, T. M. and Ewing, B. E. and Fafone, V. and Fair, H. and Fairhurst, S. and Farah, A. M. and Farinon, S. and Farr, B. and Farr, W. M. and Farrow, N. W. and Fauchon-Jones, E. J. and Favaro, G. and Favata, M. and Fays, M. and Fazio, M. and Feicht, J. and Fejer, M. M. and Fenyvesi, E. and Ferguson, D. L. and Fernandez-Galiana, A. and Ferrante, I. and Ferreira, T. A. and Fidecaro, F. and Figura, P. and Fiori, I. and Fishbach, M. and Fisher, R. P. and Fittipaldi, R. and Fiumara, V. and Flaminio, R. and Floden, E. and Fong, H. and Font, J. A. and Fornal, B. and Forsyth, P. W. F. and Franke, A. and Frasca, S. and Frasconi, F. and Frederick, C. and Freed, J. P. and Frei, Z. and Freise, A. and Frey, R. and Fritschel, P. and Frolov, V. V. and Fronz\'e, G. G. and Fujii, Y. and Fujikawa, Y. and Fukunaga, M. and Fukushima, M. and Fulda, P. and Fyffe, M. and Gabbard, H. A. and Gadre, B. U. and Gair, J. R. and Gais, J. and Galaudage, S. and Gamba, R. and Ganapathy, D. and Ganguly, A. and Gao, D. and Gaonkar, S. G. and Garaventa, B. and Garc\'{\i}a, F. and Garc\'{\i}a-N\'u\~nez, C. and Garc\'{\i}a-Quir\'os, C. and Garufi, F. and Gateley, B. and Gaudio, S. and Gayathri, V. and Ge, G.-G. and Gemme, G. and Gennai, A. and George, J. and George, R. N. and Gerberding, O. and Gergely, L. and Gewecke, P. and Ghonge, S. and Ghosh, Abhirup and Ghosh, Archisman and Ghosh, Shaon and Ghosh, Shrobana and Giacomazzo, B. and Giacoppo, L. and Giaime, J. A. and Giardina, K. D. and Gibson, D. R. and Gier, C. and Giesler, M. and Giri, P. and Gissi, F. and Glanzer, J. and Gleckl, A. E. and Godwin, P. and Golomb, J. and Goetz, E. and Goetz, R. and Gohlke, N. and Goncharov, B. and Gonz\'alez, G. and Gopakumar, A. and Gosselin, M. and Gouaty, R. and Gould, D. W. and Grace, B. and Grado, A. and Granata, M. and Granata, V. and Grant, A. and Gras, S. and Grassia, P. and Gray, C. and Gray, R. and Greco, G. and Green, A. C. and Green, R. and Gretarsson, A. M. and Gretarsson, E. M. and Griffith, D. and Griffiths, W. and Griggs, H. L. and Grignani, G. and Grimaldi, A. and Grimm, S. J. and Grote, H. and Grunewald, S. and Gruning, P. and Guerra, D. and Guidi, G. M. and Guimaraes, A. R. and Guix\'e, G. and Gulati, H. K. and Guo, H.-K. and Guo, Y. and Gupta, Anchal and Gupta, Anuradha and Gupta, P. and Gustafson, E. K. and Gustafson, R. and Guzman, F. and Ha, S. and Haegel, L. and Hagiwara, A. and Haino, S. and Halim, O. and Hall, E. D. and Hamilton, E. Z. and Hammond, G. and Han, W.-B. and Haney, M. and Hanks, J. and Hanna, C. and Hannam, M. D. and Hannuksela, O. and Hansen, H. and Hansen, T. J. and Hanson, J. and Harder, T. and Hardwick, T. and Haris, K. and Harms, J. and Harry, G. M. and Harry, I. W. and Hartwig, D. and Hasegawa, K. and Haskell, B. and Hasskew, R. K. and Haster, C.-J. and Hattori, K. and Haughian, K. and Hayakawa, H. and Hayama, K. and Hayes, F. J. and Healy, J. and Heidmann, A. and Heidt, A. and Heintze, M. C. and Heinze, J. and Heinzel, J. and Heitmann, H. and Hellman, F. and Hello, P. and Helmling-Cornell, A. F. and Hemming, G. and Hendry, M. and Heng, I. S. and Hennes, E. and Hennig, J. and Hennig, M. H. and Hernandez, A. G. and Vivanco, F. Hernandez and Heurs, M. and Hild, S. and Hill, P. and Himemoto, Y. and Hines, A. S. and Hiranuma, Y. and Hirata, N. and Hirose, E. and Hochheim, S. and Hofman, D. and Hohmann, J. N. and Holcomb, D. G. and Holland, N. A. and Hollows, I. J. and Holmes, Z. J. and Holt, K. and Holz, D. E. and Hong, Z. and Hopkins, P. and Hough, J. and Hourihane, S. and Howell, E. J. and Hoy, C. G. and Hoyland, D. and Hreibi, A. and Hsieh, B-H. and Hsu, Y. and Huang, G-Z. and Huang, H-Y. and Huang, P. and Huang, Y-C. and Huang, Y.-J. and Huang, Y. and H\"ubner, M. T. and Huddart, A. D. and Hughey, B. and Hui, D. C. Y. and Hui, V. and Husa, S. and Huttner, S. H. and Huxford, R. and Huynh-Dinh, T. and Ide, S. and Idzkowski, B. and Iess, A. and Ikenoue, B. and Imam, S. and Inayoshi, K. and Ingram, C. and Inoue, Y. and Ioka, K. and Isi, M. and Isleif, K. and Ito, K. and Itoh, Y. and Iyer, B. R. and Izumi, K. and JaberianHamedan, V. and Jacqmin, T. and Jadhav, S. J. and Jadhav, S. P. and James, A. L. and Jan, A. Z. and Jani, K. and Janquart, J. and Janssens, K. and Janthalur, N. N. and Jaranowski, P. and Jariwala, D. and Jaume, R. and Jenkins, A. C. and Jenner, K. and Jeon, C. and Jeunon, M. and Jia, W. and Jin, H.-B. and Johns, G. R. and Jones, A. W. and Jones, D. I. and Jones, J. D. and Jones, P. and Jones, R. and Jonker, R. J. G. and Ju, L. and Jung, P. and Jung, k. and Junker, J. and Juste, V. and Kaihotsu, K. and Kajita, T. and Kakizaki, M. and Kalaghatgi, C. V. and Kalogera, V. and Kamai, B. and Kamiizumi, M. and Kanda, N. and Kandhasamy, S. and Kang, G. and Kanner, J. B. and Kao, Y. and Kapadia, S. J. and Kapasi, D. P. and Karat, S. and Karathanasis, C. and Karki, S. and Kashyap, R. and Kasprzack, M. and Kastaun, W. and Katsanevas, S. and Katsavounidis, E. and Katzman, W. and Kaur, T. and Kawabe, K. and Kawaguchi, K. and Kawai, N. and Kawasaki, T. and K\'ef\'elian, F. and Keitel, D. and Key, J. S. and Khadka, S. and Khalili, F. Y. and Khan, S. and Khazanov, E. A. and Khetan, N. and Khursheed, M. and Kijbunchoo, N. and Kim, C. and Kim, J. C. and Kim, J. and Kim, K. and Kim, W. S. and Kim, Y.-M. and Kimball, C. and Kimura, N. and Kinley-Hanlon, M. and Kirchhoff, R. and Kissel, J. S. and Kita, N. and Kitazawa, H. and Kleybolte, L. and Klimenko, S. and Knee, A. M. and Knowles, T. D. and Knyazev, E. and Koch, P. and Koekoek, G. and Kojima, Y. and Kokeyama, K. and Koley, S. and Kolitsidou, P. and Kolstein, M. and Komori, K. and Kondrashov, V. and Kong, A. K. H. and Kontos, A. and Koper, N. and Korobko, M. and Kotake, K. and Kovalam, M. and Kozak, D. B. and Kozakai, C. and Kozu, R. and Kringel, V. and Krishnendu, N. V. and Kr\'olak, A. and Kuehn, G. and Kuei, F. and Kuijer, P. and Kulkarni, S. and Kumar, A. and Kumar, P. and Kumar, Rahul and Kumar, Rakesh and Kume, J. and Kuns, K. and Kuo, C. and Kuo, H-S. and Kuromiya, Y. and Kuroyanagi, S. and Kusayanagi, K. and Kuwahara, S. and Kwak, K. and Lagabbe, P. and Laghi, D. and Lalande, E. and Lam, T. L. and Lamberts, A. and Landry, M. and Landry, P. and Lane, B. B. and Lang, R. N. and Lange, J. and Lantz, B. and La Rosa, I. and Lartaux-Vollard, A. and Lasky, P. D. and Laxen, M. and Lazzarini, A. and Lazzaro, C. and Leaci, P. and Leavey, S. and Lecoeuche, Y. K. and Lee, H. K. and Lee, H. M. and Lee, H. W. and Lee, J. and Lee, K. and Lee, R. and Lehmann, J. and Lema\^{\i}tre, A. and Leonardi, M. and Leroy, N. and Letendre, N. and Levesque, C. and Levin, Y. and Leviton, J. N. and Leyde, K. and Li, A. K. Y. and Li, B. and Li, J. and Li, K. L. and Li, T. G. F. and Li, X. and Lin, C-Y. and Lin, F-K. and Lin, F-L. and Lin, H. L. and Lin, L. C.-C. and Linde, F. and Linker, S. D. and Linley, J. N. and Littenberg, T. B. and Liu, G. C. and Liu, J. and Liu, K. and Liu, X. and Llamas, F. and Llorens-Monteagudo, M. and Lo, R. K. L. and Lockwood, A. and Loh, M. and London, L. T. and Longo, A. and Lopez, D. and Portilla, M. Lopez and Lorenzini, M. and Loriette, V. and Lormand, M. and Losurdo, G. and Lott, T. P. and Lough, J. D. and Lousto, C. O. and Lovelace, G. and Lucaccioni, J. F. and L\"uck, H. and Lumaca, D. and Lundgren, A. P. and Luo, L.-W. and Lynam, J. E. and Macas, R. and MacInnis, M. and Macleod, D. M. and MacMillan, I. A. O. and Macquet, A. and Hernandez, I. Maga\~na and Magazz\`u, C. and Magee, R. M. and Maggiore, R. and Magnozzi, M. and Mahesh, S. and Majorana, E. and Makarem, C. and Maksimovic, I. and Maliakal, S. and Malik, A. and Man, N. and Mandic, V. and Mangano, V. and Mango, J. L. and Mansell, G. L. and Manske, M. and Mantovani, M. and Mapelli, M. and Marchesoni, F. and Marchio, M. and Marion, F. and Mark, Z. and M\'arka, S. and M\'arka, Z. and Markakis, C. and Markosyan, A. S. and Markowitz, A. and Maros, E. and Marquina, A. and Marsat, S. and Martelli, F. and Martin, I. W. and Martin, R. M. and Martinez, M. and Martinez, V. A. and Martinez, V. and Martinovic, K. and Martynov, D. V. and Marx, E. J. and Masalehdan, H. and Mason, K. and Massera, E. and Masserot, A. and Massinger, T. J. and Masso-Reid, M. and Mastrogiovanni, S. and Matas, A. and Mateu-Lucena, M. and Matichard, F. and Matiushechkina, M. and Mavalvala, N. and McCann, J. J. and McCarthy, R. and McClelland, D. E. and McClincy, P. K. and McCormick, S. and McCuller, L. and McGhee, G. I. and McGuire, S. C. and McIsaac, C. and McIver, J. and McRae, T. and McWilliams, S. T. and Meacher, D. and Mehmet, M. and Mehta, A. K. and Meijer, Q. and Melatos, A. and Melchor, D. A. and Mendell, G. and Menendez-Vazquez, A. and Menoni, C. S. and Mercer, R. A. and Mereni, L. and Merfeld, K. and Merilh, E. L. and Merritt, J. D. and Merzougui, M. and Meshkov, S. and Messenger, C. and Messick, C. and Meyers, P. M. and Meylahn, F. and Mhaske, A. and Miani, A. and Miao, H. and Michaloliakos, I. and Michel, C. and Michimura, Y. and Middleton, H. and Milano, L. and Miller, A. L. and Miller, A. and Miller, B. and Miller, S. and Millhouse, M. and Mills, J. C. and Milotti, E. and Minazzoli, O. and Minenkov, Y. and Mio, N. and Mir, Ll. M. and Miravet-Ten\'es, M. and Mishra, C. and Mishra, T. and Mistry, T. and Mitra, S. and Mitrofanov, V. P. and Mitselmakher, G. and Mittleman, R. and Miyakawa, O. and Miyamoto, A. and Miyazaki, Y. and Miyo, K. and Miyoki, S. and Mo, Geoffrey and Modafferi, L. M. and Moguel, E. and Mogushi, K. and Mohapatra, S. R. P. and Mohite, S. R. and Molina, I. and Molina-Ruiz, M. and Mondin, M. and Montani, M. and Moore, C. J. and Moraru, D. and Morawski, F. and More, A. and Moreno, C. and Moreno, G. and Mori, Y. and Morisaki, S. and Moriwaki, Y. and Morr\'as, G. and Mours, B. and Mow-Lowry, C. M. and Mozzon, S. and Muciaccia, F. and Mukherjee, Arunava and Mukherjee, D. and Mukherjee, Soma and Mukherjee, Subroto and Mukherjee, Suvodip and Mukund, N. and Mullavey, A. and Munch, J. and Mu\~niz, E. A. and Murray, P. G. and Musenich, R. and Muusse, S. and Nadji, S. L. and Nagano, K. and Nagano, S. and Nagar, A. and Nakamura, K. and Nakano, H. and Nakano, M. and Nakashima, R. and Nakayama, Y. and Napolano, V. and Nardecchia, I. and Narikawa, T. and Naticchioni, L. and Nayak, B. and Nayak, R. K. and Negishi, R. and Neil, B. F. and Neilson, J. and Nelemans, G. and Nelson, T. J. N. and Nery, M. and Neubauer, P. and Neunzert, A. and Ng, K. Y. and Ng, S. W. S. and Nguyen, C. and Nguyen, P. and Nguyen, T. and Quynh, L. Nguyen and Ni, W.-T. and Nichols, S. A. and Nishizawa, A. and Nissanke, S. and Nitoglia, E. and Nocera, F. and Norman, M. and North, C. and Nozaki, S. and Siles, J. F. Nu\~no and Nuttall, L. K. and Oberling, J. and O'Brien, B. D. and Obuchi, Y. and O'Dell, J. and Oelker, E. and Ogaki, W. and Oganesyan, G. and Oh, J. J. and Oh, K. and Oh, S. H. and Ohashi, M. and Ohishi, N. and Ohkawa, M. and Ohme, F. and Ohta, H. and Okada, M. A. and Okutani, Y. and Okutomi, K. and Olivetto, C. and Oohara, K. and Ooi, C. and Oram, R. and O'Reilly, B. and Ormiston, R. G. and Ormsby, N. D. and Ortega, L. F. and O'Shaughnessy, R. and O'Shea, E. and Oshino, S. and Ossokine, S. and Osthelder, C. and Otabe, S. and Ottaway, D. J. and Overmier, H. and Pace, A. E. and Pagano, G. and Page, M. A. and Pagliaroli, G. and Pai, A. and Pai, S. A. and Palamos, J. R. and Palashov, O. and Palomba, C. and Pan, H. and Pan, K. and Panda, P. K. and Pang, H. and Pang, P. T. H. and Pankow, C. and Pannarale, F. and Pant, B. C. and Panther, F. H. and Paoletti, F. and Paoli, A. and Paolone, A. and Parisi, A. and Park, H. and Park, J. and Parker, W. and Pascucci, D. and Pasqualetti, A. and Passaquieti, R. and Passuello, D. and Patel, M. and Pathak, M. and Patricelli, B. and Patron, A. S. and Paul, S. and Payne, E. and Pedraza, M. and Pegoraro, M. and Pele, A. and Arellano, F. E. Pe\~na and Penn, S. and Perego, A. and Pereira, A. and Pereira, T. and Perez, C. J. and P\'erigois, C. and Perkins, C. C. and Perreca, A. and Perri\`es, S. and Petermann, J. and Petterson, D. and Pfeiffer, H. P. and Pham, K. A. and Phukon, K. S. and Piccinni, O. J. and Pichot, M. and Piendibene, M. and Piergiovanni, F. and Pierini, L. and Pierro, V. and Pillant, G. and Pillas, M. and Pilo, F. and Pinard, L. and Pinto, I. M. and Pinto, M. and Piotrzkowski, B. and Piotrzkowski, K. and Pirello, M. and Pitkin, M. D. and Placidi, E. and Planas, L. and Plastino, W. and Pluchar, C. and Poggiani, R. and Polini, E. and Pong, D. Y. T. and Ponrathnam, S. and Popolizio, P. and Porter, E. K. and Poulton, R. and Powell, J. and Pracchia, M. and Pradier, T. and Prajapati, A. K. and Prasai, K. and Prasanna, R. and Pratten, G. and Principe, M. and Prodi, G. A. and Prokhorov, L. and Prosposito, P. and Prudenzi, L. and Puecher, A. and Punturo, M. and Puosi, F. and Puppo, P. and P\"urrer, M. and Qi, H. and Quetschke, V. and Quitzow-James, R. and Raab, F. J. and Raaijmakers, G. and Radkins, H. and Radulesco, N. and Raffai, P. and Rail, S. X. and Raja, S. and Rajan, C. and Ramirez, K. E. and Ramirez, T. D. and Ramos-Buades, A. and Rana, J. and Rapagnani, P. and Rapol, U. D. and Ray, A. and Raymond, V. and Raza, N. and Razzano, M. and Read, J. and Rees, L. A. and Regimbau, T. and Rei, L. and Reid, S. and Reid, S. W. and Reitze, D. H. and Relton, P. and Renzini, A. and Rettegno, P. and Reza, A. and Rezac, M. and Ricci, F. and Richards, D. and Richardson, J. W. and Richardson, L. and Riemenschneider, G. and Riles, K. and Rinaldi, S. and Rink, K. and Rizzo, M. and Robertson, N. A. and Robie, R. and Robinet, F. and Rocchi, A. and Rodriguez, S. and Rolland, L. and Rollins, J. G. and Romanelli, M. and Romano, R. and Romel, C. L. and Romero-Rodr\'{\i}guez, A. and Romero-Shaw, I. M. and Romie, J. H. and Ronchini, S. and Rosa, L. and Rose, C. A. and Rosi\ifmmode \acute{n}\else \'{n}\fi{}ska, D. and Ross, M. P. and Rowan, S. and Rowlinson, S. J. and Roy, S. and Roy, Santosh and Roy, Soumen and Rozza, D. and Ruggi, P. and Ryan, K. and Sachdev, S. and Sadecki, T. and Sadiq, J. and Sago, N. and Saito, S. and Saito, Y. and Sakai, K. and Sakai, Y. and Sakellariadou, M. and Sakuno, Y. and Salafia, O. S. and Salconi, L. and Saleem, M. and Salemi, F. and Samajdar, A. and Sanchez, E. J. and Sanchez, J. H. and Sanchez, L. E. and Sanchis-Gual, N. and Sanders, J. R. and Sanuy, A. and Saravanan, T. R. and Sarin, N. and Sassolas, B. and Satari, H. and Sathyaprakash, B. S. and Sato, S. and Sato, T. and Sauter, O. and Savage, R. L. and Sawada, T. and Sawant, D. and Sawant, H. L. and Sayah, S. and Schaetzl, D. and Scheel, M. and Scheuer, J. and Schiworski, M. and Schmidt, P. and Schmidt, S. and Schnabel, R. and Schneewind, M. and Schofield, R. M. S. and Sch\"onbeck, A. and Schulte, B. W. and Schutz, B. F. and Schwartz, E. and Scott, J. and Scott, S. M. and Seglar-Arroyo, M. and Sekiguchi, T. and Sekiguchi, Y. and Sellers, D. and Sengupta, A. S. and Sentenac, D. and Seo, E. G. and Sequino, V. and Sergeev, A. and Setyawati, Y. and Shaffer, T. and Shahriar, M. S. and Shams, B. and Shao, L. and Sharma, A. and Sharma, P. and Shawhan, P. and Shcheblanov, N. S. and Shibagaki, S. and Shikauchi, M. and Shimizu, R. and Shimoda, T. and Shimode, K. and Shinkai, H. and Shishido, T. and Shoda, A. and Shoemaker, D. H. and Shoemaker, D. M. and ShyamSundar, S. and Sieniawska, M. and Sigg, D. and Singer, L. P. and Singh, D. and Singh, N. and Singha, A. and Sintes, A. M. and Sipala, V. and Skliris, V. and Slagmolen, B. J. J. and Slaven-Blair, T. J. and Smetana, J. and Smith, J. R. and Smith, R. J. E. and Soldateschi, J. and Somala, S. N. and Somiya, K. and Son, E. J. and Soni, K. and Soni, S. and Sordini, V. and Sorrentino, F. and Sorrentino, N. and Sotani, H. and Soulard, R. and Souradeep, T. and Sowell, E. and Spagnuolo, V. and Spencer, A. P. and Spera, M. and Srinivasan, R. and Srivastava, A. K. and Srivastava, V. and Staats, K. and Stachie, C. and Steer, D. A. and Steinhoff, J. and Steinlechner, J. and Steinlechner, S. and Stevenson, S. P. and Stops, D. J. and Stover, M. and Strain, K. A. and Strang, L. C. and Stratta, G. and Strunk, A. and Sturani, R. and Stuver, A. L. and Sudhagar, S. and Sudhir, V. and Sugimoto, R. and Suh, H. G. and Sullivan, A. G. and Summerscales, T. Z. and Sun, H. and Sun, L. and Sunil, S. and Sur, A. and Suresh, J. and Sutton, P. J. and Suzuki, Takamasa and Suzuki, Toshikazu and Swinkels, B. L. and Szczepa\ifmmode \acute{n}\else \'{n}\fi{}czyk, M. J. and Szewczyk, P. and Tacca, M. and Tagoshi, H. and Tait, S. C. and Takahashi, H. and Takahashi, R. and Takamori, A. and Takano, S. and Takeda, H. and Takeda, M. and Talbot, C. J. and Talbot, C. and Tanaka, H. and Tanaka, Kazuyuki and Tanaka, Kenta and Tanaka, Taiki and Tanaka, Takahiro and Tanasijczuk, A. J. and Tanioka, S. and Tanner, D. B. and Tao, D. and Tao, L. and Mart\'{\i}n, E. N. Tapia San and Taranto, C. and Tasson, J. D. and Telada, S. and Tenorio, R. and Terhune, J. E. and Terkowski, L. and Thirugnanasambandam, M. P. and Thomas, L. and Thomas, M. and Thomas, P. and Thompson, J. E. and Thondapu, S. R. and Thorne, K. A. and Thrane, E. and Tiwari, Shubhanshu and Tiwari, Srishti and Tiwari, V. and Toivonen, A. M. and Toland, K. and Tolley, A. E. and Tomaru, T. and Tomigami, Y. and Tomura, T. and Tonelli, M. and Torres-Forn\'e, A. and Torrie, C. I. and e Melo, I. Tosta and T\"oyr\"a, D. and Trapananti, A. and Travasso, F. and Traylor, G. and Trevor, M. and Tringali, M. C. and Tripathee, A. and Troiano, L. and Trovato, A. and Trozzo, L. and Trudeau, R. J. and Tsai, D. S. and Tsai, D. and Tsang, K. W. and Tsang, T. and Tsao, J-S. and Tse, M. and Tso, R. and Tsubono, K. and Tsuchida, S. and Tsukada, L. and Tsuna, D. and Tsutsui, T. and Tsuzuki, T. and Turbang, K. and Turconi, M. and Tuyenbayev, D. and Ubhi, A. S. and Uchikata, N. and Uchiyama, T. and Udall, R. P. and Ueda, A. and Uehara, T. and Ueno, K. and Ueshima, G. and Unnikrishnan, C. S. and Uraguchi, F. and Urban, A. L. and Ushiba, T. and Utina, A. and Vahlbruch, H. and Vajente, G. and Vajpeyi, A. and Valdes, G. and Valentini, M. and Valsan, V. and van Bakel, N. and van Beuzekom, M. and van den Brand, J. F. J. and Van Den Broeck, C. and Vander-Hyde, D. C. and van der Schaaf, L. and van Heijningen, J. V. and Vanosky, J. and van Putten, M. H. P. M. and van Remortel, N. and Vardaro, M. and Vargas, A. F. and Varma, V. and Vas\'uth, M. and Vecchio, A. and Vedovato, G. and Veitch, J. and Veitch, P. J. and Venneberg, J. and Venugopalan, G. and Verkindt, D. and Verma, P. and Verma, Y. and Veske, D. and Vetrano, F. and Vicer\'e, A. and Vidyant, S. and Viets, A. D. and Vijaykumar, A. and Villa-Ortega, V. and Vinet, J.-Y. and Virtuoso, A. and Vitale, S. and Vo, T. and Vocca, H. and von Reis, E. R. G. and von Wrangel, J. S. A. and Vorvick, C. and Vyatchanin, S. P. and Wade, L. E. and Wade, M. and Wagner, K. J. and Walet, R. C. and Walker, M. and Wallace, G. S. and Wallace, L. and Walsh, S. and Wang, J. and Wang, J. Z. and Wang, W. H. and Ward, R. L. and Warner, J. and Was, M. and Washimi, T. and Washington, N. Y. and Watchi, J. and Weaver, B. and Webster, S. A. and Weinert, M. and Weinstein, A. J. and Weiss, R. and Weller, C. M. and Wellmann, F. and Wen, L. and We\ss{}els, P. and Wette, K. and Whelan, J. T. and White, D. D. and Whiting, B. F. and Whittle, C. and Wilken, D. and Williams, D. and Williams, M. J. and Williamson, A. R. and Willis, J. L. and Willke, B. and Wilson, D. J. and Winkler, W. and Wipf, C. C. and Wlodarczyk, T. and Woan, G. and Woehler, J. and Wofford, J. K. and Wong, I. C. F. and Wu, C. and Wu, D. S. and Wu, H. and Wu, S. and Wysocki, D. M. and Xiao, L. and Xu, W-R. and Yamada, T. and Yamamoto, H. and Yamamoto, Kazuhiro and Yamamoto, Kohei and Yamamoto, T. and Yamashita, K. and Yamazaki, R. and Yang, F. W. and Yang, L. and Yang, Y. and Yang, Yang and Yang, Z. and Yap, M. J. and Yeeles, D. W. and Yelikar, A. B. and Ying, M. and Yokogawa, K. and Yokoyama, J. and Yokozawa, T. and Yoo, J. and Yoshioka, T. and Yu, Hang and Yu, Haocun and Yuzurihara, H. and Zadro\ifmmode \dot{z}\else \.{z}\fi{}ny, A. and Zanolin, M. and Zeidler, S. and Zelenova, T. and Zendri, J.-P. and Zevin, M. and Zhan, M. and Zhang, H. and Zhang, J. and Zhang, L. and Zhang, T. and Zhang, Y. and Zhao, C. and Zhao, G. and Zhao, Y. and Zhao, Yue and Zheng, Y. and Zhou, R. and Zhou, Z. and Zhu, X. J. and Zhu, Z.-H. and Zimmerman, A. B. and Zlochower, Y. and Zucker, M. E. and Zweizig, J.},
  collaboration = {LIGO Scientific Collaboration, Virgo Collaboration, and KAGRA Collaboration},
  journal = {Phys. Rev. X},
  volume = {13},
  issue = {1},
  pages = {011048},
  numpages = {75},
  year = {2023},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.13.011048},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.13.011048}
}


% -------------------------- M --------------------------
@ARTICLE{Munakata1985,
       author = {{Munakata}, H. and {Kohyama}, Y. and {Itoh}, N.},
        title = "{Neutrino Energy Loss in Stellar Interiors}",
      journal = {\apj},
     keywords = {Energy Dissipation, Neutrinos, Pair Production, Stellar Evolution, Stellar Interiors, Stellar Structure, Bremsstrahlung, Integral Equations, Astrophysics},
         year = 1985,
        month = sep,
       volume = {296},
        pages = {197},
          doi = {10.1086/163436},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1985ApJ...296..197M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Massey2001,
       author = {{Massey}, Philip and {DeGioia-Eastwood}, Kathleen and {Waterhouse}, Elizabeth},
        title = "{The Progenitor Masses of Wolf-Rayet Stars and Luminous Blue Variables Determined from Cluster Turnoffs. II. Results from 12 Galactic Clusters and OB Associations}",
      journal = {\aj},
     keywords = {Galaxy: Open Clusters and Associations: General, Stars: Early-Type, Stars: Evolution, Stars: Wolf-Rayet, Astrophysics},
         year = 2001,
        month = feb,
       volume = {121},
       number = {2},
        pages = {1050-1070},
          doi = {10.1086/318769},
archivePrefix = {arXiv},
       eprint = {astro-ph/0010654},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001AJ....121.1050M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2001A&A...371..152M,
       author = {{Marigo}, P. and {Girardi}, L. and {Chiosi}, C. and {Wood}, P.~R.},
        title = "{Zero-metallicity stars. I. Evolution at constant mass}",
      journal = {\aap},
     keywords = {STARS: EVOLUTION, STARS: INTERIORS, STARS: HERTZSPRUNG-RUSSELL (HR) DIAGRAM, STARS: LOW-MASS, Astrophysics},
         year = 2001,
        month = may,
       volume = {371},
        pages = {152-173},
          doi = {10.1051/0004-6361:20010309},
archivePrefix = {arXiv},
       eprint = {astro-ph/0102253},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...371..152M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Marigo2001,
       author = {{Marigo}, P. and {Girardi}, L. and {Chiosi}, C. and {Wood}, P.~R.},
        title = "{Zero-metallicity stars. I. Evolution at constant mass}",
      journal = {\aap},
     keywords = {STARS: EVOLUTION, STARS: INTERIORS, STARS: HERTZSPRUNG-RUSSELL (HR) DIAGRAM, STARS: LOW-MASS, Astrophysics},
         year = 2001,
        month = may,
       volume = {371},
        pages = {152-173},
          doi = {10.1051/0004-6361:20010309},
archivePrefix = {arXiv},
       eprint = {astro-ph/0102253},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...371..152M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Marigo2009,
       author = {{Marigo}, P. and {Aringer}, B.},
        title = "{Low-temperature gas opacity. {\AE}SOPUS: a versatile and quick computational tool}",
      journal = {\aap},
     keywords = {equation of state, atomic processes, molecular processes, stars: abundances, stars: atmospheres, stars: AGB and post-AGB, Astrophysics - Solar and Stellar Astrophysics},
         year = 2009,
        month = dec,
       volume = {508},
       number = {3},
        pages = {1539-1569},
          doi = {10.1051/0004-6361/200912598},
archivePrefix = {arXiv},
       eprint = {0907.3248},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A&A...508.1539M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Marigo2013,
    author = {Marigo, Paola and Bressan, Alessandro and Nanni, Ambra and Girardi, Léo and Pumo, Maria Letizia},
    title = "{Evolution of thermally pulsing asymptotic giant branch stars – I. The colibri code}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {434},
    number = {1},
    pages = {488-526},
    year = {2013},
    month = {07},
    issn = {0035-8711},
    doi = {10.1093/mnras/stt1034},
    url = {https://doi.org/10.1093/mnras/stt1034},
    eprint = {https://academic.oup.com/mnras/article-pdf/434/1/488/18500845/stt1034.pdf},
}
@ARTICLE{Mapelli2020,
       author = {{Mapelli}, Michela and {Spera}, Mario and {Montanari}, Enrico and {Limongi}, Marco and {Chieffi}, Alessandro and {Giacobbo}, Nicola and {Bressan}, Alessandro and {Bouffanais}, Yann},
        title = "{Impact of the Rotation and Compactness of Progenitors on the Mass of Black Holes}",
      journal = {\apj},
     keywords = {Astrophysical black holes, Stellar mass black holes, Stellar mass loss, Computational methods, Gravitational wave astronomy, Massive stars, 98, 1611, 1613, 1965, 675, 732, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = jan,
       volume = {888},
       number = {2},
          eid = {76},
        pages = {76},
          doi = {10.3847/1538-4357/ab584d10.48550/arXiv.1909.01371},
archivePrefix = {arXiv},
       eprint = {1909.01371},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...888...76M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Miller-Jones2021,
       author = {{Miller-Jones}, James C.~A. and {Bahramian}, Arash and {Orosz}, Jerome A. and {Mandel}, Ilya and {Gou}, Lijun and {Maccarone}, Thomas J. and {Neijssel}, Coenraad J. and {Zhao}, Xueshan and {Zi{\'o}{\l}kowski}, Janusz and {Reid}, Mark J. and {Uttley}, Phil and {Zheng}, Xueying and {Byun}, Do-Young and {Dodson}, Richard and {Grinberg}, Victoria and {Jung}, Taehyun and {Kim}, Jeong-Sook and {Marcote}, Benito and {Markoff}, Sera and {Rioja}, Mar{\'\i}a J. and {Rushton}, Anthony P. and {Russell}, David M. and {Sivakoff}, Gregory R. and {Tetarenko}, Alexandra J. and {Tudose}, Valeriu and {Wilms}, Joern},
        title = "{Cygnus X-1 contains a 21-solar mass black hole{\textemdash}Implications for massive star winds}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = mar,
       volume = {371},
       number = {6533},
        pages = {1046-1049},
          doi = {10.1126/science.abb3363},
archivePrefix = {arXiv},
       eprint = {2102.09091},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021Sci...371.1046M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Matteucci2021,
       author = {{Matteucci}, Francesca},
        title = "{Modelling the chemical evolution of the Milky Way}",
      journal = {\aapr},
     keywords = {The Galaxy, Chemical evolution, Chemical abundances, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = dec,
       volume = {29},
       number = {1},
          eid = {5},
        pages = {5},
          doi = {10.1007/s00159-021-00133-8},
archivePrefix = {arXiv},
       eprint = {2106.13145},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&ARv..29....5M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Mestric2023,
       author = {{Me{\v{s}}tri{\'c}}, U. and {Vanzella}, E. and {Upadhyaya}, A. and {Martins}, F. and {Marques-Chaves}, R. and {Schaerer}, D. and {Guibert}, J. and {Zanella}, A. and {Grillo}, C. and {Rosati}, P. and {Calura}, F. and {Caminha}, G.~B. and {Bolamperti}, A. and {Meneghetti}, M. and {Bergamini}, P. and {Mercurio}, A. and {Nonino}, M. and {Pascale}, R.},
        title = "{Clues on the presence and segregation of very massive stars in the Sunburst Lyman-continuum cluster at z = 2.37}",
      journal = {\aap},
     keywords = {stars: massive, Galaxy: stellar content, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = may,
       volume = {673},
          eid = {A50},
        pages = {A50},
          doi = {10.1051/0004-6361/202345895},
archivePrefix = {arXiv},
       eprint = {2301.04672},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A&A...673A..50M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Martins2023b,
       author = {{Martins}, F. and {Schaerer}, D. and {Marques-Chaves}, R. and {Upadhyaya}, A.},
        title = "{Inferring the presence of very massive stars in local star-forming regions}",
      journal = {\aap},
     keywords = {stars: massive, galaxies: starburst, galaxies: stellar content},
         year = 2023,
        month = oct,
       volume = {678},
          eid = {A159},
        pages = {A159},
          doi = {10.1051/0004-6361/202346732},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A&A...678A.159M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


% -------------------------- N --------------------------
@ARTICLE{NugisLamers2000,
       author = {{Nugis}, T. and {Lamers}, H.~J.~G.~L.~M.},
        title = "{Mass-loss rates of Wolf-Rayet stars as a function of stellar parameters}",
      journal = {\aap},
     keywords = {STARS: ATMOSPHERES, STARS: MASS-LOSS, STARS: EMISSION-LINE, BE, STARS: EVOLUTION, STARS: WOLF-RAYET},
         year = 2000,
        month = aug,
       volume = {360},
        pages = {227-244},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&A...360..227N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Nguyen2022,
       author = {{Nguyen}, C.~T. and {Costa}, G. and {Girardi}, L. and {Volpato}, G. and {Bressan}, A. and {Chen}, Y. and {Marigo}, P. and {Fu}, X. and {Goudfrooij}, P.},
        title = "{PARSEC V2.0: Stellar tracks and isochrones of low- and intermediate-mass stars with rotation}",
      journal = {\aap},
     keywords = {stars: evolution, stars: rotation, Hertzsprung-Russell and C-M diagrams, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = sep,
       volume = {665},
          eid = {A126},
        pages = {A126},
          doi = {10.1051/0004-6361/202244166},
archivePrefix = {arXiv},
       eprint = {2207.08642},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A&A...665A.126N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Nayak2023,
       author = {{Nayak}, Omnarayani and {Green}, Alex and {Hirschauer}, Alec S. and {Indebetouw}, R{\'e}my and {Meixner}, Margaret and {Wong}, Tony and {Chevance}, M{\'e}lanie and {De Marchi}, Guido and {Lebouteiller}, Vianney and {Lee}, Min-Young and {Looney}, Leslie W. and {Madden}, Suzanne C. and {Roman-Duval}, Julia and {Fukui}, Yasuo and {Hacar}, Alvaro and {Jameson}, K.~E. and {Kalari}, Venu and {Oudshoorn}, Luuk and {Rubio}, M{\'o}nica and {Sabbi}, Elena},
        title = "{Massive Star Formation in the Tarantula Nebula}",
      journal = {\apj},
     keywords = {Star formation, Interstellar medium, Young stellar objects, 1569, 847, 1834},
         year = 2023,
        month = feb,
       volume = {944},
       number = {1},
          eid = {26},
        pages = {26},
          doi = {10.3847/1538-4357/acac8b},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023ApJ...944...26N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


% -------------------------- O --------------------------
@ARTICLE{Ohkubo2009,
       author = {{Ohkubo}, Takuya and {Nomoto}, Ken'ichi and {Umeda}, Hideyuki and {Yoshida}, Naoki and {Tsuruta}, Sachiko},
        title = "{Evolution of Very Massive Population III Stars with Mass Accretion from Pre-main Sequence to Collapse}",
      journal = {\apj},
     keywords = {accretion, accretion disks, nuclear reactions, nucleosynthesis, abundances, stars: abundances, stars: evolution, stars: formation, supernovae: general, Astrophysics - Solar and Stellar Astrophysics},
         year = 2009,
        month = dec,
       volume = {706},
       number = {2},
        pages = {1184-1193},
          doi = {10.1088/0004-637X/706/2/1184},
archivePrefix = {arXiv},
       eprint = {0902.4573},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...706.1184O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
% -------------------------- P --------------------------

@ARTICLE{Panuzzo2003,
       author = {{Panuzzo}, P. and {Bressan}, A. and {Granato}, G.~L. and {Silva}, L. and {Danese}, L.},
        title = "{Dust and nebular emission. I. Models for normal galaxies}",
      journal = {\aap},
     keywords = {ISM: HII regions, galaxies: ISM, stars: formation, galaxies: evolution, Astrophysics},
         year = 2003,
        month = oct,
       volume = {409},
        pages = {99-114},
          doi = {10.1051/0004-6361:20031094},
archivePrefix = {arXiv},
       eprint = {astro-ph/0307096},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...409...99P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Paxton2011,
       author = {{Paxton}, Bill and {Bildsten}, Lars and {Dotter}, Aaron and {Herwig}, Falk and {Lesaffre}, Pierre and {Timmes}, Frank},
        title = "{Modules for Experiments in Stellar Astrophysics (MESA)}",
      journal = {\apjs},
     keywords = {methods: numerical, stars: evolution, stars: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = jan,
       volume = {192},
       number = {1},
          eid = {3},
        pages = {3},
          doi = {10.1088/0067-0049/192/1/3},
archivePrefix = {arXiv},
       eprint = {1009.1622},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJS..192....3P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Prantzos2018,
    author = {Prantzos, N and Abia, C and Limongi, M and Chieffi, A and Cristallo, S},
    title = "{Chemical evolution with rotating massive star yields – I. The solar neighbourhood and the s-process elements}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {476},
    number = {3},
    pages = {3432-3459},
    year = {2018},
    month = {02},
    abstract = "{}",
    issn = {0035-8711},
    doi = {10.1093/mnras/sty316},
    url = {https://doi.org/10.1093/mnras/sty316},
    eprint = {https://academic.oup.com/mnras/article-pdf/476/3/3432/24502702/sty316.pdf},
}

% -------------------------- R --------------------------
@ARTICLE{Renzo2017,
       author = {{Renzo}, M. and {Ott}, C.~D. and {Shore}, S.~N. and {de Mink}, S.~E.},
        title = "{Systematic survey of the effects of wind mass loss algorithms on the evolution of single massive stars}",
      journal = {\aap},
     keywords = {stars: evolution, stars: massive, stars: mass-loss, stars: winds, outflows, supernovae: general, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jul,
       volume = {603},
          eid = {A118},
        pages = {A118},
          doi = {10.1051/0004-6361/201730698},
archivePrefix = {arXiv},
       eprint = {1703.09705},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...603A.118R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Romagnolo2024,
       author = {{Romagnolo}, Amedeo and {Gormaz-Matamala}, Alex C. and {Belczynski}, Krzysztof},
        title = "{On the Maximum Black Hole Mass at Solar Metallicity}",
      journal = {\apjl},
     keywords = {Black holes, Stellar evolution, 162, 1599, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2024,
        month = apr,
       volume = {964},
       number = {2},
          eid = {L23},
        pages = {L23},
          doi = {10.3847/2041-8213/ad2fbe},
archivePrefix = {arXiv},
       eprint = {2311.18841},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024ApJ...964L..23R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


% -------------------------- S --------------------------
@BOOK{Schwarzschild1958,
       author = {{Schwarzschild}, Martin},
        title = "{Structure and evolution of the stars.}",
         year = 1958,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1958ses..book.....S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Spitzer1978,
       author = {{Spitzer}, Lyman and {Arny}, Thomas T.},
        title = "{Physical Processes in the Interstellar Medium}",
      journal = {American Journal of Physics},
     keywords = {98.40.Bs},
         year = 1978,
        month = nov,
       volume = {46},
       number = {11},
        pages = {1201-1201},
          doi = {10.1119/1.11466},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1978AmJPh..46.1201S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Stothers1999,
       author = {{Stothers}, Richard B.},
        title = "{Criterion for the dynamical stability of a non-adiabatic spherical self-gravitating body}",
      journal = {\mnras},
     keywords = {INSTABILITIES, STARS: OSCILLATIONS, STARS: VARIABLES: OTHER},
         year = 1999,
        month = apr,
       volume = {305},
       number = {2},
        pages = {365-372},
          doi = {10.1046/j.1365-8711.1999.02444.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999MNRAS.305..365S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Spera2017,
       author = {{Spera}, Mario and {Mapelli}, Michela},
        title = "{Very massive stars, pair-instability supernovae and intermediate-mass black holes with the sevn code}",
      journal = {\mnras},
     keywords = {black hole physics, gravitational waves, methods: numerical, stars: mass-loss, supernovae: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = oct,
       volume = {470},
       number = {4},
        pages = {4739-4749},
          doi = {10.1093/mnras/stx157610.48550/arXiv.1706.06109},
archivePrefix = {arXiv},
       eprint = {1706.06109},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.470.4739S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@MISC{Sander2019,
       author = {{Sander}, Andreas and {Hainich}, Rainer and {Hamann}, Wolf-Rainer and {Ignace}, Richard and {Oskinova}, Lida and {Shenar}, Tomer and {Todt}, Helge and {Vink}, Jorick},
        title = "{Anchoring mass-loss and metallicity for the WR population in M31 - A prototype study}",
 howpublished = {HST Proposal. Cycle 27, ID. \#15822},
         year = 2019,
        month = jun,
        pages = {15822},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019hst..prop15822S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schneider2018,
       author = {{Schneider}, F.~R.~N. and {Sana}, H. and {Evans}, C.~J. and {Bestenlehner}, J.~M. and {Castro}, N. and {Fossati}, L. and {Gr{\"a}fener}, G. and {Langer}, N. and {Ram{\'\i}rez-Agudelo}, O.~H. and {Sab{\'\i}n-Sanjuli{\'a}n}, C. and {Sim{\'o}n-D{\'\i}az}, S. and {Tramper}, F. and {Crowther}, P.~A. and {de Koter}, A. and {de Mink}, S.~E. and {Dufton}, P.~L. and {Garcia}, M. and {Gieles}, M. and {H{\'e}nault-Brunet}, V. and {Herrero}, A. and {Izzard}, R.~G. and {Kalari}, V. and {Lennon}, D.~J. and {Ma{\'\i}z Apell{\'a}niz}, J. and {Markova}, N. and {Najarro}, F. and {Podsiadlowski}, Ph. and {Puls}, J. and {Taylor}, W.~D. and {van Loon}, J. Th. and {Vink}, J.~S. and {Norman}, C.},
        title = "{An excess of massive stars in the local 30 Doradus starburst}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = jan,
       volume = {359},
       number = {6371},
        pages = {69-71},
          doi = {10.1126/science.aan0106},
archivePrefix = {arXiv},
       eprint = {1801.03107},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018Sci...359...69S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Samsing2022,
       author = {{Samsing}, J. and {Bartos}, I. and {D'Orazio}, D.~J. and {Haiman}, Z. and {Kocsis}, B. and {Leigh}, N.~W.~C. and {Liu}, B. and {Pessah}, M.~E. and {Tagawa}, H.},
        title = "{AGN as potential factories for eccentric black hole mergers}",
      journal = {\nat},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = mar,
       volume = {603},
       number = {7900},
        pages = {237-240},
          doi = {10.1038/s41586-021-04333-1},
archivePrefix = {arXiv},
       eprint = {2010.09765},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022Natur.603..237S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Shenar2023,
       author = {{Shenar}, T. and {Sana}, H. and {Crowther}, P.~A. and {Bostroem}, K.~A. and {Mahy}, L. and {Najarro}, F. and {Oskinova}, L. and {Sander}, A.~A.~C.},
        title = "{Constraints on the multiplicity of the most massive stars known: R136 a1, a2, a3, and c}",
      journal = {\aap},
     keywords = {stars: Wolf-Rayet, binaries: spectroscopic, stars: massive, Magellanic Clouds, Astrophysics - Solar and Stellar Astrophysics},
         year = 2023,
        month = nov,
       volume = {679},
          eid = {A36},
        pages = {A36},
          doi = {10.1051/0004-6361/202346930},
archivePrefix = {arXiv},
       eprint = {2309.13113},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A&A...679A..36S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Sibony2024,
       author = {{Sibony}, Yves and {Shepherd}, Kendall G. and {Yusof}, Norhasliza and {Hirschi}, Raphael and {Chambers}, Caitlan and {Tsiatsiou}, Sophie and {Nandal}, Devesh and {Sciarini}, Luca and {Moyano}, Facundo D. and {B{\'e}trisey}, J{\'e}r{\^o}me and {Buldgen}, Ga{\"e}l and {Georgy}, Cyril and {Ekstr{\"o}m}, Sylvia and {Eggenberger}, Patrick and {Meynet}, Georges},
        title = "{Grids of stellar models with rotation: VIII. Models from 1.7 to 500 M$_{{\ensuremath{\odot}}}$ at metallicity Z = 10$^{‑5}$}",
      journal = {\aap},
     keywords = {stars: evolution, stars: massive, stars: Population II, stars: rotation, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2024,
        month = oct,
       volume = {690},
          eid = {A91},
        pages = {A91},
          doi = {10.1051/0004-6361/202450180},
archivePrefix = {arXiv},
       eprint = {2407.06739},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024A&A...690A..91S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



% -------------------------- T --------------------------
@ARTICLE{Timmes1999,
       author = {{Timmes}, F.~X. and {Arnett}, Dave},
        title = "{The Accuracy, Consistency, and Speed of Five Equations of State for Stellar Hydrodynamics}",
      journal = {\apjs},
     keywords = {EQUATION OF STATE, HYDRODYNAMICS, METHODS: NUMERICAL, STARS: GENERAL, STARS: INTERIORS, Equation of State, Hydrodynamics, Methods: Numerical, Stars: General, Stars: Interiors},
         year = 1999,
        month = nov,
       volume = {125},
       number = {1},
        pages = {277-294},
          doi = {10.1086/313271},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJS..125..277T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Tsiatsiou2024,
       author = {{Tsiatsiou}, Sophie and {Sibony}, Yves and {Nandal}, Devesh and {Sciarini}, Luca and {Hirai}, Yutaka and {Ekstr{\"o}m}, Sylvia and {Farrell}, Eoin and {Murphy}, Laura and {Choplin}, Arthur and {Hirschi}, Raphael and {Chiappini}, Cristina and {Liu}, Boyuan and {Bromm}, Volker and {Groh}, Jose and {Meynet}, Georges},
        title = "{Rapidly rotating Population III stellar models as a source of primary nitrogen}",
      journal = {\aap},
     keywords = {stars: abundances, stars: massive, stars: Population III, stars: rotation, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2024,
        month = jul,
       volume = {687},
          eid = {A307},
        pages = {A307},
          doi = {10.1051/0004-6361/202449156},
archivePrefix = {arXiv},
       eprint = {2404.16512},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024A&A...687A.307T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Topping2015,
       author = {{Topping}, Michael W. and {Shull}, J. Michael},
        title = "{The Efficiency of Stellar Reionization: Effects of Rotation, Metallicity, and Initial Mass Function}",
      journal = {\apj},
     keywords = {dark ages, reionization, first stars, stars: atmospheres, stars: evolution, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = feb,
       volume = {800},
       number = {2},
          eid = {97},
        pages = {97},
          doi = {10.1088/0004-637X/800/2/97},
archivePrefix = {arXiv},
       eprint = {1501.01976},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...800...97T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



% -------------------------- V --------------------------
@INPROCEEDINGS{Vink2015,
       author = {{Vink}, J.~S.},
        title = "{The True origin of Wolf-Rayet stars}",
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
    booktitle = {Wolf-Rayet Stars},
         year = 2015,
       editor = {{Hamann}, Wolf-Rainer and {Sander}, Andreas and {Todt}, Helge},
        month = jan,
        pages = {133-138},
          doi = {10.48550/arXiv.1510.00227},
archivePrefix = {arXiv},
       eprint = {1510.00227},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015wrs..conf..133V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Vink2011,
       author = {{Vink}, Jorick S. and {Muijres}, L.~E. and {Anthonisse}, B. and {de Koter}, A. and {Gr{\"a}fener}, G. and {Langer}, N.},
        title = "{Wind modelling of very massive stars up to 300 solar masses}",
      journal = {\aap},
     keywords = {stars: massive, supergiants, stars: winds, outflows, stars: Wolf-Rayet, stars: mass-loss, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2011,
        month = jul,
       volume = {531},
          eid = {A132},
        pages = {A132},
          doi = {10.1051/0004-6361/201116614},
archivePrefix = {arXiv},
       eprint = {1105.0556},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...531A.132V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Vink2001,
       author = {{Vink}, Jorick S. and {de Koter}, A. and {Lamers}, H.~J.~G.~L.~M.},
        title = "{Mass-loss predictions for O and B stars as a function of metallicity}",
      journal = {\aap},
     keywords = {STARS: EARLY-TYPE, STARS: MASS-LOSS, STARS: SUPERGIANTS, STARS: WINDS, STARS: EVOLUTION, Astrophysics},
         year = 2001,
        month = apr,
       volume = {369},
        pages = {574-588},
          doi = {10.1051/0004-6361:20010127},
archivePrefix = {arXiv},
       eprint = {astro-ph/0101509},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...369..574V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Volpato2023,
       author = {{Volpato}, Guglielmo and {Marigo}, Paola and {Costa}, Guglielmo and {Bressan}, Alessandro and {Trabucchi}, Michele and {Girardi}, L{\'e}o},
        title = "{A Study of Primordial Very Massive Star Evolution}",
      journal = {\apj},
     keywords = {Stellar evolution, Stellar remnants, Stellar winds, Population III stars, 1599, 1627, 1636, 1285, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2023,
        month = feb,
       volume = {944},
       number = {1},
          eid = {40},
        pages = {40},
          doi = {10.3847/1538-4357/acac91},
archivePrefix = {arXiv},
       eprint = {2212.09629},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023ApJ...944...40V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Vink2024,
       author = {{Vink}, Jorick S. and {Sabhahit}, Gautham N. and {Higgins}, Erin R.},
        title = "{The maximum black hole mass at solar metallicity}",
      journal = {\aap},
     keywords = {stars: evolution, stars: massive, stars: mass-loss, supergiants, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2024,
        month = aug,
       volume = {688},
          eid = {L10},
        pages = {L10},
          doi = {10.1051/0004-6361/202450655},
archivePrefix = {arXiv},
       eprint = {2407.07204},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024A&A...688L..10V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



% -------------------------- W --------------------------
@ARTICLE{Weaver1993,
       author = {{Weaver}, Thomas A. and {Woosley}, S.~E.},
        title = "{Nucleosynthesis in massive stars and the $^{12}$C({\ensuremath{\alpha}}, {\ensuremath{\gamma}})$^{16}$O reaction rate}",
      journal = {\physrep},
     keywords = {Stellar Evolution: Nucleosynthesis, Stellar Interiors: Nuclear Reactions, Nucleosynthesis: Supernovae},
         year = 1993,
        month = may,
       volume = {227},
       number = {1-5},
        pages = {65-96},
          doi = {10.1016/0370-1573(93)90058-L},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993PhR...227...65W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Woosley2017,
       author = {{Woosley}, S.~E.},
        title = "{Pulsational Pair-instability Supernovae}",
      journal = {\apj},
     keywords = {stars: black holes, stars: evolution, gravitational waves, hydrodynamics, nuclear reactions, nucleosynthesis, abundances, supernovae: general, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = feb,
       volume = {836},
       number = {2},
          eid = {244},
        pages = {244},
          doi = {10.3847/1538-4357/836/2/244},
archivePrefix = {arXiv},
       eprint = {1608.08939},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...836..244W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{WoosleyHeger2002,
       author = {{Woosley}, S.~E. and {Heger}, A. and {Weaver}, T.~A.},
        title = "{The evolution and explosion of massive stars}",
      journal = {Reviews of Modern Physics},
     keywords = {26.30.+k, 97.60.Bw, 26.20.+f, 95.30.Cq, 97.10.Cv, 97.60.Jd, 95.30.Sf, Nucleosynthesis in novae supernovae and other explosive environments, Supernovae, Hydrostatic stellar nucleosynthesis, Elementary particle processes, Stellar structure interiors evolution nucleosynthesis ages, Neutron stars, Relativity and gravitation},
         year = 2002,
        month = nov,
       volume = {74},
       number = {4},
        pages = {1015-1071},
          doi = {10.1103/RevModPhys.74.1015},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002RvMP...74.1015W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Wu2016,
       author = {{Wu}, Shi-Wei and {Bik}, Arjan and {Bestenlehner}, Joachim M. and {Henning}, Thomas and {Pasquali}, Anna and {Brandner}, Wolfgang and {Stolte}, Andrea},
        title = "{The massive stellar population of W49: A spectroscopic survey}",
      journal = {\aap},
     keywords = {stars: formation, stars: massive, supergiants, infrared:, stars, techniques: spectroscopic, open clusters and associations:, individual: W49, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = may,
       volume = {589},
          eid = {A16},
        pages = {A16},
          doi = {10.1051/0004-6361/201527823},
archivePrefix = {arXiv},
       eprint = {1602.05190},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...589A..16W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Wise2014,
       author = {{Wise}, John H. and {Demchenko}, Vasiliy G. and {Halicek}, Martin T. and {Norman}, Michael L. and {Turk}, Matthew J. and {Abel}, Tom and {Smith}, Britton D.},
        title = "{The birth of a galaxy - III. Propelling reionization with the faintest galaxies}",
      journal = {\mnras},
     keywords = {radiative transfer, methods: numerical, galaxies: dwarf, galaxies: formation, galaxies: high-redshift, dark ages, reionization, first stars, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = aug,
       volume = {442},
       number = {3},
        pages = {2560-2579},
          doi = {10.1093/mnras/stu979},
archivePrefix = {arXiv},
       eprint = {1403.6123},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.442.2560W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Volpato2024,
       author = {{Volpato}, Guglielmo and {Marigo}, Paola and {Costa}, Guglielmo and {Bressan}, Alessandro and {Trabucchi}, Michele and {Girardi}, L{\'e}o and {Addari}, Francesco},
        title = "{A Study of Primordial Very Massive Star Evolution. II. Stellar Rotation and Gamma-Ray Burst Progenitors}",
      journal = {\apj},
     keywords = {Stellar evolution, Stellar remnants, Stellar rotation, Population III stars, Stellar winds, Gamma-ray bursts, 1599, 1627, 1629, 1285, 1636, 629, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2024,
        month = jan,
       volume = {961},
       number = {1},
          eid = {89},
        pages = {89},
          doi = {10.3847/1538-4357/ad1185},
archivePrefix = {arXiv},
       eprint = {2311.18429},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024ApJ...961...89V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Xing2023,
       author = {{Xing}, Qian-Fan and {Zhao}, Gang and {Liu}, Zheng-Wei and {Heger}, Alexander and {Han}, Zhan-Wen and {Aoki}, Wako and {Chen}, Yu-Qin and {Ishigaki}, Miho N. and {Li}, Hai-Ning and {Zhao}, Jing-Kun},
        title = "{A metal-poor star with abundances from a pair-instability supernova}",
      journal = {\nat},
         year = 2023,
        month = jun,
       volume = {618},
       number = {7966},
        pages = {712-715},
          doi = {10.1038/s41586-023-06028-1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023Natur.618..712X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Woosley2021,
       author = {{Woosley}, S.~E. and {Heger}, Alexander},
        title = "{The Pair-instability Mass Gap for Black Holes}",
      journal = {\apjl},
     keywords = {Stellar mass black holes, Core-collapse supernovae, Hypernovae, Gravitational wave astronomy, 1611, 304, 775, 675, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena, General Relativity and Quantum Cosmology, Nuclear Theory},
         year = 2021,
        month = may,
       volume = {912},
       number = {2},
          eid = {L31},
        pages = {L31},
          doi = {10.3847/2041-8213/abf2c4},
archivePrefix = {arXiv},
       eprint = {2103.07933},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...912L..31W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Farmer2020,
       author = {{Farmer}, R. and {Renzo}, M. and {de Mink}, S.~E. and {Fishbach}, M. and {Justham}, S.},
        title = "{Constraints from Gravitational-wave Detections of Binary Black Hole Mergers on the $^{12}$C({\ensuremath{\alpha}}, {\ensuremath{\gamma}})$^{16}$O Rate}",
      journal = {\apjl},
     keywords = {Stellar evolution, Supernovae, Core-collapse supernovae, Nuclear astrophysics, Stellar mass black holes, Astrophysical black holes, Massive stars, Late stellar evolution, 1599, 1668, 304, 1129, 1611, 98, 732, 911, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = oct,
       volume = {902},
       number = {2},
          eid = {L36},
        pages = {L36},
          doi = {10.3847/2041-8213/abbadd},
archivePrefix = {arXiv},
       eprint = {2006.06678},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...902L..36F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chieffi2004,
       author = {{Chieffi}, Alessandro and {Limongi}, Marco},
        title = "{Explosive Yields of Massive Stars from Z = 0 to Z = Z$_{solar}$}",
      journal = {\apj},
     keywords = {Nuclear Reactions, Nucleosynthesis, Abundances, Stars: Evolution, Stars: Supernovae: General, Astrophysics},
         year = 2004,
        month = jun,
       volume = {608},
       number = {1},
        pages = {405-410},
          doi = {10.1086/392523},
archivePrefix = {arXiv},
       eprint = {astro-ph/0402625},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...608..405C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zevin2020,
       author = {{Zevin}, Michael and {Spera}, Mario and {Berry}, Christopher P.~L. and {Kalogera}, Vicky},
        title = "{Exploring the Lower Mass Gap and Unequal Mass Regime in Compact Binary Evolution}",
      journal = {\apjl},
     keywords = {Gravitational waves, Gravitational wave sources, Neutron stars, Stellar mass black holes, Astrophysical black holes, Supernovae, Core-collapse supernovae, Stellar evolutionary models, 678, 677, 1108, 1611, 98, 1668, 304, 2046, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics, General Relativity and Quantum Cosmology},
         year = 2020,
        month = aug,
       volume = {899},
       number = {1},
          eid = {L1},
        pages = {L1},
          doi = {10.3847/2041-8213/aba74e},
archivePrefix = {arXiv},
       eprint = {2006.14573},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...899L...1Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Iorio2023,
       author = {{Iorio}, Giuliano and {Mapelli}, Michela and {Costa}, Guglielmo and {Spera}, Mario and {Escobar}, Gast{\'o}n J. and {Sgalletta}, Cecilia and {Trani}, Alessandro A. and {Korb}, Erika and {Santoliquido}, Filippo and {Dall'Amico}, Marco and {Gaspari}, Nicola and {Bressan}, Alessandro},
        title = "{Compact object mergers: exploring uncertainties from stellar and binary evolution with SEVN}",
      journal = {\mnras},
     keywords = {gravitational waves, methods: numerical, binaries: general, stars: black holes, stars: mass-loss, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2023,
        month = sep,
       volume = {524},
       number = {1},
        pages = {426-470},
          doi = {10.1093/mnras/stad1630},
archivePrefix = {arXiv},
       eprint = {2211.11774},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023MNRAS.524..426I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Farrell2020,
       author = {{Farrell}, Eoin J. and {Groh}, Jose H. and {Meynet}, Georges and {Eldridge}, J.~J.},
        title = "{The uncertain masses of progenitors of core-collapse supernovae and direct-collapse black holes}",
      journal = {\mnras},
     keywords = {stars: evolution, stars: massive, stars: supernovae, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = may,
       volume = {494},
       number = {1},
        pages = {L53-L58},
          doi = {10.1093/mnrasl/slaa035},
archivePrefix = {arXiv},
       eprint = {2001.08711},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.494L..53F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Clarkson2021,
       author = {{Clarkson}, O. and {Herwig}, F.},
        title = "{Convective H-He interactions in massive population III stellar evolution models}",
      journal = {\mnras},
     keywords = {nuclear reactions, nucleosynthesis, abundances, stars: evolution, stars: massive, stars: Population III, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = jan,
       volume = {500},
       number = {2},
        pages = {2685-2703},
          doi = {10.1093/mnras/staa3328},
archivePrefix = {arXiv},
       eprint = {2005.07748},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.500.2685C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vink2021,
       author = {{Vink}, Jorick S. and {Higgins}, Erin R. and {Sander}, Andreas A.~C. and {Sabhahit}, Gautham N.},
        title = "{Maximum black hole mass across cosmic time}",
      journal = {\mnras},
     keywords = {gravitational waves, stars: black holes, stars: evolution, stars: massive, stars: mass-loss, stars: winds, outflows, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = jun,
       volume = {504},
       number = {1},
        pages = {146-154},
          doi = {10.1093/mnras/stab842},
archivePrefix = {arXiv},
       eprint = {2010.11730},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.504..146V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Spera2019,
       author = {{Spera}, Mario and {Mapelli}, Michela and {Giacobbo}, Nicola and {Trani}, Alessandro A. and {Bressan}, Alessandro and {Costa}, Guglielmo},
        title = "{Merging black hole binaries with the SEVN code}",
      journal = {\mnras},
     keywords = {black hole physics, gravitational waves, methods: numerical, binaries: general, stars: mass-loss, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = may,
       volume = {485},
       number = {1},
        pages = {889-907},
          doi = {10.1093/mnras/stz359},
archivePrefix = {arXiv},
       eprint = {1809.04605},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.485..889S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Belczynski2010,
       author = {{Belczynski}, Krzysztof and {Bulik}, Tomasz and {Fryer}, Chris L. and {Ruiter}, Ashley and {Valsecchi}, Francesca and {Vink}, Jorick S. and {Hurley}, Jarrod R.},
        title = "{On the Maximum Mass of Stellar Black Holes}",
      journal = {\apj},
     keywords = {binaries: close, black hole physics, gravitational waves, stars: evolution, stars: neutron, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2010,
        month = may,
       volume = {714},
       number = {2},
        pages = {1217-1226},
          doi = {10.1088/0004-637X/714/2/1217},
archivePrefix = {arXiv},
       eprint = {0904.2784},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...714.1217B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Belczynski2016,
       author = {{Belczynski}, K. and {Heger}, A. and {Gladysz}, W. and {Ruiter}, A.~J. and {Woosley}, S. and {Wiktorowicz}, G. and {Chen}, H. -Y. and {Bulik}, T. and {O'Shaughnessy}, R. and {Holz}, D.~E. and {Fryer}, C.~L. and {Berti}, E.},
        title = "{The effect of pair-instability mass loss on black-hole mergers}",
      journal = {\aap},
     keywords = {stars: massive, black hole physics, gravitational waves, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = oct,
       volume = {594},
          eid = {A97},
        pages = {A97},
          doi = {10.1051/0004-6361/201628980},
archivePrefix = {arXiv},
       eprint = {1607.03116},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...594A..97B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Renzo2020,
       author = {{Renzo}, M. and {Cantiello}, M. and {Metzger}, B.~D. and {Jiang}, Y. -F.},
        title = "{The Stellar Merger Scenario for Black Holes in the Pair-instability Gap}",
      journal = {\apjl},
     keywords = {Massive stars, Black holes, Luminous blue variable stars, Stellar mergers, 732, 162, 944, 2157, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = dec,
       volume = {904},
       number = {2},
          eid = {L13},
        pages = {L13},
          doi = {10.3847/2041-8213/abc6a6},
archivePrefix = {arXiv},
       eprint = {2010.00705},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...904L..13R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fryer2012,
       author = {{Fryer}, Chris L. and {Belczynski}, Krzysztof and {Wiktorowicz}, Grzegorz and {Dominik}, Michal and {Kalogera}, Vicky and {Holz}, Daniel E.},
        title = "{Compact Remnant Mass Function: Dependence on the Explosion Mechanism and Metallicity}",
      journal = {\apj},
     keywords = {black hole physics, stars: neutron, supernovae: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = apr,
       volume = {749},
       number = {1},
          eid = {91},
        pages = {91},
          doi = {10.1088/0004-637X/749/1/91},
archivePrefix = {arXiv},
       eprint = {1110.1726},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...749...91F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Woosley2002,
       author = {{Woosley}, S.~E. and {Heger}, A. and {Weaver}, T.~A.},
        title = "{The evolution and explosion of massive stars}",
      journal = {Reviews of Modern Physics},
     keywords = {26.30.+k, 97.60.Bw, 26.20.+f, 95.30.Cq, 97.10.Cv, 97.60.Jd, 95.30.Sf, Nucleosynthesis in novae supernovae and other explosive environments, Supernovae, Hydrostatic stellar nucleosynthesis, Elementary particle processes, Stellar structure interiors evolution nucleosynthesis ages, Neutron stars, Relativity and gravitation},
         year = 2002,
        month = nov,
       volume = {74},
       number = {4},
        pages = {1015-1071},
          doi = {10.1103/RevModPhys.74.1015},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002RvMP...74.1015W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fryer2001,
       author = {{Fryer}, Chris L. and {Kalogera}, Vassiliki},
        title = "{Theoretical Black Hole Mass Distributions}",
      journal = {\apj},
     keywords = {Stars: Binaries: General, Black Hole Physics, Stars: Evolution, Stars: Mass Loss, Stars: Neutron, Stars: Supernovae: General, Astrophysics},
         year = 2001,
        month = jun,
       volume = {554},
       number = {1},
        pages = {548-560},
          doi = {10.1086/321359},
archivePrefix = {arXiv},
       eprint = {astro-ph/9911312},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...554..548F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Nomoto2013,
       author = {{Nomoto}, Ken'ichi and {Kobayashi}, Chiaki and {Tominaga}, Nozomu},
        title = "{Nucleosynthesis in Stars and the Chemical Enrichment of Galaxies}",
      journal = {\araa},
         year = 2013,
        month = aug,
       volume = {51},
       number = {1},
        pages = {457-509},
          doi = {10.1146/annurev-astro-082812-140956},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ARA&A..51..457N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Goswami2022,
       author = {{Goswami}, S. and {Silva}, L. and {Bressan}, A. and {Grisoni}, V. and {Costa}, G. and {Marigo}, P. and {Granato}, G.~L. and {Lapi}, A. and {Spera}, M.},
        title = "{Impact of very massive stars on the chemical evolution of extremely metal-poor galaxies}",
      journal = {\aap},
     keywords = {galaxies: abundances, galaxies: starburst, galaxies: formation, stars: massive, galaxies: structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = jul,
       volume = {663},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/202142031},
archivePrefix = {arXiv},
       eprint = {2205.03402},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A&A...663A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schaerer2024,
       author = {{Schaerer}, D. and {Guibert}, J. and {Marques-Chaves}, R. and {Martins}, F.},
        title = "{Observable and ionizing properties of star-forming galaxies with very massive stars and different IMFs}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2024,
        month = jul,
          eid = {arXiv:2407.12122},
        pages = {arXiv:2407.12122},
          doi = {10.48550/arXiv.2407.12122},
archivePrefix = {arXiv},
       eprint = {2407.12122},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024arXiv240712122S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Martins2023,
       author = {{Martins}, F. and {Schaerer}, D. and {Marques-Chaves}, R. and {Upadhyaya}, A.},
        title = "{Inferring the presence of very massive stars in local star-forming regions}",
      journal = {\aap},
     keywords = {stars: massive, galaxies: starburst, galaxies: stellar content, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = oct,
       volume = {678},
          eid = {A159},
        pages = {A159},
          doi = {10.1051/0004-6361/202346732},
archivePrefix = {arXiv},
       eprint = {2308.14489},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A&A...678A.159M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chon2024,
       author = {{Chon}, Sunmyon and {Hosokawa}, Takashi and {Omukai}, Kazuyuki and {Schneider}, Raffaella},
        title = "{Impact of radiative feedback on the initial mass function of metal-poor stars}",
      journal = {\mnras},
     keywords = {stars: formation, stars: Population II, stars: Population III, galaxies: evolution, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2024,
        month = may,
       volume = {530},
       number = {3},
        pages = {2453-2474},
          doi = {10.1093/mnras/stae1027},
archivePrefix = {arXiv},
       eprint = {2312.13339},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024MNRAS.530.2453C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lecroq2024,
       author = {{Lecroq}, Marie and {Charlot}, St{\'e}phane and {Bressan}, Alessandro and {Bruzual}, Gustavo and {Costa}, Guglielmo and {Iorio}, Giuliano and {Spera}, Mario and {Mapelli}, Michela and {Chen}, Yang and {Chevallard}, Jacopo and {Dall'Amico}, Marco},
        title = "{Nebular emission from young stellar populations including binary stars}",
      journal = {\mnras},
     keywords = {binaries: general, galaxies: general, galaxies: high-redshift, galaxies: ISM, X-rays: binaries, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2024,
        month = jan,
       volume = {527},
       number = {3},
        pages = {9480-9504},
          doi = {10.1093/mnras/stad3838},
archivePrefix = {arXiv},
       eprint = {2312.08432},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024MNRAS.527.9480L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stanway2018,
       author = {{Stanway}, E.~R. and {Eldridge}, J.~J.},
        title = "{Re-evaluating old stellar populations}",
      journal = {\mnras},
     keywords = {methods: numerical, binaries: general, galaxies: stellar content, globular clusters: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = sep,
       volume = {479},
       number = {1},
        pages = {75-93},
          doi = {10.1093/mnras/sty1353},
archivePrefix = {arXiv},
       eprint = {1805.08784},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.479...75S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Humphreys1979,
       author = {{Humphreys}, R.~M. and {Davidson}, K.},
        title = "{Studies of luminous stars in nearby galaxies. III. Comments on the evolution of the most massive stars in the Milky Way and the Large Magellanic Cloud.}",
      journal = {\apj},
     keywords = {Magellanic Clouds, Stellar Evolution, Supergiant Stars, Supermassive Stars, Hertzsprung-Russell Diagram, Stellar Luminosity, Stellar Mass Ejection, Stellar Spectra, Astrophysics, Galaxy:HR Diagrams, Galaxy:Supergiants, HR Diagrams:Magellanic Clouds, HR Diagrams:Supergiants, Magellanic Clouds:Supergiants},
         year = 1979,
        month = sep,
       volume = {232},
        pages = {409-420},
          doi = {10.1086/157301},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1979ApJ...232..409H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Salpeter1955,
       author = {{Salpeter}, Edwin E.},
        title = "{The Luminosity Function and Stellar Evolution.}",
      journal = {\apj},
         year = 1955,
        month = jan,
       volume = {121},
        pages = {161},
          doi = {10.1086/145971},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1955ApJ...121..161S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sabhahit2022,
       author = {{Sabhahit}, Gautham N. and {Vink}, Jorick S. and {Higgins}, Erin R. and {Sander}, Andreas A.~C.},
        title = "{Mass-loss implementation and temperature evolution of very massive stars}",
      journal = {\mnras},
     keywords = {stars: evolution, stars: massive, stars: mass-loss, stars: winds, outflows, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2022,
        month = aug,
       volume = {514},
       number = {3},
        pages = {3736-3753},
          doi = {10.1093/mnras/stac1410},
archivePrefix = {arXiv},
       eprint = {2205.09125},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.514.3736S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yusof2022,
       author = {{Yusof}, Norhasliza and {Hirschi}, Raphael and {Eggenberger}, Patrick and {Ekstr{\"o}m}, Sylvia and {Georgy}, Cyril and {Sibony}, Yves and {Crowther}, Paul A. and {Meynet}, Georges and {Kassim}, Hasan Abu and {Harun}, Wan Aishah Wan and {Maeder}, Andr{\'e} and {Groh}, Jose H. and {Farrell}, Eoin and {Murphy}, Laura},
        title = "{Grids of stellar models with rotation VII: models from 0.8 to 300 M$_{{\ensuremath{\odot}}}$ at supersolar metallicity (Z = 0.020)}",
      journal = {\mnras},
     keywords = {stars: evolution, stars: massive, stars: rotation, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = apr,
       volume = {511},
       number = {2},
        pages = {2814-2828},
          doi = {10.1093/mnras/stac230},
archivePrefix = {arXiv},
       eprint = {2201.08645},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.511.2814Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yusof2013,
       author = {{Yusof}, Norhasliza and {Hirschi}, Raphael and {Meynet}, Georges and {Crowther}, Paul A. and {Ekstr{\"o}m}, Sylvia and {Frischknecht}, Urs and {Georgy}, Cyril and {Abu Kassim}, Hasan and {Schnurr}, Olivier},
        title = "{Evolution and fate of very massive stars}",
      journal = {\mnras},
     keywords = {stars: evolution, stars: massive, stars: mass-loss, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = aug,
       volume = {433},
       number = {2},
        pages = {1114-1132},
          doi = {10.1093/mnras/stt794},
archivePrefix = {arXiv},
       eprint = {1305.2099},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.433.1114Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Martinet2023,
       author = {{Martinet}, S{\'e}bastien and {Meynet}, Georges and {Ekstr{\"o}m}, Sylvia and {Georgy}, Cyril and {Hirschi}, Raphael},
        title = "{Very massive star models. I. Impact of rotation and metallicity and comparisons with observations}",
      journal = {\aap},
     keywords = {stars: evolution, stars: massive, stars: rotation, stars: Wolf-Rayet, stars: mass-loss, stars: Population III, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = nov,
       volume = {679},
          eid = {A137},
        pages = {A137},
          doi = {10.1051/0004-6361/202347514},
archivePrefix = {arXiv},
       eprint = {2309.00062},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A&A...679A.137M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Crowther2016,
       author = {{Crowther}, Paul A. and {Caballero-Nieves}, S.~M. and {Bostroem}, K.~A. and {Ma{\'\i}z Apell{\'a}niz}, J. and {Schneider}, F.~R.~N. and {Walborn}, N.~R. and {Angus}, C.~R. and {Brott}, I. and {Bonanos}, A. and {de Koter}, A. and {de Mink}, S.~E. and {Evans}, C.~J. and {Gr{\"a}fener}, G. and {Herrero}, A. and {Howarth}, I.~D. and {Langer}, N. and {Lennon}, D.~J. and {Puls}, J. and {Sana}, H. and {Vink}, J.~S.},
        title = "{The R136 star cluster dissected with Hubble Space Telescope/STIS. I. Far-ultraviolet spectroscopic census and the origin of He II {\ensuremath{\lambda}}1640 in young star clusters}",
      journal = {\mnras},
     keywords = {stars: early-type, stars: massive, stars: winds, outflows, Magellanic Clouds, galaxies: star clusters: individual: R136a, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = may,
       volume = {458},
       number = {1},
        pages = {624-659},
          doi = {10.1093/mnras/stw273},
archivePrefix = {arXiv},
       eprint = {1603.04994},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.458..624C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Tang2014,
       author = {{Tang}, Jing and {Bressan}, Alessandro and {Rosenfield}, Philip and {Slemer}, Alessandra and {Marigo}, Paola and {Girardi}, L{\'e}o and {Bianchi}, Luciana},
        title = "{New PARSEC evolutionary tracks of massive stars at low metallicity: testing canonical stellar evolution in nearby star-forming dwarf galaxies}",
      journal = {\mnras},
     keywords = {stars: evolution, Hertzsprung-Russell and colour-magnitude diagrams, stars: interiors, stars: massive, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = dec,
       volume = {445},
       number = {4},
        pages = {4287-4305},
          doi = {10.1093/mnras/stu2029},
archivePrefix = {arXiv},
       eprint = {1410.1745},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.445.4287T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gerosa2021,
       author = {{Gerosa}, Davide and {Fishbach}, Maya},
        title = "{Hierarchical mergers of stellar-mass black holes and their gravitational-wave signatures}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics, General Relativity and Quantum Cosmology},
         year = 2021,
        month = jul,
       volume = {5},
        pages = {749-760},
          doi = {10.1038/s41550-021-01398-w},
archivePrefix = {arXiv},
       eprint = {2105.03439},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021NatAs...5..749G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Belczynski2020,
       author = {{Belczynski}, Krzysztof},
        title = "{The Most Ordinary Formation of the Most Unusual Double Black Hole Merger}",
      journal = {\apjl},
     keywords = {Black hole physics, Stellar evolution, Stellar remnants, 159, 1599, 1627, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = dec,
       volume = {905},
       number = {2},
          eid = {L15},
        pages = {L15},
          doi = {10.3847/2041-8213/abcbf1},
archivePrefix = {arXiv},
       eprint = {2009.13526},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...905L..15B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Spera2022,
       author = {{Spera}, Mario and {Trani}, Alessandro Alberto and {Mencagli}, Mattia},
        title = "{Compact Binary Coalescences: Astrophysical Processes and Lessons Learned}",
      journal = {Galaxies},
     keywords = {gravitational-wave astrophysics, stars, black holes, stellar evolution, binary stars, stellar dynamics, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = jun,
       volume = {10},
       number = {4},
          eid = {76},
        pages = {76},
          doi = {10.3390/galaxies10040076},
archivePrefix = {arXiv},
       eprint = {2206.15392},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022Galax..10...76S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Farrell2021,
       author = {{Farrell}, Eoin and {Groh}, Jose H. and {Hirschi}, Raphael and {Murphy}, Laura and {Kaiser}, Etienne and {Ekstr{\"o}m}, Sylvia and {Georgy}, Cyril and {Meynet}, Georges},
        title = "{Is GW190521 the merger of black holes from the first stellar generations?}",
      journal = {\mnras},
     keywords = {stars: evolution, stars: massive, stars: mass-loss, stars: black holes, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = mar,
       volume = {502},
       number = {1},
        pages = {L40-L44},
          doi = {10.1093/mnrasl/slaa196},
archivePrefix = {arXiv},
       eprint = {2009.06585},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.502L..40F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bavera2023,
       author = {{Bavera}, Simone S. and {Fragos}, Tassos and {Zapartas}, Emmanouil and {Andrews}, Jeff J. and {Kalogera}, Vicky and {Berry}, Christopher P.~L. and {Kruckow}, Matthias and {Dotter}, Aaron and {Kovlakas}, Konstantinos and {Misra}, Devina and {Rocha}, Kyle A. and {Srivastava}, Philipp M. and {Sun}, Meng and {Xing}, Zepei},
        title = "{The formation of merging black holes with masses beyond 30 M$_{{\ensuremath{\odot}}}$ at solar metallicity}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics, General Relativity and Quantum Cosmology},
         year = 2023,
        month = sep,
       volume = {7},
        pages = {1090-1097},
          doi = {10.1038/s41550-023-02018-5},
archivePrefix = {arXiv},
       eprint = {2212.10924},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023NatAs...7.1090B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pina2024,
       author = {{Mar{\'\i}n Pina}, Daniel and {Rastello}, Sara and {Gieles}, Mark and {Kremer}, Kyle and {Fitzgerald}, Laura and {Rando Forastier}, Bruno},
        title = "{Dynamical formation of Gaia BH3 in the progenitor globular cluster of the ED-2 stream}",
      journal = {\aap},
     keywords = {stars: black holes, stars: Population II, globular clusters: general, Galaxy: halo, Galaxy: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2024,
        month = aug,
       volume = {688},
          eid = {L2},
        pages = {L2},
          doi = {10.1051/0004-6361/202450460},
archivePrefix = {arXiv},
       eprint = {2404.13036},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024A&A...688L...2M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bressan1993,
       author = {{Bressan}, A. and {Fagotto}, F. and {Bertelli}, G. and {Chiosi}, C.},
        title = "{Evolutionary Sequences of Stellar Models with New Radiative Opacities. II. Z = 0.02}",
      journal = {\aaps},
     keywords = {Stellar Composition, Stellar Evolution, Stellar Interiors, Stellar Mass, Stellar Models, Hertzsprung-Russell Diagram, Mixing, Opacity, Reaction Kinetics, Astrophysics},
         year = 1993,
        month = sep,
       volume = {100},
        pages = {647},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993A&AS..100..647B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Riess2019,
       author = {{Riess}, Adam G. and {Casertano}, Stefano and {Yuan}, Wenlong and {Macri}, Lucas M. and {Scolnic}, Dan},
        title = "{Large Magellanic Cloud Cepheid Standards Provide a 1\% Foundation for the Determination of the Hubble Constant and Stronger Evidence for Physics beyond {\ensuremath{\Lambda}}CDM}",
      journal = {\apj},
     keywords = {cosmological parameters, distance scale, stars: variables: Cepheids, supernovae: general, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = may,
       volume = {876},
       number = {1},
          eid = {85},
        pages = {85},
          doi = {10.3847/1538-4357/ab1422},
archivePrefix = {arXiv},
       eprint = {1903.07603},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...876...85R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Valcin2020,
       author = {{Valcin}, David and {Bernal}, Jos{\'e} Luis and {Jimenez}, Raul and {Verde}, Licia and {Wandelt}, Benjamin D.},
        title = "{Inferring the age of the universe with globular clusters}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = dec,
       volume = {2020},
       number = {12},
          eid = {002},
        pages = {002},
          doi = {10.1088/1475-7516/2020/12/002},
archivePrefix = {arXiv},
       eprint = {2007.06594},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020JCAP...12..002V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bruzual2003,
       author = {{Bruzual}, G. and {Charlot}, S.},
        title = "{Stellar population synthesis at the resolution of 2003}",
      journal = {\mnras},
     keywords = {stars: evolution, galaxies: evolution, galaxies: formation, galaxies: stellar content, Astrophysics},
         year = 2003,
        month = oct,
       volume = {344},
       number = {4},
        pages = {1000-1028},
          doi = {10.1046/j.1365-8711.2003.06897.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0309134},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003MNRAS.344.1000B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zevin2021,
       author = {{Zevin}, Michael and {Bavera}, Simone S. and {Berry}, Christopher P.~L. and {Kalogera}, Vicky and {Fragos}, Tassos and {Marchant}, Pablo and {Rodriguez}, Carl L. and {Antonini}, Fabio and {Holz}, Daniel E. and {Pankow}, Chris},
        title = "{One Channel to Rule Them All? Constraining the Origins of Binary Black Holes Using Multiple Formation Pathways}",
      journal = {\apj},
     keywords = {Gravitational wave sources, Gravitational wave astronomy, Stellar mass black holes, LIGO, Stellar evolution, Compact objects, Bayesian statistics, 677, 675, 1611, 920, 1599, 288, 1900, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics, General Relativity and Quantum Cosmology},
         year = 2021,
        month = apr,
       volume = {910},
       number = {2},
          eid = {152},
        pages = {152},
          doi = {10.3847/1538-4357/abe40e},
archivePrefix = {arXiv},
       eprint = {2011.10057},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...910..152Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brott2011,
       author = {{Brott}, I. and {de Mink}, S.~E. and {Cantiello}, M. and {Langer}, N. and {de Koter}, A. and {Evans}, C.~J. and {Hunter}, I. and {Trundle}, C. and {Vink}, J.~S.},
        title = "{Rotating massive main-sequence stars. I. Grids of evolutionary models and isochrones}",
      journal = {\aap},
     keywords = {stars: abundances, stars: evolution, stars: early-type, stars: rotation, stars: massive, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = jun,
       volume = {530},
          eid = {A115},
        pages = {A115},
          doi = {10.1051/0004-6361/201016113},
archivePrefix = {arXiv},
       eprint = {1102.0530},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...530A.115B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Spada2017,
       author = {{Spada}, F. and {Demarque}, P. and {Kim}, Y. -C. and {Boyajian}, T.~S. and {Brewer}, J.~M.},
        title = "{The Yale-Potsdam Stellar Isochrones}",
      journal = {\apj},
     keywords = {Hertzsprung{\textendash}Russell and C{\textendash}M diagrams, planetary systems, stars: evolution, stars: fundamental parameters, stars: interiors, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = apr,
       volume = {838},
       number = {2},
          eid = {161},
        pages = {161},
          doi = {10.3847/1538-4357/aa661d},
archivePrefix = {arXiv},
       eprint = {1703.03975},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...838..161S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Szecsi2022,
       author = {{Sz{\'e}csi}, Dorottya and {Agrawal}, Poojan and {W{\"u}nsch}, Richard and {Langer}, Norbert},
        title = "{Bonn Optimized Stellar Tracks (BoOST). Simulated populations of massive and very massive stars for astrophysical applications}",
      journal = {\aap},
     keywords = {stars: massive, stars: evolution, stars: formation, gravitational waves, stars: black holes, methods: numerical, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2022,
        month = feb,
       volume = {658},
          eid = {A125},
        pages = {A125},
          doi = {10.1051/0004-6361/202141536},
archivePrefix = {arXiv},
       eprint = {2004.08203},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A&A...658A.125S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hidalgo2018,
       author = {{Hidalgo}, Sebastian L. and {Pietrinferni}, Adriano and {Cassisi}, Santi and {Salaris}, Maurizio and {Mucciarelli}, Alessio and {Savino}, Alessandro and {Aparicio}, Antonio and {Silva Aguirre}, Victor and {Verma}, Kuldeep},
        title = "{The Updated BaSTI Stellar Evolution Models and Isochrones. I. Solar-scaled Calculations}",
      journal = {\apj},
     keywords = {galaxies: stellar content, Galaxy: disk, open clusters and associations: general, stars: evolution, stars: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = apr,
       volume = {856},
       number = {2},
          eid = {125},
        pages = {125},
          doi = {10.3847/1538-4357/aab158},
archivePrefix = {arXiv},
       eprint = {1802.07319},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...856..125H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Amard2019,
       author = {{Amard}, L. and {Palacios}, A. and {Charbonnel}, C. and {Gallet}, F. and {Georgy}, C. and {Lagarde}, N. and {Siess}, L.},
        title = "{First grids of low-mass stellar models and isochrones with self-consistent treatment of rotation. From 0.2 to 1.5 M$_{{\ensuremath{\odot}}}$ at seven metallicities from PMS to TAMS}",
      journal = {\aap},
     keywords = {stars: evolution, stars: rotation, stars: low-mass, stars: pre-main sequence, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = nov,
       volume = {631},
          eid = {A77},
        pages = {A77},
          doi = {10.1051/0004-6361/201935160},
archivePrefix = {arXiv},
       eprint = {1905.08516},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...631A..77A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rosdahl2018,
       author = {{Rosdahl}, Joakim and {Katz}, Harley and {Blaizot}, J{\'e}r{\'e}my and {Kimm}, Taysun and {Michel-Dansac}, L{\'e}o and {Garel}, Thibault and {Haehnelt}, Martin and {Ocvirk}, Pierre and {Teyssier}, Romain},
        title = "{The SPHINX cosmological simulations of the first billion years: the impact of binary stars on reionization}",
      journal = {\mnras},
     keywords = {methods: numerical, galaxies: high-redshift, dark ages, reionization, first stars, early Universe, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = sep,
       volume = {479},
       number = {1},
        pages = {994-1016},
          doi = {10.1093/mnras/sty1655},
archivePrefix = {arXiv},
       eprint = {1801.07259},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.479..994R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tayar2022,
       author = {{Tayar}, Jamie and {Claytor}, Zachary R. and {Huber}, Daniel and {van Saders}, Jennifer},
        title = "{A Guide to Realistic Uncertainties on the Fundamental Properties of Solar-type Exoplanet Host Stars}",
      journal = {\apj},
     keywords = {Exoplanets, Stellar ages, Stellar properties, Stellar luminosities, Stellar effective temperatures, Stellar masses, 498, 1581, 1624, 1609, 1597, 1614, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = mar,
       volume = {927},
       number = {1},
          eid = {31},
        pages = {31},
          doi = {10.3847/1538-4357/ac4bbc},
archivePrefix = {arXiv},
       eprint = {2012.07957},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJ...927...31T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Frebel2019,
       author = {{Frebel}, Anna and {Ji}, Alexander P. and {Ezzeddine}, Rana and {Hansen}, Terese T. and {Chiti}, Anirudh and {Thompson}, Ian B. and {Merle}, Thibault},
        title = "{Chemical Abundance Signature of J0023+0307: A Second-generation Main-sequence Star with [Fe/H] < -6}",
      journal = {\apj},
     keywords = {Galaxy: halo, nuclear reactions, nucleosynthesis, abundances, stars: abundances, stars: individual: J0023+0307, stars: Population II, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = feb,
       volume = {871},
       number = {2},
          eid = {146},
        pages = {146},
          doi = {10.3847/1538-4357/aae848},
archivePrefix = {arXiv},
       eprint = {1810.01228},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...871..146F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DalTio2021,
       author = {{Dal Tio}, Piero and {Mazzi}, Alessandro and {Girardi}, L{\'e}o and {Barbieri}, Mauro and {Zaggia}, Simone and {Bressan}, Alessandro and {Chen}, Yang and {Costa}, Guglielmo and {Marigo}, Paola},
        title = "{Dissecting the Gaia HR diagram within 200 pc}",
      journal = {\mnras},
     keywords = {binaries: general, Hertzsprung-Russell and colour-magnitude diagrams, solar neighbourhood, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = oct,
       volume = {506},
       number = {4},
        pages = {5681-5697},
          doi = {10.1093/mnras/stab1964},
archivePrefix = {arXiv},
       eprint = {2107.01844},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.506.5681D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DalTio2022,
       author = {{Dal Tio}, Piero and {Pastorelli}, Giada and {Mazzi}, Alessandro and {Trabucchi}, Michele and {Costa}, Guglielmo and {Jacques}, Alice and {Pieres}, Adriano and {Girardi}, L{\'e}o and {Chen}, Yang and {Olsen}, Knut A.~G. and {Juric}, Mario and {Ivezi{\'c}}, {\v{Z}}eljko and {Yoachim}, Peter and {Clarkson}, William I. and {Marigo}, Paola and {Rodrigues}, Thaise S. and {Zaggia}, Simone and {Barbieri}, Mauro and {Momany}, Yazan and {Bressan}, Alessandro and {Nikutta}, Robert and {da Costa}, Luiz Nicolaci},
        title = "{Simulating the Legacy Survey of Space and Time Stellar Content with TRILEGAL}",
      journal = {\apjs},
     keywords = {Large Magellanic Cloud, Small Magellanic Cloud, Local Group, Galactic bulge, Milky Way Galaxy, 903, 1468, 929, 2041, 1054, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = sep,
       volume = {262},
       number = {1},
          eid = {22},
        pages = {22},
          doi = {10.3847/1538-4365/ac7be6},
archivePrefix = {arXiv},
       eprint = {2208.00829},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJS..262...22D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mazzi2024,
       author = {{Mazzi}, Alessandro and {Girardi}, L{\'e}o and {Trabucchi}, Michele and {Dalcanton}, Julianne J. and {Luger}, Rodrigo and {Marigo}, Paola and {Miglio}, Andrea and {Costa}, Guglielmo and {Chen}, Yang and {Pastorelli}, Giada and {Fouesneau}, Morgan and {Zaggia}, Simone and {Bressan}, Alessandro and {Dal Tio}, Piero},
        title = "{Dissecting the Gaia HR diagram - II. The vertical structure of the star formation history across the solar cylinder}",
      journal = {\mnras},
     keywords = {Hertzsprung-Russell and colour-magnitude diagrams, solar neighbourhood, Astrophysics - Astrophysics of Galaxies},
         year = 2024,
        month = jan,
       volume = {527},
       number = {1},
        pages = {583-602},
          doi = {10.1093/mnras/stad2952},
archivePrefix = {arXiv},
       eprint = {2309.13453},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024MNRAS.527..583M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kobayashi2020,
       author = {{Kobayashi}, Chiaki and {Karakas}, Amanda I. and {Lugaro}, Maria},
        title = "{The Origin of Elements from Carbon to Uranium}",
      journal = {\apj},
     keywords = {Galaxy abundances, Stellar abundances, Chemical abundances, Stellar physics, Asymptotic giant branch stars, Core-collapse supernovae, Type Ia supernovae, Nucleosynthesis, Milky Way Galaxy, Galaxy chemical evolution, Galaxy evolution, Isotopic abundances, 574, 1577, 224, 1621, 2100, 304, 1728, 1131, 1054, 580, 594, 867, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = sep,
       volume = {900},
       number = {2},
          eid = {179},
        pages = {179},
          doi = {10.3847/1538-4357/abae65},
archivePrefix = {arXiv},
       eprint = {2008.04660},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...900..179K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kroupa2001,
       author = {{Kroupa}, Pavel},
        title = "{On the variation of the initial mass function}",
      journal = {\mnras},
     keywords = {BINARIES: GENERAL, STARS: FORMATION, STARS: KINEMATICS, STARS: LUMINOSITY FUNCTION, MASS FUNCTION, GLOBULAR CLUSTERS: GENERAL, OPEN CLUSTERS AND ASSOCIATIONS: GENERAL, Astrophysics},
         year = 2001,
        month = apr,
       volume = {322},
       number = {2},
        pages = {231-246},
          doi = {10.1046/j.1365-8711.2001.04022.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0009005},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001MNRAS.322..231K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chabrier2003,
       author = {{Chabrier}, Gilles},
        title = "{Galactic Stellar and Substellar Initial Mass Function}",
      journal = {\pasp},
     keywords = {Galaxies: Luminosity Function, Mass Function, Invited Reviews, Astrophysics},
         year = 2003,
        month = jul,
       volume = {115},
       number = {809},
        pages = {763-795},
          doi = {10.1086/376392},
archivePrefix = {arXiv},
       eprint = {astro-ph/0304382},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003PASP..115..763C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Gabrielli2024,
       author = {{Gabrielli}, Francesco and {Lapi}, Andrea and {Boco}, Lumen and {Ugolini}, Cristiano and {Costa}, Guglielmo and {Sgalletta}, Cecilia and {Shepherd}, Kendall and {Di Carlo}, Ugo N. and {Bressan}, Alessandro and {Limongi}, Marco and {Spera}, Mario},
        title = "{The cosmic rate of pair-instability supernovae}",
      journal = {\mnras},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2024,
        month = oct,
       volume = {534},
       number = {1},
        pages = {151-172},
          doi = {10.1093/mnras/stae2048},
archivePrefix = {arXiv},
       eprint = {2408.16823},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024MNRAS.534..151G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Vink2022,
       author = {{Vink}, Jorick S.},
        title = "{Theory and Diagnostics of Hot Star Mass Loss}",
      journal = {\araa},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2022,
        month = aug,
       volume = {60},
        pages = {203-246},
          doi = {10.1146/annurev-astro-052920-094949},
archivePrefix = {arXiv},
       eprint = {2109.08164},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ARA&A..60..203V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Janka2016,
       author = {{Janka}, Hans-Thomas and {Melson}, Tobias and {Summa}, Alexander},
        title = "{Physics of Core-Collapse Supernovae in Three Dimensions: A Sneak Preview}",
      journal = {Annual Review of Nuclear and Particle Science},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, High Energy Physics - Phenomenology, Nuclear Theory},
         year = 2016,
        month = oct,
       volume = {66},
       number = {1},
        pages = {341-375},
          doi = {10.1146/annurev-nucl-102115-044747},
archivePrefix = {arXiv},
       eprint = {1602.05576},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ARNPS..66..341J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Patton2020,
       author = {{Patton}, Rachel A. and {Sukhbold}, Tuguldur},
        title = "{Towards a realistic explosion landscape for binary population synthesis}",
      journal = {\mnras},
     keywords = {stars: evolution, stars: massive, supernovae: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = dec,
       volume = {499},
       number = {2},
        pages = {2803-2816},
          doi = {10.1093/mnras/staa3029},
archivePrefix = {arXiv},
       eprint = {2005.03055},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.499.2803P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Mezzacappa2023,
       author = {{Mezzacappa}, Anthony},
        title = "{Toward Realistic Models of Core Collapse Supernovae: A Brief Review}",
     keywords = {supernovae: general, neutrinos, hydrodynamics, relativity, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
    booktitle = {The Predictive Power of Computational Astrophysics as a Discover Tool},
         year = 2023,
       editor = {{Bisikalo}, Dmitry and {Wiebe}, Dmitri and {Boily}, Christian},
       series = {IAU Symposium},
       volume = {362},
        month = jan,
        pages = {215-227},
          doi = {10.1017/S1743921322001831},
archivePrefix = {arXiv},
       eprint = {2205.13438},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023IAUS..362..215M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Martins2013,
       author = {{Martins}, F. and {Palacios}, A.},
        title = "{A comparison of evolutionary tracks for single Galactic massive stars}",
      journal = {\aap},
     keywords = {stars: massive, stars: evolution, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = dec,
       volume = {560},
          eid = {A16},
        pages = {A16},
          doi = {10.1051/0004-6361/201322480},
archivePrefix = {arXiv},
       eprint = {1310.7218},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...560A..16M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gratton2019,
       author = {{Gratton}, Raffaele and {Bragaglia}, Angela and {Carretta}, Eugenio and {D'Orazi}, Valentina and {Lucatello}, Sara and {Sollima}, Antonio},
        title = "{What is a globular cluster? An observational perspective}",
      journal = {\aapr},
     keywords = {Globular clusters, Open clusters, The Galaxy, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = nov,
       volume = {27},
       number = {1},
          eid = {8},
        pages = {8},
          doi = {10.1007/s00159-019-0119-3},
archivePrefix = {arXiv},
       eprint = {1911.02835},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&ARv..27....8G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Allard2012,
       author = {{Allard}, F. and {Homeier}, D. and {Freytag}, B. and {Sharp}, C.~M.},
        title = "{Atmospheres From Very Low-Mass Stars to Extrasolar Planets}",
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
    booktitle = {EAS Publications Series},
         year = 2012,
       editor = {{Reyl{\'e}}, C{\'e}line and {Charbonnel}, Corinne and {Schultheis}, Mathias},
       series = {EAS Publications Series},
       volume = {57},
        month = nov,
        pages = {3-43},
          doi = {10.1051/eas/1257001},
archivePrefix = {arXiv},
       eprint = {1206.1021},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012EAS....57....3A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INCOLLECTION{Kurucz2014,
       author = {{Kurucz}, Robert L.},
        title = "{Model Atmosphere Codes: ATLAS12 and ATLAS9}",
    booktitle = {Determination of Atmospheric Parameters of B},
         year = 2014,
       editor = {{Niemczura}, Ewa and {Smalley}, Barry and {Pych}, Wojtek},
        pages = {39-51},
          doi = {10.1007/978-3-319-06956-2_4},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014dapb.book...39K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pauldrach1986,
       author = {{Pauldrach}, A. and {Puls}, J. and {Kudritzki}, R.~P.},
        title = "{Radiation-driven winds of hot luminous stars. Improvements of the theory and first results.}",
      journal = {\aap},
     keywords = {Hot Stars, Stellar Atmospheres, Stellar Radiation, Stellar Winds, Approximation, Photosphere, Radiation Pressure, Shock Waves, Stellar Magnetic Fields, Stellar Models, Stellar Rotation, Astrophysics},
         year = 1986,
        month = aug,
       volume = {164},
        pages = {86-100},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1986A&A...164...86P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Todt2015,
       author = {{Todt}, H. and {Sander}, A. and {Hainich}, R. and {Hamann}, W. -R. and {Quade}, M. and {Shenar}, T.},
        title = "{Potsdam Wolf-Rayet model atmosphere grids for WN stars}",
      journal = {\aap},
     keywords = {stars: evolution, stars: mass-loss, stars: winds, outflows, stars: Wolf-Rayet, stars: atmospheres, stars: massive},
         year = 2015,
        month = jul,
       volume = {579},
          eid = {A75},
        pages = {A75},
          doi = {10.1051/0004-6361/201526253},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...579A..75T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nomoto1984,
       author = {{Nomoto}, K. and {Thielemann}, F. -K. and {Yokoi}, K.},
        title = "{Accreting white dwarf models for type I supernovae. III. Carbon deflagration supernovae.}",
      journal = {\apj},
     keywords = {Carbon Stars, Deflagration, Nuclear Fusion, Stellar Mass Accretion, Supernovae, White Dwarf Stars, Hydrodynamics, Light Curve, Neutrinos, Stellar Composition, Stellar Models, Wave Propagation, Astrophysics},
         year = 1984,
        month = nov,
       volume = {286},
        pages = {644-658},
          doi = {10.1086/162639},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1984ApJ...286..644N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Takahashi2013,
       author = {{Takahashi}, Koh and {Yoshida}, Takashi and {Umeda}, Hideyuki},
        title = "{Evolution of Progenitors for Electron Capture Supernovae}",
      journal = {\apj},
     keywords = {nuclear reactions, nucleosynthesis, abundances, stars: evolution, stars: interiors, supernovae: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = jul,
       volume = {771},
       number = {1},
          eid = {28},
        pages = {28},
          doi = {10.1088/0004-637X/771/1/28},
archivePrefix = {arXiv},
       eprint = {1302.6402},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...771...28T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Miyaji1980,
       author = {{Miyaji}, S. and {Nomoto}, K. and {Yokoi}, K. and {Sugimoto}, D.},
        title = "{Supernova triggered by electron captures.}",
      journal = {\pasj},
         year = 1980,
        month = jan,
       volume = {32},
        pages = {303-329},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1980PASJ...32..303M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sanyal2015,
       author = {{Sanyal}, D. and {Grassitelli}, L. and {Langer}, N. and {Bestenlehner}, J.~M.},
        title = "{Massive main-sequence stars evolving at the Eddington limit}",
      journal = {\aap},
     keywords = {stars: evolution, stars: interiors, stars: massive, stars: mass-loss, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = aug,
       volume = {580},
          eid = {A20},
        pages = {A20},
          doi = {10.1051/0004-6361/201525945},
archivePrefix = {arXiv},
       eprint = {1506.02997},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...580A..20S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Miglio2012,
       author = {{Miglio}, A. and {Brogaard}, K. and {Stello}, D. and {Chaplin}, W.~J. and {D'Antona}, F. and {Montalb{\'a}n}, J. and {Basu}, S. and {Bressan}, A. and {Grundahl}, F. and {Pinsonneault}, M. and {Serenelli}, A.~M. and {Elsworth}, Y. and {Hekker}, S. and {Kallinger}, T. and {Mosser}, B. and {Ventura}, P. and {Bonanno}, A. and {Noels}, A. and {Silva Aguirre}, V. and {Szabo}, R. and {Li}, J. and {McCauliff}, S. and {Middour}, C.~K. and {Kjeldsen}, H.},
        title = "{Asteroseismology of old open clusters with Kepler: direct estimate of the integrated red giant branch mass-loss in NGC 6791 and 6819}",
      journal = {\mnras},
     keywords = {asteroseismology, stars: late-type, stars: mass-loss, open clusters and associations: individual: NGC 6791, open clusters and associations: individual: NGC 6819, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = jan,
       volume = {419},
       number = {3},
        pages = {2077-2088},
          doi = {10.1111/j.1365-2966.2011.19859.x},
archivePrefix = {arXiv},
       eprint = {1109.4376},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.419.2077M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fields2011,
       author = {{Fields}, Brian D.},
        title = "{The Primordial Lithium Problem}",
      journal = {Annual Review of Nuclear and Particle Science},
     keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics, High Energy Physics - Phenomenology, Nuclear Theory},
         year = 2011,
        month = nov,
       volume = {61},
       number = {1},
        pages = {47-68},
          doi = {10.1146/annurev-nucl-102010-130445},
archivePrefix = {arXiv},
       eprint = {1203.3551},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ARNPS..61...47F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Renzo2024,
       author = {{Renzo}, M. and {Smith}, N.},
        title = "{Pair-instability evolution and explosions in massive stars}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2024,
        month = jul,
          eid = {arXiv:2407.16113},
        pages = {arXiv:2407.16113},
          doi = {10.48550/arXiv.2407.16113},
archivePrefix = {arXiv},
       eprint = {2407.16113},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024arXiv240716113R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mehta2022,
       author = {{Mehta}, Ajit Kumar and {Buonanno}, Alessandra and {Gair}, Jonathan and {Miller}, M. Coleman and {Farag}, Ebraheem and {deBoer}, R.~J. and {Wiescher}, M. and {Timmes}, F.~X.},
        title = "{Observing Intermediate-mass Black Holes and the Upper Stellar-mass gap with LIGO and Virgo}",
      journal = {\apj},
     keywords = {675, 1043, 678, General Relativity and Quantum Cosmology, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2022,
        month = jan,
       volume = {924},
       number = {1},
          eid = {39},
        pages = {39},
          doi = {10.3847/1538-4357/ac3130},
archivePrefix = {arXiv},
       eprint = {2105.06366},
 primaryClass = {gr-qc},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJ...924...39M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Farag2022,
       author = {{Farag}, Ebraheem and {Renzo}, Mathieu and {Farmer}, Robert and {Chidester}, Morgan T. and {Timmes}, F.~X.},
        title = "{Resolving the Peak of the Black Hole Mass Spectrum}",
      journal = {\apj},
     keywords = {Gravitational waves, Black holes, Nuclear astrophysics, Stellar physics, Core-collapse supernovae, 678, 162, 1129, 1621, 304, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics, General Relativity and Quantum Cosmology},
         year = 2022,
        month = oct,
       volume = {937},
       number = {2},
          eid = {112},
        pages = {112},
          doi = {10.3847/1538-4357/ac8b83},
archivePrefix = {arXiv},
       eprint = {2208.09624},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJ...937..112F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Mestichelli2024,
       author = {{Mestichelli}, Benedetta and {Mapelli}, Michela and {Torniamenti}, Stefano and {Sedda}, Manuel Arca and {Branchesi}, Marica and {Costa}, Guglielmo and {Iorio}, Giuliano and {Santoliquido}, Filippo},
        title = "{Binary black hole mergers from Population III star clusters}",
      journal = {\aap},
     keywords = {black hole physics, gravitational waves, stars: black holes, stars: Population III, galaxies: star clusters: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2024,
        month = oct,
       volume = {690},
          eid = {A106},
        pages = {A106},
          doi = {10.1051/0004-6361/202450667},
archivePrefix = {arXiv},
       eprint = {2405.06037},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024A&A...690A.106M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Liu2024,
       author = {{Liu}, Boyuan and {Hartwig}, Tilman and {Sartorio}, Nina S. and {Dvorkin}, Irina and {Costa}, Guglielmo and {Santoliquido}, Filippo and {Fialkov}, Anastasia and {Klessen}, Ralf S. and {Bromm}, Volker},
        title = "{Gravitational waves from mergers of Population III binary black holes: roles played by two evolution channels}",
      journal = {\mnras},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2024,
        month = nov,
       volume = {534},
       number = {3},
        pages = {1634-1667},
          doi = {10.1093/mnras/stae2120},
archivePrefix = {arXiv},
       eprint = {2406.17397},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024MNRAS.534.1634L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Winters2000,
       author = {{Winters}, J.~M. and {Le Bertre}, T. and {Jeong}, K.~S. and {Helling}, Ch. and {Sedlmayr}, E.},
        title = "{A systematic investigation of the mass loss mechanism in dust forming long-period variable stars}",
      journal = {\aap},
     keywords = {HYDRODYNAMICS, STARS: WINDS, OUTFLOWS, STARS: CARBON, STARS: CIRCUMSTELLAR MATTER, STARS: MASS-LOSS, STARS: AGB AND POST-AGB},
         year = 2000,
        month = sep,
       volume = {361},
        pages = {641-659},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&A...361..641W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Herwig1997,
       author = {{Herwig}, F. and {Bloecker}, T. and {Schoenberner}, D. and {El Eid}, M.},
        title = "{Stellar evolution of low and intermediate-mass stars. IV. Hydrodynamically-based overshoot and nucleosynthesis in AGB stars.}",
      journal = {\aap},
     keywords = {STARS: EVOLUTION, STARS: AGB, POST-AGB, STARS: ABUNDANCES, Astrophysics},
         year = 1997,
        month = aug,
       volume = {324},
        pages = {L81-L84},
          doi = {10.48550/arXiv.astro-ph/9706122},
archivePrefix = {arXiv},
       eprint = {astro-ph/9706122},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997A&A...324L..81H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fu2015,
       author = {{Fu}, Xiaoting and {Bressan}, Alessandro and {Molaro}, Paolo and {Marigo}, Paola},
        title = "{Lithium evolution in metal-poor stars: from pre-main sequence to the Spite plateau}",
      journal = {\mnras},
     keywords = {stars abundances, stars: pre-main sequence, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = sep,
       volume = {452},
       number = {3},
        pages = {3256-3265},
          doi = {10.1093/mnras/stv1384},
archivePrefix = {arXiv},
       eprint = {1506.05993},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.452.3256F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Grisoni2017,
       author = {{Grisoni}, V. and {Spitoni}, E. and {Matteucci}, F. and {Recio-Blanco}, A. and {de Laverny}, P. and {Hayden}, M. and {Mikolaitis}, {\^{S}}. and {Worley}, C.~C.},
        title = "{The AMBRE project: chemical evolution models for the Milky Way thick and thin discs}",
      journal = {\mnras},
     keywords = {Galaxy: abundances, Galaxy: evolution, Galaxy: formation, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = dec,
       volume = {472},
       number = {3},
        pages = {3637-3647},
          doi = {10.1093/mnras/stx2201},
archivePrefix = {arXiv},
       eprint = {1706.02614},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.472.3637G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Micali2013,
       author = {{Micali}, A. and {Matteucci}, F. and {Romano}, D.},
        title = "{The chemical evolution of the Milky Way: the Three Infall Model}",
      journal = {\mnras},
     keywords = {Galaxy: abundances, Galaxy: evolution, Galaxy: formation, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = dec,
       volume = {436},
       number = {2},
        pages = {1648-1658},
          doi = {10.1093/mnras/stt1681},
archivePrefix = {arXiv},
       eprint = {1309.1283},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.436.1648M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kojima2020,
       author = {{Kojima}, Takashi and {Ouchi}, Masami and {Rauch}, Michael and {Ono}, Yoshiaki and {Nakajima}, Kimihiko and {Isobe}, Yuki and {Fujimoto}, Seiji and {Harikane}, Yuichi and {Hashimoto}, Takuya and {Hayashi}, Masao and {Komiyama}, Yutaka and {Kusakabe}, Haruka and {Kim}, Ji Hoon and {Lee}, Chien-Hsiu and {Mukae}, Shiro and {Nagao}, Tohru and {Onodera}, Masato and {Shibuya}, Takatoshi and {Sugahara}, Yuma and {Umemura}, Masayuki and {Yabe}, Kiyoto},
        title = "{Extremely Metal-poor Representatives Explored by the Subaru Survey (EMPRESS). I. A Successful Machine-learning Selection of Metal-poor Galaxies and the Discovery of a Galaxy with M* < {}10$^{6}$ M$_{{\ensuremath{\odot}}}$ and 0.016 Z$_{{\ensuremath{\odot}}}$}",
      journal = {\apj},
     keywords = {Galaxy evolution, Galaxy formation, Galaxy abundances, Interstellar medium, Emission nebulae, 594, 595, 574, 847, 461, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = aug,
       volume = {898},
       number = {2},
          eid = {142},
        pages = {142},
          doi = {10.3847/1538-4357/aba047},
archivePrefix = {arXiv},
       eprint = {1910.08559},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...898..142K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Izotov2018,
       author = {{Izotov}, Y.~I. and {Thuan}, T.~X. and {Guseva}, N.~G. and {Liss}, S.~E.},
        title = "{J0811+4730: the most metal-poor star-forming dwarf galaxy known}",
      journal = {\mnras},
     keywords = {galaxies: abundances, galaxies: dwarf, galaxies: ISM, galaxies: starburst, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = jan,
       volume = {473},
       number = {2},
        pages = {1956-1966},
          doi = {10.1093/mnras/stx2478},
archivePrefix = {arXiv},
       eprint = {1709.00202},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.473.1956I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Meynet2006,
       author = {{Meynet}, G. and {Ekstr{\"o}m}, S. and {Maeder}, A.},
        title = "{The early star generations: the dominant effect of rotation on the CNO yields}",
      journal = {\aap},
     keywords = {Astrophysics},
         year = 2006,
        month = feb,
       volume = {447},
       number = {2},
        pages = {623-639},
          doi = {10.1051/0004-6361:20053070},
archivePrefix = {arXiv},
       eprint = {astro-ph/0510560},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006A&A...447..623M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
